The Power-Oriented Graphs Modeling Technique: From the Fundamental Principles to the Systematic, Step-by-Step Modeling of Complex Physical Systems

Modeling physical systems is an essential skill for a control engineer, since it enables to achieve a deep understanding of their dynamic behavior and, consequently, the development of effective control strategies. The first part of this article provides a tutorial description of the fundamental principles and properties of the Power-Oriented Graphs (POG) modeling technique. Various case studies in different energetic domains are then presented to consolidate the fundamental principles, each highlighting different features of the POG modeling technique. The latter is then compared with the other two main graphical modeling techniques available in the literature, namely Bond Graph (BG) and Energetic Macroscopic Representation (EMR). The second part of this article assumes once again a tutorial nature, in order to introduce the new Fast Modeling POG (FMPOG) procedure. The FMPOG, which operates in the POG framework, is a methodical step-by-step procedure that enables the readers to quickly derive the power-oriented graphical model of physical systems starting from their schematics. From the power-oriented graphical model, the state-space model can then be directly determined. To ensure the FMPOG procedure is easily usable by the entire community, we apply it to three examples in different energetic domains in this article, guiding the reader step-by-step through the derivation of the physical systems models. A freely available Matlab/Simulink program is provided in a repository, allowing the users to automatically apply the FMPOG procedure to various classes of physical systems. This program allows to convert the physical systems schematics into the corresponding POG block schemes and, ultimately, into the state-space mathematical models.

==> BG_base_01_2010.tex <==
%
% Author: Zanasi Roberto
% e-mail: roberto.zanasi@unimo.it
% Date: 07 Dicember 2007
%
% This "reserved" file is given (and can be freely used) only
% to friends of Roberto Zanasi which use Power Oriented Graphs.
%

 \setlength{\unitlength}{1mm}
 \psset{unit=1.0\unitlength}
 \SpecialCoor

%%%%% Schema a blocchi Bond Graph

%%>>%%      'schemaBG','','\small Crea uno schema a blocchi Bond Graph:\\ \\ 1=(x,y);\\ 2=unitlength;\\ 3=blocchi.'
\newcommand{\schemaBG}[3]{
 \setlength{\unitlength}{#2}
 \psset{unit=1.0\unitlength}
 \SpecialCoor
 \begin{pspicture}#1
 \put(0,0){$#3$}
 \end{pspicture}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%>>%%      'schemaEMR','','\small Crea uno schema a blocchi EMR:\\ \\ 1=(x,y);\\ 2=unitlength;\\ 3=blocchi.'
\newcommand{\schemaEMR}[3]{
 \setlength{\unitlength}{#2}
 \psset{unit=1.0\unitlength}
 \SpecialCoor
 \begin{pspicture}#1
 \put(0,0){$#3$}
 \end{pspicture}
}

\newrgbcolor{greenSor}{0.8 1 0.8}
\newrgbcolor{rosaAcc}{1 0.8 0.6}

%%>>%%      'EMRspazio','','\small Inserisce uno spazio x negli schemi a blocchi EMR.'
\newcommand{\EMRspazio}[1]{\begin{picture}(#1,0)\end{picture}}

%%>>%%      'EMRlinee','{3}','\small Inserisce una linea x negli schemi a blocchi EMR.'
\newcommand{\EMRlinee}[1]{\begin{picture}(#1,0)\psline(0,1)(#1,1)\psline(0,4)(#1,4)\end{picture}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\BGdstdst}[4]{\begin{picture}(0,0)
   \rput(0,0){\psline(0.75,0)(3.25,0)(2.85,0.3)}
   \rput(0,0){$#1$}
   \rput[l](3.55,0){$#2$}
   \rput[b](1.8,0.2){$#3$}
   \rput[t](1.8,-0.2){$#4$}
   \end{picture}}


\newcommand{\BGsntsnt}[4]{\begin{picture}(0,0)
   \rput(0,0){\psline(-0.75,0)(-3.25,0)(-2.85,0.3)}
   \rput(0,0){$#1$}
   \rput[r](-3.55,0){$#2$}
   \rput[b](-1.8,0.2){$#3$}
   \rput[t](-1.8,-0.2){$#4$}
   \end{picture}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\NrSz}[1]{\small\cput[linewidth=0.3pt,framesep=1pt](0,0){\tiny #1}}

%%>>%%      'scrittabase','{1}{2}{3}{4}{5}{6}{7}{8}{9}(0,-10)(8,6)B','\small 1=xlarg\\ 2=xgiu\\ 3=scritta\\ 4=larg\\ 1=larg\\ 1=larg\\ 1=larg\\ 1=larg\\ '
\newcommand{\scrittabase}[9]{\begin{picture}(#1,0)
   \psline[linestyle=dashed,linewidth=0.2pt](0,-#2)
   \rput[#6](0,#5){#4}
   \put(0,0){#9}
   \psset{unit=0.5\unitlength}
   \put(0,-#8){\put(0,-#5){\rput[#7](#1,-#5){#3}}}
   \psset{unit=2.0\unitlength}
\end{picture}}


\newcommand{\scrittasutop}[7]{\scrittabase{#1}{#2}{#3}{#4}{#5}{b}{t}{#6}{#7}}
\newcommand{\BGscrittasutop}[5]{\scrittasutop{#1}{#2}{#3}{#4}{0.5}{#5}{0}}
\newcommand{\scrittasutoparr}[7]{\scrittasutop{#1}{#2}{#3}{#4}{#5}{#6}{\psline[linewidth=0.3pt,linestyle=dashed]{<->}(0,-#6)(#1,-#6)}}
\newcommand{\BGscrittasutoparr}[5]{\scrittasutoparr{#1}{#2}{#3}{#4}{0.5}{#5}{}}

%\newcommand{\EMRscrittasutop}[4]{\scrittasutop{#1}{#2}{#3}{#4}{0.5}}
%\newcommand{\EMRscrittasutoparr}[5]{\scrittasutoparr{#1}{#2}{#3}{#4}{0.5}{#5}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\EMRscritta}[2]{\begin{picture}(0,0)
   \psline[linewidth=0.3pt,linestyle=dashed]{<->}(0,0)(#1,0)
   \psset{unit=0.5\unitlength}
   \rput[b](#1,0.8){#2}
   \psset{unit=2.0\unitlength}
\end{picture}}

\newcommand{\EMRnrsezgiu}[2]{\begin{picture}(0,0)
 \rput[b](0,1){\small\cput[linewidth=0.3pt,framesep=1pt](0,0){\tiny #1}}
 \psline[linestyle=dashed,linewidth=0.2pt](0,-#2)
 \end{picture}}


%%>>%%      'EMRsorin','{1}{2}{3}(0,-2)(8,10)B',''
\newcommand{\EMRsorin}[3]{\begin{picture}(7.5,5)
 \psellipse[linecolor=green,fillstyle=solid,fillcolor=greenSor](3,2.5)(3,2)
 \rput(3,2.5){\normalsize #1}
 \psline(5,4)(7.5,4)
 \psline{<-}(5,1)(7.5,1)
 \rput[b](7.5,4.5){$#2$}
 \rput[t](7.5,0.5){$#3$}
\end{picture}}

\newcommand{\EMRsorout}[1]{\begin{picture}(7.5,5)
 \psellipse[linecolor=green,fillstyle=solid,fillcolor=greenSor](4.5,2.5)(3,2)
 \rput(4.5,2.5){\normalsize #1}
 \psline{->}(0,4)(2.5,4)
 \psline(0,1)(2.5,1)
\end{picture}}


\newcommand{\EMRacc}[2]{\begin{picture}(7,5)
 \psline{->}(0,4)(2.5,4)
 \psline(0,1)(2.5,1)
 \psframe[linecolor=red,fillstyle=solid,fillcolor=rosaAcc](2.5,0)(4.5,5)
 \psline[linecolor=red](2.5,0)(4.5,5)
 \psline(4.5,4)(7,4)
 \psline{<-}(4.5,1)(7,1)
 \rput[b](7,4.5){$#1$}
 \rput[t](7,0.5){$#2$}
\end{picture}}

\newcommand{\EMReleconuno}[2]{\begin{picture}(10,5)
 \psline{->}(0,4)(2.5,4)
 \psline(0,1)(2.5,1)
 \psframe[linecolor=red,fillstyle=solid,fillcolor=rosaAcc](2.5,0)(7.5,5)
 \psline(7.5,4)(10,4)
 \psline{<-}(7.5,1)(10,1)
 \rput[b](10,4.5){$#1$}
 \rput[t](10,0.5){$#2$}
\end{picture}}

\newcommand{\EMRmecconuno}[2]{\begin{picture}(10,5)
 \psline{->}(0,4)(4.5,4)
 \psline(0,1)(2.9,1)
 \psline(5.5,4)(10,4)
 \psline{<-}(7.1,1)(10,1)
 \pspolygon[linecolor=red,fillstyle=solid,fillcolor=rosaAcc](2.5,0)(7.5,0)(5,5)
 \rput[b](10,4.5){$#1$}
 \rput[t](10,0.5){$#2$}
\end{picture}}

%%>>%%      'EMRmeccongiudue','{1}{2}(0,-8)(8,20)B',''
\newcommand{\EMRmeccongiudue}[2]{\begin{picture}(10,5)
 \psline{->}(0,11)(2.0,11)(4.75,6.0)
 \psline(0,8)(1.5,8)(3.65,4.0)
 \psline{->}(0,-3)(2.0,-3)(3.5,-1.5)
 \psline(0,-6)(2.0,-6)(6.5,-1.5)
 %
 \psline(6.25,4)(10,4)
 \psline{<-}(6.25,1)(10,1)
 \pspolygon[linecolor=red,fillstyle=solid,fillcolor=rosaAcc](2.5,1.5)(7.5,1.5)(5,6.5)
 \pspolygon[linecolor=red,fillstyle=solid,fillcolor=rosaAcc](2.5,-1.5)(7.5,-1.5)(5,3.5)
 \pspolygon[linecolor=red](2.5,1.5)(7.5,1.5)(5,6.5)
 \rput[b](10,4.5){$#1$}
 \rput[t](10,0.5){$#2$}
\end{picture}}


\newcommand{\EMReleconsudue}[6]{\begin{picture}(11,5)
 \psline{->}(0,4)(2.5,4)
 \psline(0,1)(3.5,1)
 \psframe[linecolor=red,fillstyle=solid,fillcolor=rosaAcc](2.5,1.5)(7.5,6.5)
 \psframe[linecolor=red,fillstyle=solid,fillcolor=rosaAcc](3.5,-1.5)(8.5,3.5)
 \psframe[linecolor=red](2.5,1.5)(7.5,6.5)
 \psline(7.5,6.5)(11,6.5)
 \psline{<-}(8.5,3.5)(11,3.5)
 \rput[b](11,7.0){$#1$}
 \rput[b](11,4.0){$#2$}
 \psline(8.5,1.5)(11,1.5)
 \psline{<-}(8.5,-1.5)(11,-1.5)
 \rput[t](11,1.25){$#3$}
 \rput[t](11,-2.0){$#4$}
 \put(11,7){#5}
 \put(11,-7){#6}
\end{picture}}

\newcommand{\EMReleconsutre}[9]{\begin{picture}(12,5)
 \psline{->}(0,4)(2.5,4)
 \psline(0,1)(3.5,1)
 \psframe[linecolor=red,fillstyle=solid,fillcolor=rosaAcc](2.5,3)(7.5,8)
 \psframe[linecolor=red,fillstyle=solid,fillcolor=rosaAcc](3.5,0)(8.5,5)
 \psframe[linecolor=red,fillstyle=solid,fillcolor=rosaAcc](4.5,-3)(9.5,2)
 \psframe[linecolor=red](2.5,3)(7.5,8)
 \psframe[linecolor=red](3.5,0)(8.5,5)
 \psframe[linecolor=red](4.5,-3)(9.5,2)
 \psline(3.5,8)(9.5,15.5)(12,15.5)
 \psline{<-}(6.5,8)(10,12.5)(12,12.5)
 \rput[b](12,16.0){$#1$}
 \rput[t](12,12.0){$#2$}
 \psline(8.5,4)(12,4)
 \psline{<-}(9.5,1)(12,1)
 \rput[b](12,4.5){$#3$}
 \rput[t](12,0.5){$#4$}
 \psline(8.5,-3)(10,-7.5)(12,-7.5)
 \psline{<-}(5.5,-3)(8.25,-10.5)(12,-10.5)
 \rput[b](12,-7.0){$#5$}
 \rput[t](12,-11.0){$#6$}
 \put(12,11.5){#7}
 \put(12,0){#8}
 \put(12,-11.5){#9}
\end{picture}}

\newcommand{\EMRelmcongiudue}[2]{\begin{picture}(10,5)
 \psline{->}(0,-0.5)(1.5,-0.5)(2.65,0.5)
 \psline(0,-3.5)(2.0,-3.5)(4.5,-1.25)
 \psline(0,5.5)(1.5,5.5)(2.65,4.5)
 \psline{->}(0,8.5)(2.0,8.5)(4.5,6.25)
 \pscircle[linecolor=red,fillstyle=solid,fillcolor=rosaAcc](5,4){2.5}
 \pscircle[linecolor=red,fillstyle=solid,fillcolor=rosaAcc](5,1){2.5}
 \pscircle[linecolor=red](5,4){2.5}
 \psline(7.5,4)(10,4)
 \psline{<-}(7.5,1)(10,1)
 \rput[b](10,4.5){$#1$}
 \rput[t](10,0.5){$#2$}
\end{picture}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%>>%%      'fredst','(0,-6)(8,8)B',''
\newcommand{\fredst}{\psline(0.5;143.13)}

\newcommand{\fresnt}{\psline(0.5;36.87)}

\newcommand{\str}{\psline(0,-0.4)(0,0.4)}

\newcommand{\BGscritta}[2]{\begin{picture}(0,0)
   \psline[linewidth=0.3pt,linestyle=dashed]{<->}(0,0)(#1,0)
   \psset{unit=0.5\unitlength}
   \rput[b](#1,0.6){#2}
   \psset{unit=2.0\unitlength}
\end{picture}}

\newcommand{\BGnrsezgiu}[2]{\begin{picture}(0,0)
 \rput[b](0,0.5){\small\cput[linewidth=0.3pt,framesep=1pt](0,0){\tiny #1}}
 \psline[linestyle=dashed,linewidth=0.2pt](0,-#2)
 \end{picture}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\BGruota}[2]{\begin{picture}(0,0)\rput[l]{#1}(0,0){#2}\end{picture}}

\newcommand{\BGxlinebase}[8]{\begin{picture}(#1,0)
   \pnode(0.75,0){A}
   \put(-0.75,0){\pnode(#1,0){B}}
   \ncline{A}{B}
   \put(0.75,0){#4}
   \put(-0.75,0){\put(#1,0){#5}}
   \psset{unit=0.5\unitlength}
   \put(-0.2,0){\rput[#6]{#80}(#1,0.4){$#2$}}
   \put(-0.2,0){\rput[#7]{#80}(#1,-0.4){$#3$}}
   \psset{unit=2.0\unitlength}
   \end{picture}}

\newcommand{\BGab}[4]{\begin{picture}(0,0)
   \rput{*0}(0,0){$#2$}
   \put(-0.45,0){\rput[#4]{*0}(#1,0){$#3$}}
   \end{picture}}


%\newcommand{\BGxstrline}[3]{\BGxlinebase{#1}{#2}{#3}{\str}{\fredst}{b}{t}{}}
%\newcommand{\BGxlinestr}[3]{\BGxlinebase{#1}{#2}{#3}{}{\fredst\str}{b}{t}{}}

%%>>%%      'BGxthdststr','{5}{30}{3}{4}',''
%%>>%%      'BGxthstrdst','{5}{30}{3}{4}',''
%%>>%%      'BGxthsntstr','{5}{30}{3}{4}',''
%%>>%%      'BGxthstrsnt','{5}{30}{3}{4}','1=lung\\2=ang'
\newcommand{\BGxthdststr}[4]{\BGruota{#2}{\BGxlinebase{#1}{#3}{#4}{}{\fredst\str}{b}{t}{}}}
\newcommand{\BGxthstrdst}[4]{\BGruota{#2}{\BGxlinebase{#1}{#3}{#4}{\str}{\fredst}{b}{t}{}}}
\newcommand{\BGxthsntstr}[4]{\BGruota{#2}{\BGxlinebase{#1}{#3}{#4}{\fresnt}{\str}{b}{t}{}}}
\newcommand{\BGxthstrsnt}[4]{\BGruota{#2}{\BGxlinebase{#1}{#3}{#4}{\fresnt\str}{}{b}{t}{}}}
%
%%>>%%      'BGxthdststrAs','{5}{30}{3}{4}{b}{t}',''
%%>>%%      'BGxthstrdstAs','{5}{30}{3}{4}{b}{t}',''
%%>>%%      'BGxthsntstrAs','{5}{30}{3}{4}{b}{t}',''
%%>>%%      'BGxthstrsntAs','{5}{30}{3}{4}{b}{t}','5=t,b,l,r\\6=t,b,l,r'
\newcommand{\BGxthdststrAs}[6]{\BGruota{#2}{\BGxlinebase{#1}{#3}{#4}{}{\fredst\str}{#5}{#6}{*}}}
\newcommand{\BGxthstrdstAs}[6]{\BGruota{#2}{\BGxlinebase{#1}{#3}{#4}{\str}{\fredst}{#5}{#6}{*}}}
\newcommand{\BGxthsntstrAs}[6]{\BGruota{#2}{\BGxlinebase{#1}{#3}{#4}{\fresnt}{\str}{#5}{#6}{*}}}
\newcommand{\BGxthstrsntAs}[6]{\BGruota{#2}{\BGxlinebase{#1}{#3}{#4}{\fresnt\str}{}{#5}{#6}{*}}}
%
%
%%>>%%      'BGxdstdststr','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxdststrdst','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxdstsntstr','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxdststrsnt','{5}{2}{3}{4}{5}','1=lung'
\newcommand{\BGxdstdststr}[5]{\BGab{#1}{#2}{#3}{l}\BGxlinebase{#1}{#4}{#5}{}{\fredst\str}{b}{t}{}}
\newcommand{\BGxdststrdst}[5]{\BGab{#1}{#2}{#3}{l}\BGxlinebase{#1}{#4}{#5}{\str}{\fredst}{b}{t}{}}
\newcommand{\BGxdstsntstr}[5]{\BGab{#1}{#2}{#3}{l}\BGxlinebase{#1}{#4}{#5}{\fresnt}{\str}{b}{t}{}}
\newcommand{\BGxdststrsnt}[5]{\BGab{#1}{#2}{#3}{l}\BGxlinebase{#1}{#4}{#5}{\fresnt\str}{}{b}{t}{}}
%
%%>>%%      'BGxnenestr','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxnestrne','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxnesostr','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxnestrso','{5}{2}{3}{4}{5}','1=lung'
\newcommand{\BGxnenestr}[5]{\BGruota{45}{\BGab{#1}{#2}{#3}{lb}\BGxlinebase{#1}{#4}{#5}{}{\fredst\str}{br}{tl}{*}}}
\newcommand{\BGxnestrne}[5]{\BGruota{45}{\BGab{#1}{#2}{#3}{lb}\BGxlinebase{#1}{#4}{#5}{\str}{\fredst}{br}{tl}{*}}}
\newcommand{\BGxnesostr}[5]{\BGruota{45}{\BGab{#1}{#2}{#3}{lb}\BGxlinebase{#1}{#4}{#5}{\fresnt}{\str}{br}{tl}{*}}}
\newcommand{\BGxnestrso}[5]{\BGruota{45}{\BGab{#1}{#2}{#3}{lb}\BGxlinebase{#1}{#4}{#5}{\fresnt\str}{}{br}{tl}{*}}}
%
%%>>%%      'BGxsusustr','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxsustrsu','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxsugiustr','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxsustrgiu','{5}{2}{3}{4}{5}','1=lung'
\newcommand{\BGxsusustr}[5]{\BGruota{90}{\BGab{#1}{#2}{#3}{b}\BGxlinebase{#1}{#4}{#5}{}{\fredst\str}{r}{l}{*}}}
\newcommand{\BGxsustrsu}[5]{\BGruota{90}{\BGab{#1}{#2}{#3}{b}\BGxlinebase{#1}{#4}{#5}{\str}{\fredst}{r}{l}{*}}}
\newcommand{\BGxsugiustr}[5]{\BGruota{90}{\BGab{#1}{#2}{#3}{b}\BGxlinebase{#1}{#4}{#5}{\fresnt}{\str}{r}{l}{*}}}
\newcommand{\BGxsustrgiu}[5]{\BGruota{90}{\BGab{#1}{#2}{#3}{b}\BGxlinebase{#1}{#4}{#5}{\fresnt\str}{}{r}{l}{*}}}
%
%%>>%%      'BGxnonostr','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxnostrno','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxnosestr','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxnostrse','{5}{2}{3}{4}{5}','1=lung'
\newcommand{\BGxnonostr}[5]{\BGruota{135}{\BGab{#1}{#2}{#3}{br}\BGxlinebase{#1}{#5}{#4}{}{\fredst\str}{rt}{lb}{*}}}
\newcommand{\BGxnostrno}[5]{\BGruota{135}{\BGab{#1}{#2}{#3}{br}\BGxlinebase{#1}{#5}{#4}{\str}{\fredst}{rt}{lb}{*}}}
\newcommand{\BGxnosestr}[5]{\BGruota{135}{\BGab{#1}{#2}{#3}{br}\BGxlinebase{#1}{#5}{#4}{\fresnt}{\str}{rt}{lb}{*}}}
\newcommand{\BGxnostrse}[5]{\BGruota{135}{\BGab{#1}{#2}{#3}{br}\BGxlinebase{#1}{#5}{#4}{\fresnt\str}{}{rt}{lb}{*}}}
%
%%>>%%      'BGxsntsntstr','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxsntstrsnt','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxsntdststr','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxsntstrdst','{5}{2}{3}{4}{5}','1=lung'
\newcommand{\BGxsntsntstr}[5]{\BGruota{180}{\BGab{#1}{#2}{#3}{r}\BGxlinebase{#1}{#5}{#4}{}{\fredst\str}{t}{b}{*}}}
\newcommand{\BGxsntstrsnt}[5]{\BGruota{180}{\BGab{#1}{#2}{#3}{r}\BGxlinebase{#1}{#5}{#4}{\str}{\fredst}{t}{b}{*}}}
\newcommand{\BGxsntdststr}[5]{\BGruota{180}{\BGab{#1}{#2}{#3}{r}\BGxlinebase{#1}{#5}{#4}{\fresnt}{\str}{t}{b}{*}}}
\newcommand{\BGxsntstrdst}[5]{\BGruota{180}{\BGab{#1}{#2}{#3}{r}\BGxlinebase{#1}{#5}{#4}{\fresnt\str}{}{t}{b}{*}}}
%
%%>>%%      'BGxsosostr','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxsostrso','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxsonestr','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxsostrne','{5}{2}{3}{4}{5}','1=lung'
\newcommand{\BGxsosostr}[5]{\BGruota{-135}{\BGab{#1}{#2}{#3}{tr}\BGxlinebase{#1}{#5}{#4}{}{\fredst\str}{lt}{rb}{*}}}
\newcommand{\BGxsostrso}[5]{\BGruota{-135}{\BGab{#1}{#2}{#3}{tr}\BGxlinebase{#1}{#5}{#4}{\str}{\fredst}{lt}{rb}{*}}}
\newcommand{\BGxsonestr}[5]{\BGruota{-135}{\BGab{#1}{#2}{#3}{tr}\BGxlinebase{#1}{#5}{#4}{\fresnt}{\str}{lt}{rb}{*}}}
\newcommand{\BGxsostrne}[5]{\BGruota{-135}{\BGab{#1}{#2}{#3}{tr}\BGxlinebase{#1}{#5}{#4}{\fresnt\str}{}{lt}{rb}{*}}}
%
%%>>%%      'BGxgiugiustr','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxgiustrgiu','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxgiusustr','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxgiustrsu','{5}{2}{3}{4}{5}','1=lung'
\newcommand{\BGxgiugiustr}[5]{\BGruota{-90}{\BGab{#1}{#2}{#3}{t}\BGxlinebase{#1}{#5}{#4}{}{\fredst\str}{l}{r}{*}}}
\newcommand{\BGxgiustrgiu}[5]{\BGruota{-90}{\BGab{#1}{#2}{#3}{t}\BGxlinebase{#1}{#5}{#4}{\str}{\fredst}{l}{r}{*}}}
\newcommand{\BGxgiusustr}[5]{\BGruota{-90}{\BGab{#1}{#2}{#3}{t}\BGxlinebase{#1}{#5}{#4}{\fresnt}{\str}{l}{r}{*}}}
\newcommand{\BGxgiustrsu}[5]{\BGruota{-90}{\BGab{#1}{#2}{#3}{t}\BGxlinebase{#1}{#5}{#4}{\fresnt\str}{}{l}{r}{*}}}
%
%%>>%%      'BGxsesestr','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxsestrse','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxsenostr','{5}{2}{3}{4}{5}',''
%%>>%%      'BGxsestrno','{5}{2}{3}{4}{5}','1=lung'
\newcommand{\BGxsesestr}[5]{\BGruota{-45}{\BGab{#1}{#2}{#3}{lt}\BGxlinebase{#1}{#4}{#5}{}{\fredst\str}{bl}{tr}{*}}}
\newcommand{\BGxsestrse}[5]{\BGruota{-45}{\BGab{#1}{#2}{#3}{lt}\BGxlinebase{#1}{#4}{#5}{\str}{\fredst}{bl}{tr}{*}}}
\newcommand{\BGxsenostr}[5]{\BGruota{-45}{\BGab{#1}{#2}{#3}{lt}\BGxlinebase{#1}{#4}{#5}{\fresnt}{\str}{bl}{tr}{*}}}
\newcommand{\BGxsestrno}[5]{\BGruota{-45}{\BGab{#1}{#2}{#3}{lt}\BGxlinebase{#1}{#4}{#5}{\fresnt\str}{}{bl}{tr}{*}}}
%
%
%%>>%%      'BGdstdststr','{1}{2}{3}{4}(0,-6)(8,8)B',''
\newcommand{\BGdstdststr}[4]{\BGxdstdststr{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGdststrdst}[4]{\BGxdststrdst{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGdstsntstr}[4]{\BGxdstsntstr{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGdststrsnt}[4]{\BGxdststrsnt{4}{#1}{#2}{#3}{#4}}
%
\newcommand{\BGnenestr}[4]{\BGxnenestr{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGnestrne}[4]{\BGxnestrne{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGnesostr}[4]{\BGxnesostr{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGnestrso}[4]{\BGxnestrso{4}{#1}{#2}{#3}{#4}}
%
\newcommand{\BGsusustr}[4]{\BGxsusustr{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGsustrsu}[4]{\BGxsustrsu{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGsugiustr}[4]{\BGxsugiustr{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGsustrgiu}[4]{\BGxsustrgiu{4}{#1}{#2}{#3}{#4}}
%
\newcommand{\BGnonostr}[4]{\BGxnonostr{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGnostrno}[4]{\BGxnostrno{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGnosestr}[4]{\BGxnosestr{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGnostrse}[4]{\BGxnostrse{4}{#1}{#2}{#3}{#4}}
%
\newcommand{\BGsntsntstr}[4]{\BGxsntsntstr{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGsntstrsnt}[4]{\BGxsntstrsnt{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGsntdststr}[4]{\BGxsntdststr{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGsntstrdst}[4]{\BGxsntstrdst{4}{#1}{#2}{#3}{#4}}
%
\newcommand{\BGsosostr}[4]{\BGxsosostr{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGsostrso}[4]{\BGxsostrso{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGsonestr}[4]{\BGxsonestr{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGsostrne}[4]{\BGxsostrne{4}{#1}{#2}{#3}{#4}}
%
\newcommand{\BGgiugiustr}[4]{\BGxgiugiustr{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGgiustrgiu}[4]{\BGxgiustrgiu{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGgiusustr}[4]{\BGxgiusustr{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGgiustrsu}[4]{\BGxgiustrsu{4}{#1}{#2}{#3}{#4}}
%
\newcommand{\BGsesestr}[4]{\BGxsesestr{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGsestrse}[4]{\BGxsestrse{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGsenostr}[4]{\BGxsenostr{4}{#1}{#2}{#3}{#4}}
\newcommand{\BGsestrno}[4]{\BGxsestrno{4}{#1}{#2}{#3}{#4}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\SbaseBf}[5]{\begin{picture}(#3,0)
\psset{unit=0.5\unitlength}
\put(#3,-0.6){\makebox(0,0)[#2]{\shortstack{$#1$\\[-0.5mm].\,.\\[-0.5mm]#5 #4}}}
\psset{unit=2.0\unitlength}
\end{picture}}
%
\newcommand{\Se}[3]{\SbaseBf{#1}{#2}{#3}{Se}{\bf}}
\newcommand{\Sf}[3]{\SbaseBf{#1}{#2}{#3}{Sf}{\bf}}
\newcommand{\TF}[3]{\SbaseBf{#1}{#2}{#3}{TF}{\bf}}
\newcommand{\MTF}[3]{\SbaseBf{#1}{#2}{#3}{MTF}{\bf}}
\newcommand{\GY}[3]{\SbaseBf{#1}{#2}{#3}{GY}{\bf}}
\newcommand{\MGY}[3]{\SbaseBf{#1}{#2}{#3}{MGY}{\bf}}
%
\newcommand{\nSe}[3]{\SbaseBf{#1}{#2}{#3}{Se}{}}
\newcommand{\nSf}[3]{\SbaseBf{#1}{#2}{#3}{Sf}{}}
\newcommand{\nTF}[3]{\SbaseBf{#1}{#2}{#3}{TF}{}}
\newcommand{\nMTF}[3]{\SbaseBf{#1}{#2}{#3}{MTF}{}}
\newcommand{\nGY}[3]{\SbaseBf{#1}{#2}{#3}{GY}{}}
\newcommand{\nMGY}[3]{\SbaseBf{#1}{#2}{#3}{MGY}{}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\SbaseBfgiu}[5]{\begin{picture}(#3,0)
\psset{unit=0.5\unitlength}
\put(#3,0.6){\makebox(0,0)[#2]{\shortstack{#4\\[-0.5mm].\,.\\[-0.5mm]#5 $#1$}}}
\psset{unit=2.0\unitlength}
\end{picture}}
%
\newcommand{\Segiu}[3]{\SbaseBfgiu{#1}{#2}{#3}{Se}{\bf}}
\newcommand{\Sfgiu}[3]{\SbaseBfgiu{#1}{#2}{#3}{Sf}{\bf}}
\newcommand{\TFgiu}[3]{\SbaseBfgiu{#1}{#2}{#3}{TF}{\bf}}
\newcommand{\MTFgiu}[3]{\SbaseBfgiu{#1}{#2}{#3}{MTF}{\bf}}
\newcommand{\GYgiu}[3]{\SbaseBfgiu{#1}{#2}{#3}{GY}{\bf}}
\newcommand{\MGYgiu}[3]{\SbaseBfgiu{#1}{#2}{#3}{MGY}{\bf}}
%
\newcommand{\nSegiu}[3]{\SbaseBfgiu{#1}{#2}{#3}{Se}{}}
\newcommand{\nSfgiu}[3]{\SbaseBfgiu{#1}{#2}{#3}{Sf}{}}
\newcommand{\nTFgiu}[3]{\SbaseBfgiu{#1}{#2}{#3}{TF}{}}
\newcommand{\nMTFgiu}[3]{\SbaseBfgiu{#1}{#2}{#3}{MTF}{}}
\newcommand{\nGYgiu}[3]{\SbaseBfgiu{#1}{#2}{#3}{GY}{}}
\newcommand{\nMGYgiu}[3]{\SbaseBfgiu{#1}{#2}{#3}{MGY}{}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\BGspazio}[1]{\begin{picture}(#1,0)\end{picture}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Ebase}[2]{\mbox{#1:\,}#2}

\newcommand{\bR}[1]{\Ebase{\bf R}{#1}}
\newcommand{\bI}[1]{\Ebase{\bf I}{#1}}
\newcommand{\bC}[1]{\Ebase{\bf C}{#1}}
%
\newcommand{\nR}[1]{\Ebase{R}{#1}}
\newcommand{\nI}[1]{\Ebase{I}{#1}}
\newcommand{\nC}[1]{\Ebase{C}{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> MCSEM_Luc_base_2023.tex <==
   \oddsidemargin -1.5cm
   \evensidemargin -1.5cm
   \topmargin -2.2cm
   \parindent      = 0cm

   \setlength{\textwidth}{18.5cm}
   \setlength{\textheight}{26cm}

% \definecolor{mygreen}{RGB}{28,172,0}
% \lstset{language=Matlab,
%      basicstyle=\scriptsize\ttfamily,
%%      basicstyle=\footnotesize\ttfamily,
%      numberstyle=\tiny,
%      commentstyle=\color{mygreen},
%      stepnumber=0.1,
%      frame=single,
%      rulecolor=\color{blue},
%}

 \definecolor{mygreen}{RGB}{28,172,0}
 \newcommand{\setlarge}{
 \lstset{language=Matlab,
      basicstyle=\scriptsize\ttfamily,
      %basicstyle=\tiny\ttfamily,
      numberstyle=\tiny,
      commentstyle=\color{mygreen},
      stepnumber=0.1,
      frame=single,
      rulecolor=\color{blue}}
      } % setlargs

 \newcommand{\setsmall}{
 \lstset{language=Matlab,
        deletekeywords={zeros,length,max,min,interp2},
        %basicstyle=\scriptsize\ttfamily,
        basicstyle=\tiny,
        numberstyle=\tiny,
        commentstyle=\color{mygreen},
        keywordstyle=\color{blue},
%       stringstyle=\color{red},
        stepnumber=0.1,
        numbers=left,
        firstnumber = 1,
        numberfirstline=false,
        stepnumber=1,
        %rulecolor=\color{black},
        frame=single,
        rulecolor=\color{blue},
 }
 } % setsmall

 \setsmall


\newrgbcolor{verylightgiallo}{0.99    0.99   0.82 }
\newrgbcolor{verylightmagenta}{1  0.85  1    }
\newrgbcolor{verylightgrigio}{0.85 0.85 0.85    }
\newrgbcolor{lightgrigio}{0.75 0.75 0.75    }
\newrgbcolor{verylightverde}{0.75 1 0.75    }
%\newrgbcolor{verylightciano}{1  0  1    }

 \newcommand{\sign}[1]{\mbox{sign}(#1)}


 \def\bPhi{{\bf \Phi}} \def\bphi{{\bf \phi}}
  %\newcommand{\vero}{\bigcirc}
 \newcommand{\vero}{\bigotimes}
 \newcommand{\falso}{\bigcirc}
\newcommand{\PER}[1]{[#1\times\!]}
\newcommand{\zero}{{\bf 0}}
\newcommand{\IC}[1]{|\![ #1]\!|\,\!}
\newcommand{\vtheta}{\vec{\theta}}
\newcommand{\vomega}{\vec{\omega}}
\newcommand{\hfi}{\hspace{0.4cm} }
\newcommand{\hfii}{\hspace{0.8cm} }
\newcommand{\hfiii}{\hspace{1.2cm} }
 \newrgbcolor{verylightgray}{0.85 0.85 0.85}
 \newcommand{\matll}[5]{
  \begin{array}{@{}c@{}}
     \scr #1 \hfill \scr #3 \\[-1.5mm]
     \left|\!\left[\;#5\;\right]\!\right|\\[-1.5mm]
     \scr #2 \hfill  \scr #4
  \end{array}}



%  \newcommand{\nuovasezione}[2]{
%  \setcounter{section}{#1}
%  \setcounter{page}{1}
%  \markboth
%  {Zanasi Roberto -  Modeling and Control of Electromechanical Systems \hfill A.A.~2017/2018}
%  {Chapter\ \thesection.\ \MakeUppercase{#2}}
% }
%

  \newcommand{\nomecapitolo}{}
  \newcommand{\nomesezione}{}


  \newcommand{\nuovocapitolo}[2]{
  \setcounter{section}{#1}
  \setcounter{subsection}{0}
  \setcounter{page}{1}
  \renewcommand{\nomecapitolo}{#2 }
  \markboth
  {\thesubsection.\  \MakeUppercase{\nomesezione}}  %\MakeUppercase{#2}}
  { R.~Zanasi (UNIMORE) - MCEMS 2023/24 \hfill  \thesection. \nomecapitolo}
 }

  \newcommand{\nuovasezione}[2]{
  \setcounter{subsection}{#1}
  \setcounter{page}{1}
  \renewcommand{\nomesezione}{#2}
  \markboth
  {\thesubsection.\  \MakeUppercase{\nomesezione}}  %\MakeUppercase{#2}}
  { R.~Zanasi (UNIMORE) - MCEMS 2023/24 \hfill  \thesection. \nomecapitolo}
%  {\thesubsection.\  \MakeUppercase{\nomesezione}}  %\MakeUppercase{#2}}
%  { R.~Zanasi  -  Modeling and Control of Electromechanical Systems - 2020/21 \hfill  \thesection. \MakeUppercase{\nomecapitolo}}
 }


 \newcommand{\nuovoparagrafo}[1]{
  \markboth
  {Zanasi Roberto -  Modeling and Control of Electromechanical Systems \hfill A.A.~2023/2024}
  {Chapter\ \thesection.\ \MakeUppercase{#1}}
 }

 \newcommand{\titolo}[1]{
  \begin{center}
   \psshadowbox[framesep=4mm]{\huge #1} %%%% \MakeUppercase{#1}}
  \end{center}}

   \newcommand{\titolosezione}[1]{
  \begin{center}
   \psshadowbox[framesep=4mm]{\LARGE #1} %%%% \MakeUppercase{#1}}
  \end{center}}
 \newcommand{\titoloparagrafo}[1]{
  \begin{center}
   \psshadowbox[framesep=4mm]{\Large #1} %%%% \MakeUppercase{#1}}
  \end{center}}

 \newcommand{\PoloD}[1]{\underbrace{#1}_{\mbox{\scriptsize polo dominante}}}
 \newcommand{\PoliD}[1]{\underbrace{#1}_{\mbox{\scriptsize poli dominanti}}}


 \newcommand{\Esempio}[1]{\noindent{\large  {\bf Example.} #1}}

 \renewcommand{\tras}{^{T}}
 \renewcommand{\mtras}{^{-T}}


% Funzione di transizione dello stato:
\newcommand{\trans}{\psi}

% Funzione di uscita:
 \newcommand{\uscita}{\eta}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Insieme di raggiungibilit\`a
\newcommand{\ragg}{{\cal X}^{+}}
\newcommand{\SotRag}{{\cal X}^{+}}
% Matrice di raggiungibilit\`a
\newcommand{\Mragg}{{\cal R}^{+}}
\newcommand{\MatRag}{{\cal R}^{+}}

% Insieme di controllabilit\`a
\newcommand{\contr}{{\cal X}^{-}}
\newcommand{\SotCon}{{\cal X}^{-}}
% Matrice di controllabilit\`a
\newcommand{\Mcontr}{{\cal R}^{-}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Insieme di osservabilit\`a
\def\oss{{\cal E}^{-}}
\def\SotNonOss{{\cal E}^{-}}
% Matrice di osservabilit\`a
\def\Moss{{\cal O}^{-}}
\def\MatOss{{\cal O}^{-}}

% Insieme di ricostruibilit\`a
\def\ric{{\cal E}^{+}}
\def\SotRic{{\cal E}^{+}}
% Matrice di ricostruibilit\`a
\def\Mric{{\cal O}^{+}}

% Definizioni vettoriali:

\def\bPhi{{\bf \Phi}} \def\bphi{{\bf \phi}}
\def\definisci{\stackrel{\triangle}{=}}
\def\separa{\begin{center} --------------\end{center}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \renewcommand{\punto}{\begin{picture}(0,1)
%    \put(0,0){\circle*{0.3}}
% \end{picture}}

 \newcommand{\molorz}[2]{\begin{picture}(6,2)(0,0)
    \pszigzag[coilwidth=1,coilarm=1,linearc=0](0,0)(6,0)
    \put(  3, 1.05){\makebox(0,0)[b]{$#1$}}
    \put(  3,-1.05){\makebox(0,0)[t]{$#2$}}
    \end{picture}}
 \newcommand{\molver}[2]{\begin{picture}(6,2)
    \pszigzag[coilwidth=1,coilarm=1,linearc=0](0,0)(0,6)
    \put(-1.05,3){\makebox(0,0)[r]{$#1$}}
    \put( 1.05,3){\makebox(0,0)[l]{$#2$}}
    \end{picture}}          %%%% end Molla
 %
\newcommand{\indorz}[2]{\begin{picture}(6,2)
  \pscoil[coilarm=1.2,coilwidth=1](0,0)(6,0)
  \put(  3, 1.15){\makebox(0,0)[b]{$#1$}}
  \put(  3,-0.9){\makebox(0,0)[t]{$#2$}}
  \end{picture}}
\newcommand{\indver}[2]{\begin{picture}(6,2)
  \pscoil[coilarm=1.2,coilwidth=1](0,0)(0,6)
  \put(-1.15,3){\makebox(0,0)[r]{$#1$}}
  \put( 0.9,3){\makebox(0,0)[l]{$#2$}}
 %  \put(0,4.75){\line(0,1){1.25}}
 % \put(0,   0){\line(0,1){1.25}}
\end{picture}
}
 %
\newcommand{\capver}[2]{\begin{picture}(2,6)
  \put(-1.15,3){\makebox(0,0)[r]{$#1$}}
  \put( 1.15,3){\makebox(0,0)[l]{$#2$}}
  \put(0,  0){\line(0,1){2.5}}
  \put(0,3.5){\line(0,1){2.5}}
  \put(-1,2.5){\line(1,0){2}}
  \put(-1,3.5){\line(1,0){2}}
\end{picture}
}
%\newcommand{\blovisuaor}[3]{\begin{picture}(8,10)
%   \put(0, 0){\tratteggio}
%   \put(0,10){\sumsntsntvi{#3}}
%   \put(3, 0){\midsuvipiu{#1}{#2}}
%   \put(0, 0){\dotdstdstvi}
%\end{picture}}


==> pogbase_08_2015.tex <==
%
% Author: Zanasi Roberto
% e-mail: roberto.zanasi@unimore.it
% Date: 21 Dicember 2009
%
% This "reserved" file is given (and can be freely used) only
% to friends of Roberto Zanasi which use Power Oriented Graphs.
%

 \setlength{\unitlength}{1mm}
 \psset{unit=1.0\unitlength}
 \SpecialCoor

%%%%% Schema a blocchi POG

%%>>%%      'schemaPOG','','\small Crea uno schema a blocchi POG:\\ \\ 1=(x,y);\\ 2=unitlength;\\ 3=blocchi.'
\newcommand{\schemaPOG}[3]{
 \setlength{\unitlength}{#2}
 \psset{unit=1.0\unitlength}
 \SpecialCoor
 \begin{pspicture}#1
 \put(0,0){$#3$}
 \end{pspicture}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\punto}{\pscircle*{0.15}}

\newcommand{\tratteggio}{\psline[linestyle=dashed,linewidth=0.2pt](0,-0.75)(0,10.75)}

%%>>%%      'NOtratteggio','','\small Colora di bianco il comando ``tratteggio''.'
\newcommand{\NOtratteggio}[1]{\rput(#1,0){\psline[linestyle=dashed,linecolor=white,linewidth=0.4pt](0,-0.75)(0,10.75)}}

%%>>%%      'addspace','','\small Aggiunge uno spazio tra due blocchi POG.'
\newcommand{\addspace}[1]{\begin{picture}(#1,0)
\end{picture}}

\newcommand{\piu}{\begin{picture}(0,0)
 \put(0,0){\pscircle[linewidth=0.4pt]{0.5}}
 \psline(0.5; 45)(0.5;225)
 \psline(0.5;315)(0.5;135)
\end{picture}}

\newcommand{\dst}{\begin{picture}(0,0)
 \put(0.293,0){\pscircle*{0.207}}
\end{picture}}

\newcommand{\snt}{\begin{picture}(0,0)
 \put(-0.293,0){\pscircle*{0.207}}
\end{picture}}

\newcommand{\giu}{\begin{picture}(0,0)
 \put(0      ,-0.293 ){\pscircle*{0.207}}
\end{picture}}

\newcommand{\su}{\begin{picture}(0,0)
 \put(0      ,0.293 ){\pscircle*{0.207}}
\end{picture}}

%%%%%%%%%%%%%%%%

\newcommand{\POGcontdst}{\begin{picture}(0,10)
   \put(0.5,5){\makebox(0,0)[l]{{\Large$\cdots$}}}
\end{picture}}

\newcommand{\POGcontsnt}{\begin{picture}(0,10)
   \put(-0.5,5){\makebox(0,0)[r]{{\Large$\cdots$}}}
\end{picture}}

%%%%%%%%%%%%%%%%

\newcommand{\addgiuvar}[3]{\begin{picture}(0,10)
   \put(#1,-2){\vector(0,1){1.5}}
   \put(#1,-2){\punto}
   \put(#1,-2){\put(0.5,0){\makebox(0,0)[l]{$#2$}}}
   \put(#1,0){#3}
\end{picture}}

\newcommand{\addsuvar}[3]{\begin{picture}(0,10)
   \put(#1,12){\vector(0,-1){1.5}}
   \put(#1,12){\punto}
   \put(#1,12){\put(0.5,0){\makebox(0,0)[l]{$#2$}}}
   \put(#1,10){#3}
\end{picture}}

\newcommand{\escigiuvar}[2]{\begin{picture}(0,10)
   \put(#1,0){\vector(0,-1){2}}
   \put(#1,-2){\punto}
   \put(#1,-2){\put(0.5,0){\makebox(0,0)[l]{$#2$}}}
\end{picture}}

%%>>%%      'escisuvar','{1}{2}','\small addgiuvar(x,2,3), \\addsuvar(x,2,3), \\escigiuvar(x,2), \\escisuvar(x,2): \\ \\ x = posizione.'
\newcommand{\escisuvar}[2]{\begin{picture}(0,10)
   \put(#1,10){\vector(0,1){2}}
   \put(#1,12){\punto}
   \put(#1,12){\put(0.5,0){\makebox(0,0)[l]{$#2$}}}
\end{picture}}

%%%%%%%%%%%%%%%%

\newcommand{\sumdstsnt}[1]{\begin{picture}(0,1)
   \put(4,0){\piu}
   \put(4,0){#1}
   \put(0,0){\vector(1,0){3.5}}
   \put(8,0){\vector(-1,0){3.5}}
\end{picture}}

\newcommand{\sumdstdst}[1]{\begin{picture}(0,1)
   \put(4,0){\piu}
   \put(4,0){#1}
   \put(0,0){\vector(1,0){3.5}}
   \put(4.5,0){\vector(1,0){3.5}}
\end{picture}}

\newcommand{\sumsntsnt}[1]{\begin{picture}(0,1)
   \put(4,0){\piu}
   \put(4,0){#1}
   \put(3.5,0){\vector(-1,0){3.5}}
   \put(8,0){\vector(-1,0){3.5}}
\end{picture}}

\newcommand{\sumsntdst}[1]{\begin{picture}(0,1)
   \put(4,0){\piu}
   \put(4,0){#1}
   \put(3.5,0){\vector(-1,0){3.5}}
   \put(4.5,0){\vector(1,0){3.5}}
\end{picture}}

%%%% vi

\newcommand{\sumdstsntvi}[1]{\begin{picture}(0,1)
   \put(3,0){\piu}
   \put(3,0){#1}
   \put(0,0){\vector(1,0){2.5}}
   \put(6,0){\vector(-1,0){2.5}}
\end{picture}}

\newcommand{\sumdstdstvi}[1]{\begin{picture}(0,1)
   \put(3,0){\piu}
   \put(3,0){#1}
   \put(0,0){\vector(1,0){2.5}}
   \put(3.5,0){\vector(1,0){2.5}}
\end{picture}}

\newcommand{\sumsntsntvi}[1]{\begin{picture}(0,1)
   \put(3,0){\piu}
   \put(3,0){#1}
   \put(2.5,0){\vector(-1,0){2.5}}
   \put(6,0){\vector(-1,0){2.5}}
\end{picture}}

\newcommand{\sumsntdstvi}[1]{\begin{picture}(0,1)
   \put(3,0){\piu}
   \put(3,0){#1}
   \put(2.5,0){\vector(-1,0){2.5}}
   \put(3.5,0){\vector(1,0){2.5}}
\end{picture}}

%%%% iv

\newcommand{\sumdstsntiv}[1]{\begin{picture}(0,1)
   \put(2,0){\piu}
   \put(2,0){#1}
   \put(0,0){\vector(1,0){1.5}}
   \put(4,0){\vector(-1,0){1.5}}
\end{picture}}

\newcommand{\sumdstdstiv}[1]{\begin{picture}(0,1)
   \put(2,0){\piu}
   \put(2,0){#1}
   \put(0,0){\vector(1,0){1.5}}
   \put(2.5,0){\vector(1,0){1.5}}
\end{picture}}

\newcommand{\sumsntsntiv}[1]{\begin{picture}(0,1)
   \put(2,0){\piu}
   \put(2,0){#1}
   \put(1.5,0){\vector(-1,0){1.5}}
   \put(4,0){\vector(-1,0){1.5}}
\end{picture}}

\newcommand{\sumsntdstiv}[1]{\begin{picture}(0,1)
   \put(2,0){\piu}
   \put(2,0){#1}
   \put(1.5,0){\vector(-1,0){1.5}}
   \put(2.5,0){\vector(1,0){1.5}}
\end{picture}}

%%%%

\newcommand{\dotdstsnt}{\begin{picture}(0,1)
   \put(4,0){\punto}
   \put(0,0){\vector(1,0){4}}
   \put(8,0){\vector(-1,0){4}}
\end{picture}}

\newcommand{\dotdstdst}{\begin{picture}(0,1)
   \put(4,0){\punto}
   \put(0,0){\vector(1,0){4}}
   \put(4,0){\vector(1,0){4}}
\end{picture}}

\newcommand{\dotsntsnt}{\begin{picture}(0,1)
   \put(4,0){\punto}
   \put(4,0){\vector(-1,0){4}}
   \put(8,0){\vector(-1,0){4}}
\end{picture}}

\newcommand{\dotsntdst}{\begin{picture}(0,1)
   \put(4,0){\punto}
   \put(4,0){\vector(-1,0){4}}
   \put(4,0){\vector(1,0){4}}
\end{picture}}

%%%%%%% vi

\newcommand{\dotdstsntvi}{\begin{picture}(0,1)
   \put(3,0){\punto}
   \put(0,0){\vector(1,0){3}}
   \put(6,0){\vector(-1,0){3}}
\end{picture}}

\newcommand{\dotdstdstvi}{\begin{picture}(0,1)
   \put(3,0){\punto}
   \put(0,0){\vector(1,0){3}}
   \put(3,0){\vector(1,0){3}}
\end{picture}}

\newcommand{\dotsntsntvi}{\begin{picture}(0,1)
   \put(3,0){\punto}
   \put(3,0){\vector(-1,0){3}}
   \put(6,0){\vector(-1,0){3}}
\end{picture}}

\newcommand{\dotsntdstvi}{\begin{picture}(0,1)
   \put(3,0){\punto}
   \put(3,0){\vector(-1,0){3}}
   \put(3,0){\vector(1,0){3}}
\end{picture}}

%%%%%%% iv

\newcommand{\dotdstsntiv}{\begin{picture}(0,1)
   \put(2,0){\punto}
   \put(0,0){\vector(1,0){2}}
   \put(4,0){\vector(-1,0){2}}
\end{picture}}

\newcommand{\dotdstdstiv}{\begin{picture}(0,1)
   \put(2,0){\punto}
   \put(0,0){\vector(1,0){2}}
   \put(2,0){\vector(1,0){2}}
\end{picture}}

\newcommand{\dotsntsntiv}{\begin{picture}(0,1)
   \put(2,0){\punto}
   \put(2,0){\vector(-1,0){2}}
   \put(4,0){\vector(-1,0){2}}
\end{picture}}

\newcommand{\dotsntdstiv}{\begin{picture}(0,1)
   \put(2,0){\punto}
   \put(2,0){\vector(-1,0){2}}
   \put(2,0){\vector(1,0){2}}
\end{picture}}



\newcommand{\midgiuaddbase}[2]{\begin{picture}(0,1)
   \put( 0,0.5){#1}
   \put( 0.25,1.5){\makebox(0,0)[lb]{$#2$}}
\end{picture}}

\newcommand{\midsuaddbase}[2]{\begin{picture}(0,1)
   \put( 0,-0.5){#1}
   \put( 0.25,8.5){\makebox(0,0)[lt]{$#2$}}
\end{picture}}

\newcommand{\midgiuaddbasetop}[2]{\begin{picture}(0,1)
   \put( 0,0.5){#1}
   \put( 0.25,0.75){\makebox(0,0)[lb]{$#2$}}
\end{picture}}

\newcommand{\midsuaddbasetop}[2]{\begin{picture}(0,1)
   \put( 0,-0.5){#1}
   \put( 0.25,9.25){\makebox(0,0)[lt]{$#2$}}
\end{picture}}

\newcommand{\midgiu}[2]{\begin{picture}(0,1)
   \put(-2,3){\framebox(4,4){$#1$}}
   \put(0,3){\vector(0,-1){3}}
   \put(0,9.5){\vector(0,-1){2.5}}
   \put(0,-0.5){\makebox(0,0)[t]{$#2$}}
\end{picture}}

%\newcommand{\midgiuadd}[2]{\midgiuaddbase{\midgiu{#1}{}}{#2}}

\newcommand{\midsu}[2]{\begin{picture}(0,1)
   \put(-2,3){\framebox(4,4){$#1$}}
   \put(0,7){\vector(0,1){3}}
   \put(0,0.5){\vector(0,1){2.5}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}

\newcommand{\midsuadd}[2]{\midsuaddbase{\midsu{#1}{}}{#2}}

\newcommand{\midgiularge}[2]{\begin{picture}(0,1)
   \put(-3,3){\framebox(6,4){$#1$}}
   \put(0,3){\vector(0,-1){3}}
   \put(0,9.5){\vector(0,-1){2.5}}
   \put(0,-0.5){\makebox(0,0)[t]{$#2$}}
\end{picture}}

\newcommand{\midgiulargeadd}[2]{\midgiuaddbase{\midgiularge{#1}{}}{#2}}

\newcommand{\midsularge}[2]{\begin{picture}(0,1)
   \put(-3,3){\framebox(6,4){$#1$}}
   \put(0,7){\vector(0,1){3}}
   \put(0,0.5){\vector(0,1){2.5}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}

\newcommand{\midsulargeadd}[2]{\midsuaddbase{\midsularge{#1}{}}{#2}}

\newcommand{\midgiubig}[2]{\begin{picture}(0,1)
   \put( 0, 9.5){\vector(0,-1){1.5}}
   \put(-3,   2){\framebox(6,6){$#1$}}
   \put( 0,   2){\vector(0,-1){2}}
   \put( 0,-0.5){\makebox(0,0)[t]{$#2$}}
\end{picture}}

\newcommand{\midgiubigadd}[2]{\midgiuaddbase{\midgiubig{#1}{}}{#2}}

\newcommand{\midsubig}[2]{\begin{picture}(0,1)
   \put(0,0.5){\vector(0,1){1.5}}
   \put(-3,2){\framebox(6,6){$#1$}}
   \put(0,8){\vector(0,1){2}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}

\newcommand{\midsubigadd}[2]{\midsuaddbase{\midsubig{#1}{}}{#2}}

\newcommand{\midgiuvi}[2]{\begin{picture}(0,1)
   \put(   0, 9.5){\vector(0,-1){3}}
   \put(-1.5, 3.5){\framebox(3,3){$#1$}}
   \put(   0, 3.5){\vector(0,-1){3.5}}
   \put(   0,-0.5){\makebox(0,0)[t]{$#2$}}
\end{picture}}

\newcommand{\midgiuviadd}[2]{\midgiuaddbase{\midgiuvi{#1}{}}{#2}}

\newcommand{\midsuvi}[2]{\begin{picture}(0,1)
   \put(   0, 0.5){\vector(0,1){3}}
   \put(-1.5, 3.5){\framebox(3,3){$#1$}}
   \put(   0, 6.5){\vector(0,1){3.5}}
   \put(   0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}

\newcommand{\midsuviadd}[2]{\midsuaddbase{\midsuvi{#1}{}}{#2}}

%%%% integratore 1/s

\newcommand{\midgiumint}[2]{\begin{picture}(0,1)
   \put(-2,4.5){\framebox(4,4){$#1$}}
   \put(-1.25,1){\framebox(2.5,2.5){{\bf $\frac{1}{s}$}}}
   \put(0,1){\vector(0,-1){1}}
   \put(0,4.5){\vector(0,-1){1}}
   \put(0,9.5){\vector(0,-1){1}}
   \put(0,-0.5){\makebox(0,0)[t]{$#2$}}
\end{picture}}

\newcommand{\midgiumintlarge}[2]{\begin{picture}(0,1)
   \put(-3,4.5){\framebox(6,4){$#1$}}
   \put(-1.25,1){\framebox(2.5,2.5){{\bf $\frac{1}{s}$}}}
   \put(0,1){\vector(0,-1){1}}
   \put(0,4.5){\vector(0,-1){1}}
   \put(0,9.5){\vector(0,-1){1}}
   \put(0,-0.5){\makebox(0,0)[t]{$#2$}}
\end{picture}}

\newcommand{\midgiumintadd}[2]{\midgiuaddbasetop{\midgiumint{#1}{}}{#2}}
\newcommand{\midgiumintaddlarge}[2]{\midgiuaddbasetop{\midgiumintlarge{#1}{}}{#2}}

\newcommand{\midsuintm}[2]{\begin{picture}(0,1)
   \put(    0,0.5){\vector(0,1){1}}
   \put(-1.25,1.5){\framebox(2.5,2.5){{\bf $\frac{1}{s}$}}}
   \put(    0,  4){\vector(0,1){1}}
   \put(   -2,  5){\framebox(4,4){$#1$}}
   \put(    0,  9){\vector(0,1){1}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}

\newcommand{\midsuintmlarge}[2]{\begin{picture}(0,1)
   \put(    0,0.5){\vector(0,1){1}}
   \put(-1.25,1.5){\framebox(2.5,2.5){{\bf $\frac{1}{s}$}}}
   \put(    0,  4){\vector(0,1){1}}
   \put(   -3,  5){\framebox(6,4){$#1$}}
   \put(    0,  9){\vector(0,1){1}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}

\newcommand{\midsuintmadd}[2]{\midsuaddbasetop{\midsuintm{#1}{}}{#2}}
\newcommand{\midsuintmaddlarge}[2]{\midsuaddbasetop{\midsuintmlarge{#1}{}}{#2}}

%%%% derivatore s

\newcommand{\midgiumder}[2]{\begin{picture}(0,1)
   \put(-2,4.5){\framebox(4,4){$#1$}}
   \put(-1.25,1){\framebox(2.5,2.5){{\bf $s$}}}
   \put(0,1){\vector(0,-1){1}}
   \put(0,4.5){\vector(0,-1){1}}
   \put(0,9.5){\vector(0,-1){1}}
   \put(0,-0.5){\makebox(0,0)[t]{$#2$}}
\end{picture}}

\newcommand{\midgiumderlarge}[2]{\begin{picture}(0,1)
   \put(-3,4.5){\framebox(6,4){$#1$}}
   \put(-1.25,1){\framebox(2.5,2.5){{\bf $s$}}}
   \put(0,1){\vector(0,-1){1}}
   \put(0,4.5){\vector(0,-1){1}}
   \put(0,9.5){\vector(0,-1){1}}
   \put(0,-0.5){\makebox(0,0)[t]{$#2$}}
\end{picture}}

\newcommand{\midgiumderadd}[2]{\midgiuaddbasetop{\midgiumder{#1}{}}{#2}}
\newcommand{\midgiumderaddlarge}[2]{\midgiuaddbasetop{\midgiumderlarge{#1}{}}{#2}}

\newcommand{\midsuderm}[2]{\begin{picture}(0,1)
   \put(    0,0.5){\vector(0,1){1}}
   \put(-1.25,1.5){\framebox(2.5,2.5){{\bf $s$}}}
   \put(    0,  4){\vector(0,1){1}}
   \put(   -2,  5){\framebox(4,4){$#1$}}
   \put(    0,  9){\vector(0,1){1}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}

\newcommand{\midsudermlarge}[2]{\begin{picture}(0,1)
   \put(    0,0.5){\vector(0,1){1}}
   \put(-1.25,1.5){\framebox(2.5,2.5){{\bf $s$}}}
   \put(    0,  4){\vector(0,1){1}}
   \put(   -3,  5){\framebox(6,4){$#1$}}
   \put(    0,  9){\vector(0,1){1}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}

\newcommand{\midsudermadd}[2]{\midsuaddbasetop{\midsuderm{#1}{}}{#2}}
\newcommand{\midsudermaddlarge}[2]{\midsuaddbasetop{\midsudermlarge{#1}{}}{#2}}

%%%

\newcommand{\midgiumxm}[4]{\begin{picture}(0,1)
   \put(    0,9.5){\vector(0,-1){1}}
   \put(-1.25,6.0){\framebox(2.5,2.5){{\bf $#3$}}}
   \put(    0,  6){\vector(0,-1){1}}
   \put(  0.5,5.5){\makebox(0,0)[l]{$#4$}}
   \put(   -2,  1){\framebox(4,4){$#1$}}
   \put(    0,  1){\vector(0,-1){1}}
   \put(0,-0.5){\makebox(0,0)[t]{$#2$}}
\end{picture}}

\newcommand{\midgiumxmlarge}[4]{\begin{picture}(0,1)
   \put(    0,9.5){\vector(0,-1){1}}
   \put(-1.25,6.0){\framebox(2.5,2.5){{\bf $#3$}}}
   \put(    0,  6){\vector(0,-1){1}}
   \put(  0.5,5.5){\makebox(0,0)[l]{$#4$}}
   \put(   -3,  1){\framebox(6,4){$#1$}}
   \put(    0,  1){\vector(0,-1){1}}
   \put(0,-0.5){\makebox(0,0)[t]{$#2$}}
\end{picture}}

\newcommand{\midgiumxmadd}[4]{\midgiuaddbasetop{\midgiumxm{#1}{}{#3}{#4}}{#2}}
\newcommand{\midgiumxmaddlarge}[4]{\midgiuaddbasetop{\midgiumxmlarge{#1}{}{#3}{#4}}{#2}}

\newcommand{\midgiuivxxx}[4]{\begin{picture}(0,1)
   \put(    0,9.5){\vector(0,-1){1.0}}
   \put(-1.5,6.5){\framebox(3.0,2.0){{\bf $#1$}}}
   \put(    0,6.5){\vector(0,-1){1.0}}
   \put(-1.25,4.0){\framebox(2.5,1.5){{\bf $#2$}}}
   \put(    0,4.0){\vector(0,-1){1.0}}
   \put(-1.5,1.0){\framebox(3.0,2.0){{\bf $#3$}}}
   \put(    0,1.0){\vector(0,-1){1.0}}
   \put(0,-0.5){\makebox(0,0)[t]{$#4$}}
\end{picture}}

\newcommand{\midgiuivxxxadd}[4]{\midgiuaddbasetop{\midgiuivxxx{#1}{#2}{#3}{}}{#4}}

\newcommand{\midgiuxxx}[4]{\begin{picture}(0,1)
   \put(    0,9.5){\vector(0,-1){1.0}}
   \put(-2.5,6.5){\framebox(5.0,2.0){{\bf $#1$}}}
   \put(    0,6.5){\vector(0,-1){1.0}}
   \put(-1.5,4.0){\framebox(3.0,1.5){{\bf $#2$}}}
   \put(    0,4.0){\vector(0,-1){1.0}}
   \put(-2.5,1.0){\framebox(5.0,2.0){{\bf $#3$}}}
   \put(    0,1.0){\vector(0,-1){1.0}}
   \put(0,-0.5){\makebox(0,0)[t]{$#4$}}
\end{picture}}

\newcommand{\midgiuxxxadd}[4]{\midgiuaddbasetop{\midgiuxxx{#1}{#2}{#3}{}}{#4}}

\newcommand{\midgiuxxxlarge}[4]{\begin{picture}(0,1)
   \put(    0,9.5){\vector(0,-1){1.0}}
   \put(-3.5,6.5){\framebox(7.0,2.0){{\bf $#1$}}}
   \put(    0,6.5){\vector(0,-1){1.0}}
   \put(-1.5,4.0){\framebox(3.0,1.5){{\bf $#2$}}}
   \put(    0,4.0){\vector(0,-1){1.0}}
   \put(-3.5,1.0){\framebox(7.0,2.0){{\bf $#3$}}}
   \put(    0,1.0){\vector(0,-1){1.0}}
   \put(0,-0.5){\makebox(0,0)[t]{$#4$}}
\end{picture}}

\newcommand{\midgiuxxxlargeadd}[4]{\midgiuaddbasetop{\midgiuxxxlarge{#1}{#2}{#3}{}}{#4}}

\newcommand{\midsuivxxx}[4]{\begin{picture}(0,1)
   \put(    0,0.5){\vector(0,1){1.0}}
   \put(-1.5,7.0){\framebox(3.0,2.0){{\bf $#3$}}}
   \put(    0,3.5){\vector(0,1){1.0}}
   \put(-1.25,4.5){\framebox(2.5,1.5){{\bf $#2$}}}
   \put(    0,6.0){\vector(0,1){1.0}}
   \put(-1.5,1.5){\framebox(3.0,2.0){{\bf $#1$}}}
   \put(    0,9.0){\vector(0,1){1.0}}
   \put(0,10.5){\makebox(0,0)[b]{$#4$}}
\end{picture}}

\newcommand{\midsuivxxxadd}[4]{\midsuaddbasetop{\midsuivxxx{#1}{#2}{#3}{}}{#4}}

\newcommand{\midsuxxx}[4]{\begin{picture}(0,1)
   \put(    0,0.5){\vector(0,1){1.0}}
   \put(-2.5,7.0){\framebox(5.0,2.0){{\bf $#3$}}}
   \put(    0,3.5){\vector(0,1){1.0}}
   \put(-1.5,4.5){\framebox(3.0,1.5){{\bf $#2$}}}
   \put(    0,6.0){\vector(0,1){1.0}}
   \put(-2.5,1.5){\framebox(5.0,2.0){{\bf $#1$}}}
   \put(    0,9.0){\vector(0,1){1.0}}
   \put(0,10.5){\makebox(0,0)[b]{$#4$}}
\end{picture}}

\newcommand{\midsuxxxadd}[4]{\midsuaddbasetop{\midsuxxx{#1}{#2}{#3}{}}{#4}}

\newcommand{\midsuxxxlarge}[4]{\begin{picture}(0,1)
   \put(    0,0.5){\vector(0,1){1.0}}
   \put(-3.5,7.0){\framebox(7.0,2.0){{\bf $#3$}}}
   \put(    0,3.5){\vector(0,1){1.0}}
   \put(-1.5,4.5){\framebox(3.0,1.5){{\bf $#2$}}}
   \put(    0,6.0){\vector(0,1){1.0}}
   \put(-3.5,1.5){\framebox(7.0,2.0){{\bf $#1$}}}
   \put(    0,9.0){\vector(0,1){1.0}}
   \put(0,10.5){\makebox(0,0)[b]{$#4$}}
\end{picture}}

\newcommand{\midsuxxxlargeadd}[4]{\midsuaddbasetop{\midsuxxxlarge{#1}{#2}{#3}{}}{#4}}

\newcommand{\midgiuivmxm}[4]{\begin{picture}(0,1)
   \put(    0,9.5){\vector(0,-1){1.5}}
   \put(-1.25,5.5){\framebox(2.5,2.5){{\bf $#3$}}}
   \put(    0,5.5){\vector(0,-1){1.5}}
   \put(  0.5,4.75){\makebox(0,0)[l]{$#4$}}
   \put(-1.25,1.5){\framebox(2.5,2.5){$#1$}}
   \put(    0,1.5){\vector(0,-1){1.5}}
   \put(0,-0.5){\makebox(0,0)[t]{$#2$}}
\end{picture}}

\newcommand{\midgiuivmxmadd}[4]{\midgiuaddbasetop{\midgiuivmxm{#1}{}{#3}{#4}}{#2}}

\newcommand{\midsumxm}[4]{\begin{picture}(0,1)
   \put(    0,0.5){\vector(0,1){1}}
   \put(-1.25,1.5){\framebox(2.5,2.5){{\bf $#3$}}}
   \put(    0,  4){\vector(0,1){1}}
   \put(  0.5,4.5){\makebox(0,0)[l]{$#4$}}
   \put(   -2,  5){\framebox(4,4){$#1$}}
   \put(    0,  9){\vector(0,1){1}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}

\newcommand{\midsumxmlarge}[4]{\begin{picture}(0,1)
   \put(    0,0.5){\vector(0,1){1}}
   \put(-1.25,1.5){\framebox(2.5,2.5){{\bf $#3$}}}
   \put(    0,  4){\vector(0,1){1}}
   \put(  0.5,4.5){\makebox(0,0)[l]{$#4$}}
   \put(   -3,  5){\framebox(6,4){$#1$}}
   \put(    0,  9){\vector(0,1){1}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}

\newcommand{\midsumxmadd}[4]{\midsuaddbasetop{\midsumxm{#1}{}{#3}{#4}}{#2}}
\newcommand{\midsumxmaddlarge}[4]{\midsuaddbasetop{\midsumxmlarge{#1}{}{#3}{#4}}{#2}}

\newcommand{\midsuivmxm}[4]{\begin{picture}(0,1)
   \put(    0,0.5){\vector(0,1){1.5}}
   \put(-1.25,  2){\framebox(2.5,2.5){{\bf $#3$}}}
   \put(    0,4.5){\vector(0,1){1.5}}
   \put(  0.5,5.25){\makebox(0,0)[l]{$#4$}}
   \put(-1.25,  6){\framebox(2.5,2.5){$#1$}}
   \put(    0,8.5){\vector(0,1){1.5}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}

\newcommand{\midsuivmxmadd}[4]{\midsuaddbasetop{\midsuivmxm{#1}{}{#3}{#4}}{#2}}

%%% integratore 1/s

\newcommand{\midgiuintm}[2]{\begin{picture}(0,1)
   \put(    0,9.5){\vector(0,-1){1}}
   \put(-1.25,  6){\framebox(2.5,2.5){{\bf $\frac{1}{s}$}}}
   \put(    0,  6){\vector(0,-1){1}}
   \put(   -2,  1){\framebox(4,4){$#1$}}
   \put(    0,  1){\vector(0,-1){1}}
   \put(0,-0.5  ){\makebox(0,0)[t]{$#2$}}
\end{picture}}

\newcommand{\midgiuintmlarge}[2]{\begin{picture}(0,1)
   \put(    0,9.5){\vector(0,-1){1}}
   \put(-1.25,  6){\framebox(2.5,2.5){{\bf $\frac{1}{s}$}}}
   \put(    0,  6){\vector(0,-1){1}}
   \put(   -3,  1){\framebox(6,4){$#1$}}
   \put(    0,  1){\vector(0,-1){1}}
   \put(0,-0.5  ){\makebox(0,0)[t]{$#2$}}
\end{picture}}

\newcommand{\midgiuintmadd}[2]{\midgiuaddbasetop{\midgiuintm{#1}{}}{#2}}
\newcommand{\midgiuintmaddlarge}[2]{\midgiuaddbasetop{\midgiuintmlarge{#1}{}}{#2}}

\newcommand{\midsumint}[2]{\begin{picture}(0,1)
   \put(-2,1.5){\framebox(4,4){$#1$}}
   \put(-1.25,6.5){\framebox(2.5,2.5){{\bf $\frac{1}{s}$}}}
   \put(0,0.5){\vector(0,1){1}}
   \put(0,5.5){\vector(0,1){1}}
   \put(0,9){\vector(0,1){1}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}

\newcommand{\midsumintlarge}[2]{\begin{picture}(0,1)
   \put(-3,1.5){\framebox(6,4){$#1$}}
   \put(-1.25,6.5){\framebox(2.5,2.5){{\bf $\frac{1}{s}$}}}
   \put(0,0.5){\vector(0,1){1}}
   \put(0,5.5){\vector(0,1){1}}
   \put(0,9){\vector(0,1){1}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}

\newcommand{\midsumintadd}[2]{\midsuaddbasetop{\midsumint{#1}{}}{#2}}
\newcommand{\midsumintaddlarge}[2]{\midsuaddbasetop{\midsumintlarge{#1}{}}{#2}}

%%% derivatore s

\newcommand{\midgiuderm}[2]{\begin{picture}(0,1)
   \put(    0,9.5){\vector(0,-1){1}}
   \put(-1.25,  6){\framebox(2.5,2.5){{\bf $s$}}}
   \put(    0,  6){\vector(0,-1){1}}
   \put(   -2,  1){\framebox(4,4){$#1$}}
   \put(    0,  1){\vector(0,-1){1}}
   \put(0,-0.5  ){\makebox(0,0)[t]{$#2$}}
\end{picture}}

\newcommand{\midgiudermlarge}[2]{\begin{picture}(0,1)
   \put(    0,9.5){\vector(0,-1){1}}
   \put(-1.25,  6){\framebox(2.5,2.5){{\bf $s$}}}
   \put(    0,  6){\vector(0,-1){1}}
   \put(   -3,  1){\framebox(6,4){$#1$}}
   \put(    0,  1){\vector(0,-1){1}}
   \put(0,-0.5  ){\makebox(0,0)[t]{$#2$}}
\end{picture}}

\newcommand{\midgiudermadd}[2]{\midgiuaddbasetop{\midgiuderm{#1}{}}{#2}}
\newcommand{\midgiudermaddlarge}[2]{\midgiuaddbasetop{\midgiudermlarge{#1}{}}{#2}}

\newcommand{\midsumder}[2]{\begin{picture}(0,1)
   \put(-2,1.5){\framebox(4,4){$#1$}}
   \put(-1.25,6.5){\framebox(2.5,2.5){{\bf $s$}}}
   \put(0,0.5){\vector(0,1){1}}
   \put(0,5.5){\vector(0,1){1}}
   \put(0,9){\vector(0,1){1}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}

\newcommand{\midsumderlarge}[2]{\begin{picture}(0,1)
   \put(-3,1.5){\framebox(6,4){$#1$}}
   \put(-1.25,6.5){\framebox(2.5,2.5){{\bf $s$}}}
   \put(0,0.5){\vector(0,1){1}}
   \put(0,5.5){\vector(0,1){1}}
   \put(0,9){\vector(0,1){1}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}

\newcommand{\midsumderadd}[2]{\midsuaddbasetop{\midsumder{#1}{}}{#2}}
\newcommand{\midsumderaddlarge}[2]{\midsuaddbasetop{\midsumderlarge{#1}{}}{#2}}

%%%%


\newcommand{\midgiuiv}[2]{\begin{picture}(0,1)
   \put(-1.5,3.5){\framebox(3,3){$#1$}}
   \put(0,9.5){\vector(0,-1){3}}
   \put(0,3.5){\vector(0,-1){3.5}}
   \put(0,-0.5){\makebox(0,0)[t]{$#2$}}
\end{picture}}

\newcommand{\midgiuivadd}[2]{\midgiuaddbase{\midgiuiv{#1}{}}{#2}}

\newcommand{\midsuiv}[2]{\begin{picture}(0,1)
   \put(-1.5,3.5){\framebox(3,3){$#1$}}
   \put(0,6.5){\vector(0,1){3.5}}
   \put(0,0.5){\vector(0,1){3}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}

\newcommand{\midsuivadd}[2]{\midsuaddbase{\midsuiv{#1}{}}{#2}}

%%%% integratore 1/s

\newcommand{\midgiuintmtre}[2]{\begin{picture}(0,1)
   \put(    0,9.5){\vector(0,-1){1.5}}
   \put(-1.25,5.5){\framebox(2.5,2.5){{\bf $\frac{1}{s}$}}}
   \put(    0,5.5){\vector(0,-1){1.5}}
   \put(-1.25,1.5){\framebox(2.5,2.5){$#1$}}
   \put(    0,1.5){\vector(0,-1){1.5}}
   \put(0,-0.5  ){\makebox(0,0)[t]{$#2$}}
\end{picture}}

\newcommand{\midgiuintmtreadd}[2]{\midgiuaddbasetop{\midgiuintmtre{#1}{}}{#2}}

\newcommand{\midsuintmtre}[2]{\begin{picture}(0,1)
   \put(    0,0.5){\vector(0,1){1.5}}
   \put(-1.25,2){\framebox(2.5,2.5){{\bf $\frac{1}{s}$}}}
   \put(    0,4.5){\vector(0,1){1.5}}
   \put(-1.25,  6){\framebox(2.5,2.5){$#1$}}
   \put(    0,8.5){\vector(0,1){1.5}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}

\newcommand{\midsuintmtreadd}[2]{\midsuaddbasetop{\midsuintmtre{#1}{}}{#2}}

\newcommand{\midgiuminttre}[2]{\begin{picture}(0,1)
   \put(    0,9.5){\vector(0,-1){1.5}}
   \put(-1.25,5.5){\framebox(2.5,2.5){$#1$}}
   \put(    0,5.5){\vector(0,-1){1.5}}
   \put(-1.25,1.5){\framebox(2.5,2.5){{\bf $\frac{1}{s}$}}}
   \put(    0,1.5){\vector(0,-1){1.5}}
   \put(0,-0.5  ){\makebox(0,0)[t]{$#2$}}
\end{picture}}

\newcommand{\midgiuminttreadd}[2]{\midgiuaddbasetop{\midgiuminttre{#1}{}}{#2}}

\newcommand{\midsuminttre}[2]{\begin{picture}(0,1)
   \put(0,0.5){\vector(0,1){1.5}}
   \put(-1.25,   2){\framebox(2.5,2.5){{$#1$}}}
   \put(    0, 4.5){\vector(0,1){1.5}}
   \put(-1.25,   6){\framebox(2.5,2.5){{\bf $\frac{1}{s}$}}}
   \put(    0, 8.5){\vector(0,1){1.5}}
   \put(    0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}

\newcommand{\midsuminttreadd}[2]{\midsuaddbasetop{\midsuminttre{#1}{}}{#2}}


%%%% derivatore s

\newcommand{\midgiudermtre}[2]{\begin{picture}(0,1)
   \put(    0,9.5){\vector(0,-1){1.5}}
   \put(-1.25,5.5){\framebox(2.5,2.5){{\bf $s$}}}
   \put(    0,5.5){\vector(0,-1){1.5}}
   \put(-1.25,1.5){\framebox(2.5,2.5){$#1$}}
   \put(    0,1.5){\vector(0,-1){1.5}}
   \put(0,-0.5  ){\makebox(0,0)[t]{$#2$}}
\end{picture}}

\newcommand{\midgiudermtreadd}[2]{\midgiuaddbasetop{\midgiudermtre{#1}{}}{#2}}

\newcommand{\midsudermtre}[2]{\begin{picture}(0,1)
   \put(    0,0.5){\vector(0,1){1.5}}
   \put(-1.25,2){\framebox(2.5,2.5){{\bf $s$}}}
   \put(    0,4.5){\vector(0,1){1.5}}
   \put(-1.25,  6){\framebox(2.5,2.5){$#1$}}
   \put(    0,8.5){\vector(0,1){1.5}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}

\newcommand{\midsudermtreadd}[2]{\midsuaddbasetop{\midsudermtre{#1}{}}{#2}}

\newcommand{\midgiumdertre}[2]{\begin{picture}(0,1)
   \put(    0,9.5){\vector(0,-1){1.5}}
   \put(-1.25,5.5){\framebox(2.5,2.5){$#1$}}
   \put(    0,5.5){\vector(0,-1){1.5}}
   \put(-1.25,1.5){\framebox(2.5,2.5){{\bf $s$}}}
   \put(    0,1.5){\vector(0,-1){1.5}}
   \put(0,-0.5  ){\makebox(0,0)[t]{$#2$}}
\end{picture}}

\newcommand{\midgiumdertreadd}[2]{\midgiuaddbasetop{\midgiumdertre{#1}{}}{#2}}

\newcommand{\midsumdertre}[2]{\begin{picture}(0,1)
   \put(0,0.5){\vector(0,1){1.5}}
   \put(-1.25,   2){\framebox(2.5,2.5){{$#1$}}}
   \put(    0, 4.5){\vector(0,1){1.5}}
   \put(-1.25,   6){\framebox(2.5,2.5){{\bf $s$}}}
   \put(    0, 8.5){\vector(0,1){1.5}}
   \put(    0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}

\newcommand{\midsumdertreadd}[2]{\midsuaddbasetop{\midsumdertre{#1}{}}{#2}}

%%%%%

\newcommand{\midsupiu}[4]{\begin{picture}(0,1)
   \put(-2,2.5){\framebox(4,4){$#1$}}
   \put(0,6.5){\vector(0,1){1.5}}
   \put(0,8.5){\piu}
   \put(0,9){\vector(0,1){1}}
   \put(1.5,8.5){\vector(-1,0){1}}
   \put(1.5,8.5){\punto}
   \put(0,0.5){\vector(0,1){2}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
   \put(0,8.5){\makebox(0,0){$#4$}}
   \put(1.75,8.5){\makebox(0,0)[l]{$#3$}}
\end{picture}}

\newcommand{\midsupiutre}[4]{\begin{picture}(0,1)
   \put(-1.5,2.5){\framebox(3,3){$#1$}}
   \put(0,5.5){\vector(0,1){2}}
   \put(0,8){\piu}
   \put(0,8.5){\vector(0,1){1.5}}
   \put(1.5,8){\vector(-1,0){1}}
   \put(1.5,8){\punto}
   \put(0,0.5){\vector(0,1){2}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
   \put(0,8){\makebox(0,0){$#4$}}
   \put(1.75,7.75){\makebox(0,0)[tr]{$#3$}}
\end{picture}}


\newcommand{\midgiuintmvuoto}[2]{\begin{picture}(0,1)
   \put(    0,9.5){\vector(0,-1){1}}
   \put(    0,8  ){\makebox(0,0)[t]{$#1$}}
   \put(    0,1.5){\makebox(0,0)[b]{$#2$}}
   \put(    0,  1){\punto}
   \put(    0,  1){\vector(0,-1){1}}
\end{picture}}

\newcommand{\midsuintmvuoto}[2]{\begin{picture}(0,1)
   \put(    0,0.5){\vector(0,1){1}}
   \put(    0,  2 ){\makebox(0,0)[b]{$#1$}}
   \put(    0,8.5 ){\makebox(0,0)[t]{$#2$}}
   \put(    0,  9){\punto}
   \put(    0,  9){\vector(0,1){1}}
\end{picture}}

%%%%%%  Blocchi Base

%%%%%% su

\newcommand{\blosubase}[2]{\begin{picture}(8,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\dotsntdst}
   \put(4, 0){#1}
   \put(0, 0){\sumdstsnt{#2}}
\end{picture}}

\newcommand{\blovisubase}[2]{\begin{picture}(6,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\dotsntdstvi}
   \put(3, 0){#1}
   \put(0, 0){\sumdstsntvi{#2}}
\end{picture}}

\newcommand{\bloivsubase}[2]{\begin{picture}(4,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\dotsntdstiv}
   \put(2, 0){#1}
   \put(0, 0){\sumdstsntiv{#2}}
\end{picture}}

%%%%%% su or

\newcommand{\blosuorbase}[2]{\begin{picture}(8,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\sumdstdst{#2}}
   \put(4, 0){#1}
   \put(0, 0){\dotsntsnt}
\end{picture}}

\newcommand{\blovisuorbase}[2]{\begin{picture}(6,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\sumdstdstvi{#2}}
   \put(3, 0){#1}
   \put(0, 0){\dotsntsntvi}
\end{picture}}

\newcommand{\bloivsuorbase}[2]{\begin{picture}(4,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\sumdstdstiv{#2}}
   \put(2, 0){#1}
   \put(0, 0){\dotsntsntiv}
\end{picture}}

%%%%%% su aor

\newcommand{\blosuaorbase}[2]{\begin{picture}(8,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\sumsntsnt{#2}}
   \put(4, 0){#1}
   \put(0, 0){\dotdstdst}
\end{picture}}

\newcommand{\blovisuaorbase}[2]{\begin{picture}(6,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\sumsntsntvi{#2}}
   \put(3, 0){#1}
   \put(0, 0){\dotdstdstvi}
\end{picture}}

\newcommand{\bloivsuaorbase}[2]{\begin{picture}(4,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\sumsntsntiv{#2}}
   \put(2, 0){#1}
   \put(0, 0){\dotdstdstiv}
\end{picture}}


%%%%%% su dst

\newcommand{\blosudstbase}[2]{\begin{picture}(8,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\sumdstdst{#2}}
   \put(4, 0){#1}
   \put(0, 0){\dotdstdst}
\end{picture}}

\newcommand{\bloivsudstbase}[2]{\begin{picture}(4,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\sumdstdstiv{#2}}
   \put(2, 0){#1}
   \put(0, 0){\dotdstdstiv}
\end{picture}}

\newcommand{\blovisudstbase}[2]{\begin{picture}(6,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\sumdstdstvi{#2}}
   \put(3, 0){#1}
   \put(0, 0){\dotdstdstvi}
\end{picture}}


%%%%%% su snt

\newcommand{\blosusntbase}[2]{\begin{picture}(8,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\sumsntsnt{#2}}
   \put(4, 0){#1}
   \put(0, 0){\dotsntsnt}
\end{picture}}

\newcommand{\bloivsusntbase}[2]{\begin{picture}(4,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\sumsntsntiv{#2}}
   \put(2, 0){#1}
   \put(0, 0){\dotsntsntiv}
\end{picture}}

\newcommand{\blovisusntbase}[2]{\begin{picture}(6,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\sumsntsntvi{#2}}
   \put(3, 0){#1}
   \put(0, 0){\dotsntsntvi}
\end{picture}}


%%%%%% giu

\newcommand{\blogiubase}[2]{\begin{picture}(8,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\sumdstsnt{#2}}
   \put(4, 0){#1}
   \put(0, 0){\dotsntdst}
\end{picture}}

\newcommand{\blovigiubase}[2]{\begin{picture}(6,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\sumdstsntvi{#2}}
   \put(3, 0){#1}
   \put(0, 0){\dotsntdstvi}
\end{picture}}

\newcommand{\bloivgiubase}[2]{\begin{picture}(4,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\sumdstsntiv{#2}}
   \put(2, 0){#1}
   \put(0, 0){\dotsntdstiv}
\end{picture}}

%%%%%% giuor

\newcommand{\blogiuorbase}[2]{\begin{picture}(8,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\dotdstdst}
   \put(4, 0){#1}
   \put(0, 0){\sumsntsnt{#2}}
\end{picture}}

\newcommand{\blovigiuorbase}[2]{\begin{picture}(6,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\dotdstdstvi}
   \put(3, 0){#1}
   \put(0, 0){\sumsntsntvi{#2}}
\end{picture}}

\newcommand{\bloivgiuorbase}[2]{\begin{picture}(4,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\dotdstdstiv}
   \put(2, 0){#1}
   \put(0, 0){\sumsntsntiv{#2}}
\end{picture}}

%%%%%% giuaor

\newcommand{\blogiuaorbase}[2]{\begin{picture}(8,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\dotsntsnt}
   \put(4, 0){#1}
   \put(0, 0){\sumdstdst{#2}}
\end{picture}}

\newcommand{\blovigiuaorbase}[2]{\begin{picture}(6,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\dotsntsntvi}
   \put(3, 0){#1}
   \put(0, 0){\sumdstdstvi{#2}}
\end{picture}}

\newcommand{\bloivgiuaorbase}[2]{\begin{picture}(4,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\dotsntsntiv}
   \put(2, 0){#1}
   \put(0, 0){\sumdstdstiv{#2}}
\end{picture}}


%%%%%% giu dst

\newcommand{\blogiudstbase}[2]{\begin{picture}(8,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\dotdstdst}
   \put(4, 0){#1}
   \put(0, 0){\sumdstdst{#2}}
\end{picture}}

\newcommand{\bloivgiudstbase}[2]{\begin{picture}(4,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\dotdstdstiv}
   \put(2, 0){#1}
   \put(0, 0){\sumdstdstiv{#2}}
\end{picture}}

\newcommand{\blovigiudstbase}[2]{\begin{picture}(6,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\dotdstdstvi}
   \put(3, 0){#1}
   \put(0, 0){\sumdstdstvi{#2}}
\end{picture}}


%%%%%% giu snt

\newcommand{\blogiusntbase}[2]{\begin{picture}(8,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\dotsntsnt}
   \put(4, 0){#1}
   \put(0, 0){\sumsntsnt{#2}}
\end{picture}}

\newcommand{\bloivgiusntbase}[2]{\begin{picture}(4,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\dotsntsntiv}
   \put(2, 0){#1}
   \put(0, 0){\sumsntsntiv{#2}}
\end{picture}}

\newcommand{\blovigiusntbase}[2]{\begin{picture}(6,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\dotsntsntvi}
   \put(3, 0){#1}
   \put(0, 0){\sumsntsntvi{#2}}
\end{picture}}


% ************ Blocchi

\newcommand{\bloin}[2]{\begin{picture}(0,0)
 \put(-0.5,10){\makebox(0,0)[r]{$#1$}}
 \put(-0.5, 0){\makebox(0,0)[r]{$#2$}}
 \put(0, 0){\punto}
 \put(0,10){\punto}
 \end{picture}}

\newcommand{\bloout}[2]{\begin{picture}(0,10)
   \put(0.5,10){\makebox(0,0)[l]{$#1$}}
   \put(0.5, 0){\makebox(0,0)[l]{$#2$}}
   \put(0, 0){\punto}
   \put(0,10){\punto}
   \put(0,0){\tratteggio}
\end{picture}}


\newcommand{\bloivinsu}[3]{\begin{picture}(4,0)
 \put(0,0){\tratteggio}
 \put(0,0){\dotsntdstiv}
 \put(0,10){\sumdstsntiv{#3}}
 \put(2,-2){\punto}
 \put(2,10.5){\vector(0,1){1.5}}
 \put(2.25,12){\makebox(0,0)[l]{$#2$}}
 \put(2,-2){\vector(0,1){2}}
 \put(2.25,-2){\makebox(0,0)[l]{$#1$}}
 \end{picture}}

\newcommand{\bloivingiu}[3]{\begin{picture}(4,0)
 \put(0,0){\tratteggio}
 \put(0,0){\sumdstsntiv{#3}}
 \put(0,10){\dotsntdstiv}
% \put(2,10){\punto}
 \put(2,12){\punto}
 \put(2,-0.5){\vector(0,-1){1.5}}
 \put(2.25,-2){\makebox(0,0)[l]{$#2$}}
 \put(2,12){\vector(0,-1){2}}
 \put(2.25,12){\makebox(0,0)[l]{$#1$}}
 \end{picture}}

\newcommand{\bloivinsuor}[3]{\begin{picture}(4,0)
 \put(0,0){\tratteggio}
 \put(0,0){\sumsntsntiv{#3}}
 \put(0,10){\dotdstdstiv}
 \put(2,10){\punto}
 \put(2,-2){\punto}
 \put(2,-2){\vector(0,1){1.5}}
 \put(2.25,-2){\makebox(0,0)[l]{$#1$}}
 \put(2,10){\vector(0,1){2}}
 \put(2.25,12){\makebox(0,0)[l]{$#2$}}
 \end{picture}}

\newcommand{\bloivinsuaor}[3]{\begin{picture}(4,0)
 \put(0,0){\tratteggio}
 \put(0,0){\sumdstdstiv{#3}}
 \put(0,10){\dotsntsntiv}
 \put(2,10){\punto}
 \put(2,-2){\punto}
 \put(2,-2){\vector(0,1){1.5}}
 \put(2.25,-2){\makebox(0,0)[l]{$#1$}}
 \put(2,10){\vector(0,1){2}}
 \put(2.25,12){\makebox(0,0)[l]{$#2$}}
 \end{picture}}

\newcommand{\bloivingiuaor}[3]{\begin{picture}(4,0)
 \put(0,0){\tratteggio}
 \put(0,0){\dotdstdstiv}
 \put(0,10){\sumsntsntiv{#3}}
 \put(2,12){\punto}
 \put(2,12){\vector(0,-1){1.5}}
 \put(2.25,12){\makebox(0,0)[l]{$#1$}}
 \put(2,0){\vector(0,-1){2}}
 \put(2.25,-2){\makebox(0,0)[l]{$#2$}}
 \end{picture}}

\newcommand{\bloivingiuor}[3]{\begin{picture}(4,0)
 \put(0,0){\tratteggio}
 \put(0,0){\dotsntsntiv}
 \put(0,10){\sumdstdstiv{#3}}
 \put(2,12){\punto}
 \put(2,12){\vector(0,-1){1.5}}
 \put(2.25,12){\makebox(0,0)[l]{$#1$}}
 \put(2,0){\vector(0,-1){2}}
 \put(2.25,-2){\makebox(0,0)[l]{$#2$}}
 \end{picture}}



%%%%% su
\newcommand{\blosu}[3]{\blosubase{\midsu{#1}{#2}}{#3}}
\newcommand{\blovisu}[3]{\blovisubase{\midsu{#1}{#2}}{#3}}
\newcommand{\bloivsu}[3]{\bloivsubase{\midsuiv{#1}{#2}}{#3}}
%%%%% su or
\newcommand{\blosuor}[3]{\blosuorbase{\midsuadd{#1}{#2}}{#3}}
\newcommand{\blovisuor}[3]{\blovisuorbase{\midsuadd{#1}{#2}}{#3}}
\newcommand{\bloivsuor}[3]{\bloivsuorbase{\midsuivadd{#1}{#2}}{#3}}
%%%%% su aor
\newcommand{\blosuaor}[3]{\blosuaorbase{\midsuadd{#1}{#2}}{#3}}
\newcommand{\blovisuaor}[3]{\blovisuaorbase{\midsuadd{#1}{#2}}{#3}}
\newcommand{\bloivsuaor}[3]{\bloivsuaorbase{\midsuivadd{#1}{#2}}{#3}}
%%%%% su piu
\newcommand{\blosupiu}[5]{\blosubase{\midsupiu{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\blovisupiu}[5]{\blovisubase{\midsupiu{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\bloivsupiu}[5]{\bloivsubase{\midsupiutre{#1}{#2}{#4}{#5}}{#3}}
%%%%% su large
\newcommand{\blosularge}[3]{\blosubase{\midsularge{#1}{#2}}{#3}}
%%%%% su large or
\newcommand{\blosulargeor}[3]{\blosuorbase{\midsulargeadd{#1}{#2}}{#3}}
%%%%% su large aor
\newcommand{\blosulargeaor}[3]{\blosuaorbase{\midsulargeadd{#1}{#2}}{#3}}
%%%%% su big
\newcommand{\blosubig}[3]{\blosubase{\midsubig{#1}{#2}}{#3}}
%%%%% su big or
\newcommand{\blosubigor}[3]{\blosuorbase{\midsubigadd{#1}{#2}}{#3}}
%%%%% su big aor
\newcommand{\blosubigaor}[3]{\blosuaorbase{\midsubigadd{#1}{#2}}{#3}}
%%%%% su intm
\newcommand{\blosuintmlarge}[3]{\blosubase{\midsuintmlarge{#1}{#2}}{#3}}
\newcommand{\blosuintm}[3]{\blosubase{\midsuintm{#1}{#2}}{#3}}
\newcommand{\blovisuintm}[3]{\blovisubase{\midsuintm{#1}{#2}}{#3}}
\newcommand{\bloivsuintm}[3]{\bloivsubase{\midsuintmtre{#1}{#2}}{#3}}
%%%%% su intm or
\newcommand{\blosuintmorlarge}[3]{\blosuorbase{\midsuintmaddlarge{#1}{#2}}{#3}}
\newcommand{\blosuintmor}[3]{\blosuorbase{\midsuintmadd{#1}{#2}}{#3}}
\newcommand{\blovisuintmor}[3]{\blovisuorbase{\midsuintmadd{#1}{#2}}{#3}}
\newcommand{\bloivsuintmor}[3]{\bloivsuorbase{\midsuintmtreadd{#1}{#2}}{#3}}
%%%%% su intm aor
\newcommand{\blosuintmaorlarge}[3]{\blosuaorbase{\midsuintmaddlarge{#1}{#2}}{#3}}
\newcommand{\blosuintmaor}[3]{\blosuaorbase{\midsuintmadd{#1}{#2}}{#3}}
\newcommand{\blovisuintmaor}[3]{\blovisuaorbase{\midsuintmadd{#1}{#2}}{#3}}
\newcommand{\bloivsuintmaor}[3]{\bloivsuaorbase{\midsuintmtreadd{#1}{#2}}{#3}}
%%%%% su mint
\newcommand{\blosumintlarge}[3]{\blosubase{\midsumintlarge{#1}{#2}}{#3}}
\newcommand{\blosumint}[3]{\blosubase{\midsumint{#1}{#2}}{#3}}
\newcommand{\blovisumint}[3]{\blovisubase{\midsumint{#1}{#2}}{#3}}
\newcommand{\bloivsumint}[3]{\bloivsubase{\midsuminttre{#1}{#2}}{#3}}
%%%%% su mint or
\newcommand{\blosumintorlarge}[3]{\blosuorbase{\midsumintaddlarge{#1}{#2}}{#3}}
\newcommand{\blosumintor}[3]{\blosuorbase{\midsumintadd{#1}{#2}}{#3}}
\newcommand{\blovisumintor}[3]{\blovisuorbase{\midsumintadd{#1}{#2}}{#3}}
\newcommand{\bloivsumintor}[3]{\bloivsuorbase{\midsuminttreadd{#1}{#2}}{#3}}
%%%%% su mint aor
\newcommand{\blosumintaorlarge}[3]{\blosuaorbase{\midsumintaddlarge{#1}{#2}}{#3}}
\newcommand{\blosumintaor}[3]{\blosuaorbase{\midsumintadd{#1}{#2}}{#3}}
\newcommand{\blovisumintaor}[3]{\blovisuaorbase{\midsumintadd{#1}{#2}}{#3}}
\newcommand{\bloivsumintaor}[3]{\bloivsuaorbase{\midsuminttreadd{#1}{#2}}{#3}}
%%%%% su derm
\newcommand{\blosudermlarge}[3]{\blosubase{\midsudermlarge{#1}{#2}}{#3}}
\newcommand{\blosuderm}[3]{\blosubase{\midsuderm{#1}{#2}}{#3}}
\newcommand{\blovisuderm}[3]{\blovisubase{\midsuderm{#1}{#2}}{#3}}
\newcommand{\bloivsuderm}[3]{\bloivsubase{\midsudermtre{#1}{#2}}{#3}}
%%%%% su derm or
\newcommand{\blosudermorlarge}[3]{\blosuorbase{\midsudermaddlarge{#1}{#2}}{#3}}
\newcommand{\blosudermor}[3]{\blosuorbase{\midsudermadd{#1}{#2}}{#3}}
\newcommand{\blovisudermor}[3]{\blovisuorbase{\midsudermadd{#1}{#2}}{#3}}
\newcommand{\bloivsudermor}[3]{\bloivsuorbase{\midsudermtreadd{#1}{#2}}{#3}}
%%%%% su derm aor
\newcommand{\blosudermaorlarge}[3]{\blosuaorbase{\midsudermaddlarge{#1}{#2}}{#3}}
\newcommand{\blosudermaor}[3]{\blosuaorbase{\midsudermadd{#1}{#2}}{#3}}
\newcommand{\blovisudermaor}[3]{\blovisuaorbase{\midsudermadd{#1}{#2}}{#3}}
\newcommand{\bloivsudermaor}[3]{\bloivsuaorbase{\midsudermtreadd{#1}{#2}}{#3}}
%%%%% su mder
\newcommand{\blosumderlarge}[3]{\blosubase{\midsumderlarge{#1}{#2}}{#3}}
\newcommand{\blosumder}[3]{\blosubase{\midsumder{#1}{#2}}{#3}}
\newcommand{\blovisumder}[3]{\blovisubase{\midsumder{#1}{#2}}{#3}}
\newcommand{\bloivsumder}[3]{\bloivsubase{\midsumdertre{#1}{#2}}{#3}}
%%%%% su mder or
\newcommand{\blosumderorlarge}[3]{\blosuorbase{\midsumderaddlarge{#1}{#2}}{#3}}
\newcommand{\blosumderor}[3]{\blosuorbase{\midsumderadd{#1}{#2}}{#3}}
\newcommand{\blovisumderor}[3]{\blovisuorbase{\midsumderadd{#1}{#2}}{#3}}
\newcommand{\bloivsumderor}[3]{\bloivsuorbase{\midsumdertreadd{#1}{#2}}{#3}}
%%%%% su mder aor
\newcommand{\blosumderaorlarge}[3]{\blosuaorbase{\midsumderaddlarge{#1}{#2}}{#3}}
\newcommand{\blosumderaor}[3]{\blosuaorbase{\midsumderadd{#1}{#2}}{#3}}
\newcommand{\blovisumderaor}[3]{\blovisuaorbase{\midsumderadd{#1}{#2}}{#3}}
\newcommand{\bloivsumderaor}[3]{\bloivsuaorbase{\midsumdertreadd{#1}{#2}}{#3}}
%%%%% su mxm
\newcommand{\blosumxmlarge}[5]{\blosubase{\midsumxmlarge{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\blosumxm}[5]{\blosubase{\midsumxm{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\blovisumxm}[5]{\blovisubase{\midsumxm{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\bloivsumxm}[5]{\bloivsubase{\midsuivmxm{#1}{#2}{#4}{#5}}{#3}}
%%%%% su mxm or
\newcommand{\blosumxmorlarge}[5]{\blosuorbase{\midsumxmaddlarge{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\blosumxmor}[5]{\blosuorbase{\midsumxmadd{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\blovisumxmor}[5]{\blovisuorbase{\midsumxmadd{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\bloivsumxmor}[5]{\bloivsuorbase{\midsuivmxmadd{#1}{#2}{#4}{#5}}{#3}}
%%%%% su mxm aor
\newcommand{\blosumxmaorlarge}[5]{\blosuaorbase{\midsumxmaddlarge{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\blosumxmaor}[5]{\blosuaorbase{\midsumxmadd{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\blovisumxmaor}[5]{\blovisuaorbase{\midsumxmadd{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\bloivsumxmaor}[5]{\bloivsuaorbase{\midsuivmxmadd{#1}{#2}{#4}{#5}}{#3}}
%%%%% su xxx
\newcommand{\blosuxxxlarge}[5]{\blosubase{\midsuxxxlarge{#1}{#2}{#3}{#4}}{#5}}
\newcommand{\blosuxxx}[5]{\blosubase{\midsuxxx{#1}{#2}{#3}{#4}}{#5}}
\newcommand{\blovisuxxx}[5]{\blovisubase{\midsuivxxx{#1}{#2}{#3}{#4}}{#5}}
\newcommand{\bloivsuxxx}[5]{\bloivsubase{\midsuivxxx{#1}{#2}{#3}{#4}}{#5}}
%%%%% su xxx or
\newcommand{\blosuxxxlargeor}[5]{\blosuorbase{\midsuxxxlargeadd{#1}{#2}{#3}{#4}}{#5}}
\newcommand{\blosuxxxor}[5]{\blosuorbase{\midsuxxxadd{#1}{#2}{#3}{#4}}{#5}}
\newcommand{\blovisuxxxor}[5]{\blovisuorbase{\midsuivxxxadd{#1}{#2}{#3}{#4}}{#5}}
\newcommand{\bloivsuxxxor}[5]{\bloivsuorbase{\midsuivxxxadd{#1}{#2}{#3}{#4}}{#5}}
%%%%% su xxx aor
\newcommand{\blosuxxxlargeaor}[5]{\blosuaorbase{\midsuxxxlargeadd{#1}{#2}{#3}{#4}}{#5}}
\newcommand{\blosuxxxaor}[5]{\blosuaorbase{\midsuxxxadd{#1}{#2}{#3}{#4}}{#5}}
\newcommand{\blovisuxxxaor}[5]{\blovisuaorbase{\midsuivxxxadd{#1}{#2}{#3}{#4}}{#5}}
\newcommand{\bloivsuxxxaor}[5]{\bloivsuaorbase{\midsuivxxxadd{#1}{#2}{#3}{#4}}{#5}}
%%%%% su intmvuoto
\newcommand{\blosuintmvuoto}[3]{\blosubase{\midsuintmvuoto{#1}{#2}}{#3}}
\newcommand{\blovisuintmvuoto}[3]{\blovisubase{\midsuintmvuoto{#1}{#2}}{#3}}
\newcommand{\bloivsuintmvuoto}[3]{\bloivsubase{\midsuintmvuoto{#1}{#2}}{#3}}
%%%%% su dst
\newcommand{\blosudst}[3]{\blosudstbase{\midsuadd{#1}{#2}}{#3}}
\newcommand{\bloivsudst}[3]{\bloivsudstbase{\midsuivadd{#1}{#2}}{#3}}
\newcommand{\blovisudst}[3]{\blovisudstbase{\midsuadd{#1}{#2}}{#3}}
%%%%% su snt
\newcommand{\blosusnt}[3]{\blosusntbase{\midsuadd{#1}{#2}}{#3}}
\newcommand{\bloivsusnt}[3]{\bloivsusntbase{\midsuivadd{#1}{#2}}{#3}}
\newcommand{\blovisusnt}[3]{\blovisusntbase{\midsuadd{#1}{#2}}{#3}}
%%%%% su mxm dst
\newcommand{\blosumxmdst}[5]{\blosudstbase{\midsumxmadd{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\bloivsumxmdst}[5]{\bloivsudstbase{\midsuivmxmadd{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\blovisumxmdst}[5]{\blovisudstbase{\midsumxmadd{#1}{#2}{#4}{#5}}{#3}}
%%%%% su mxm snt
\newcommand{\blosumxmsnt}[5]{\blosusntbase{\midsumxmadd{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\bloivsumxmsnt}[5]{\bloivsusntbase{\midsuivmxmadd{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\blovisumxmsnt}[5]{\blovisusntbase{\midsumxmadd{#1}{#2}{#4}{#5}}{#3}}


%%%%% giu
\newcommand{\blogiu}[3]{\blogiubase{\midgiu{#1}{#2}}{#3}}
\newcommand{\blovigiu}[3]{\blovigiubase{\midgiu{#1}{#2}}{#3}}
\newcommand{\bloivgiu}[3]{\bloivgiubase{\midgiuiv{#1}{#2}}{#3}}
%%%%% giu or
\newcommand{\blogiuor}[3]{\blogiuorbase{\midgiuadd{#1}{#2}}{#3}}
\newcommand{\blovigiuor}[3]{\blovigiuorbase{\midgiuadd{#1}{#2}}{#3}}
\newcommand{\bloivgiuor}[3]{\bloivgiuorbase{\midgiuivadd{#1}{#2}}{#3}}
%%%%% giu aor
\newcommand{\blogiuaor}[3]{\blogiuaorbase{\midgiuadd{#1}{#2}}{#3}}
\newcommand{\blovigiuaor}[3]{\blovigiuaorbase{\midgiuadd{#1}{#2}}{#3}}
\newcommand{\bloivgiuaor}[3]{\bloivgiuaorbase{\midgiuivadd{#1}{#2}}{#3}}
%%%%% giu large
\newcommand{\blogiularge}[3]{\blogiubase{\midgiularge{#1}{#2}}{#3}}
%%%%% giu large or
\newcommand{\blogiulargeor}[3]{\blogiuorbase{\midgiulargeadd{#1}{#2}}{#3}}
%%%%% giu large aor
\newcommand{\blogiulargeaor}[3]{\blogiuaorbase{\midgiulargeadd{#1}{#2}}{#3}}
%%%%% giu big
\newcommand{\blogiubig}[3]{\blogiubase{\midgiubig{#1}{#2}}{#3}}
%%%%% giu big or
\newcommand{\blogiubigor}[3]{\blogiuorbase{\midgiubigadd{#1}{#2}}{#3}}
%%%%% giu big aor
\newcommand{\blogiubigaor}[3]{\blogiuaorbase{\midgiubigadd{#1}{#2}}{#3}}
%%%%% giu intm
\newcommand{\blogiuintmlarge}[3]{\blogiubase{\midgiuintmlarge{#1}{#2}}{#3}}
\newcommand{\blogiuintm}[3]{\blogiubase{\midgiuintm{#1}{#2}}{#3}}
\newcommand{\blovigiuintm}[3]{\blovigiubase{\midgiuintm{#1}{#2}}{#3}}
\newcommand{\bloivgiuintm}[3]{\bloivgiubase{\midgiuintmtre{#1}{#2}}{#3}}
%%%%% giu intm or
\newcommand{\blogiuintmorlarge}[3]{\blogiuorbase{\midgiuintmaddlarge{#1}{#2}}{#3}}
\newcommand{\blogiuintmor}[3]{\blogiuorbase{\midgiuintmadd{#1}{#2}}{#3}}
\newcommand{\blovigiuintmor}[3]{\blovigiuorbase{\midgiuintmadd{#1}{#2}}{#3}}
\newcommand{\bloivgiuintmor}[3]{\bloivgiuorbase{\midgiuintmtreadd{#1}{#2}}{#3}}
%%%%% giu intm aor
\newcommand{\blogiuintmaorlarge}[3]{\blogiuaorbase{\midgiuintmaddlarge{#1}{#2}}{#3}}
\newcommand{\blogiuintmaor}[3]{\blogiuaorbase{\midgiuintmadd{#1}{#2}}{#3}}
\newcommand{\blovigiuintmaor}[3]{\blovigiuaorbase{\midgiuintmadd{#1}{#2}}{#3}}
\newcommand{\bloivgiuintmaor}[3]{\bloivgiuaorbase{\midgiuintmtreadd{#1}{#2}}{#3}}
%%%%% giu mint
\newcommand{\blogiumintlarge}[3]{\blogiubase{\midgiumintlarge{#1}{#2}}{#3}}
\newcommand{\blogiumint}[3]{\blogiubase{\midgiumint{#1}{#2}}{#3}}
\newcommand{\blovigiumint}[3]{\blovigiubase{\midgiumint{#1}{#2}}{#3}}
\newcommand{\bloivgiumint}[3]{\bloivgiubase{\midgiuminttre{#1}{#2}}{#3}}
%%%%% giu mint or
\newcommand{\blogiumintorlarge}[3]{\blogiuorbase{\midgiumintaddlarge{#1}{#2}}{#3}}
\newcommand{\blogiumintor}[3]{\blogiuorbase{\midgiumintadd{#1}{#2}}{#3}}
\newcommand{\blovigiumintor}[3]{\blovigiuorbase{\midgiumintadd{#1}{#2}}{#3}}
\newcommand{\bloivgiumintor}[3]{\bloivgiuorbase{\midgiuminttreadd{#1}{#2}}{#3}}
%%%%% giu mint aor
\newcommand{\blogiumintaorlarge}[3]{\blogiuaorbase{\midgiumintaddlarge{#1}{#2}}{#3}}
\newcommand{\blogiumintaor}[3]{\blogiuaorbase{\midgiumintadd{#1}{#2}}{#3}}
\newcommand{\blovigiumintaor}[3]{\blovigiuaorbase{\midgiumintadd{#1}{#2}}{#3}}
\newcommand{\bloivgiumintaor}[3]{\bloivgiuaorbase{\midgiuminttreadd{#1}{#2}}{#3}}
%%%%% giu derm
\newcommand{\blogiudermlarge}[3]{\blogiubase{\midgiudermlarge{#1}{#2}}{#3}}
\newcommand{\blogiuderm}[3]{\blogiubase{\midgiuderm{#1}{#2}}{#3}}
\newcommand{\blovigiuderm}[3]{\blovigiubase{\midgiuderm{#1}{#2}}{#3}}
\newcommand{\bloivgiuderm}[3]{\bloivgiubase{\midgiudermtre{#1}{#2}}{#3}}
%%%%% giu derm or
\newcommand{\blogiudermorlarge}[3]{\blogiuorbase{\midgiudermaddlarge{#1}{#2}}{#3}}
\newcommand{\blogiudermor}[3]{\blogiuorbase{\midgiudermadd{#1}{#2}}{#3}}
\newcommand{\blovigiudermor}[3]{\blovigiuorbase{\midgiudermadd{#1}{#2}}{#3}}
\newcommand{\bloivgiudermor}[3]{\bloivgiuorbase{\midgiudermtreadd{#1}{#2}}{#3}}
%%%%% giu derm aor
\newcommand{\blogiudermaorlarge}[3]{\blogiuaorbase{\midgiudermaddlarge{#1}{#2}}{#3}}
\newcommand{\blogiudermaor}[3]{\blogiuaorbase{\midgiudermadd{#1}{#2}}{#3}}
\newcommand{\blovigiudermaor}[3]{\blovigiuaorbase{\midgiudermadd{#1}{#2}}{#3}}
\newcommand{\bloivgiudermaor}[3]{\bloivgiuaorbase{\midgiudermtreadd{#1}{#2}}{#3}}
%%%%% giu mder
\newcommand{\blogiumderlarge}[3]{\blogiubase{\midgiumderlarge{#1}{#2}}{#3}}
\newcommand{\blogiumder}[3]{\blogiubase{\midgiumder{#1}{#2}}{#3}}
\newcommand{\blovigiumder}[3]{\blovigiubase{\midgiumder{#1}{#2}}{#3}}
\newcommand{\bloivgiumder}[3]{\bloivgiubase{\midgiumdertre{#1}{#2}}{#3}}
%%%%% giu mder or
\newcommand{\blogiumderorlarge}[3]{\blogiuorbase{\midgiumderaddlarge{#1}{#2}}{#3}}
\newcommand{\blogiumderor}[3]{\blogiuorbase{\midgiumderadd{#1}{#2}}{#3}}
\newcommand{\blovigiumderor}[3]{\blovigiuorbase{\midgiumderadd{#1}{#2}}{#3}}
\newcommand{\bloivgiumderor}[3]{\bloivgiuorbase{\midgiumdertreadd{#1}{#2}}{#3}}
%%%%% giu mder aor
\newcommand{\blogiumderaorlarge}[3]{\blogiuaorbase{\midgiumderaddlarge{#1}{#2}}{#3}}
\newcommand{\blogiumderaor}[3]{\blogiuaorbase{\midgiumderadd{#1}{#2}}{#3}}
\newcommand{\blovigiumderaor}[3]{\blovigiuaorbase{\midgiumderadd{#1}{#2}}{#3}}
\newcommand{\bloivgiumderaor}[3]{\bloivgiuaorbase{\midgiumdertreadd{#1}{#2}}{#3}}
%%%%% giu mxm
\newcommand{\blogiumxmlarge}[5]{\blogiubase{\midgiumxmlarge{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\blogiumxm}[5]{\blogiubase{\midgiumxm{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\blovigiumxm}[5]{\blovigiubase{\midgiumxm{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\bloivgiumxm}[5]{\bloivgiubase{\midgiuivmxm{#1}{#2}{#4}{#5}}{#3}}
%%%%% giu mxm or
\newcommand{\blogiumxmorlarge}[5]{\blogiuorbase{\midgiumxmaddlarge{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\blogiumxmor}[5]{\blogiuorbase{\midgiumxmadd{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\blovigiumxmor}[5]{\blovigiuorbase{\midgiumxmadd{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\bloivgiumxmor}[5]{\bloivgiuorbase{\midgiuivmxmadd{#1}{#2}{#4}{#5}}{#3}} %%
%%%%% giu mxm aor
\newcommand{\blogiumxmaorlarge}[5]{\blogiuaorbase{\midgiumxmaddlarge{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\blogiumxmaor}[5]{\blogiuaorbase{\midgiumxmadd{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\blovigiumxmaor}[5]{\blovigiuaorbase{\midgiumxmadd{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\bloivgiumxmaor}[5]{\bloivgiuaorbase{\midgiuivmxmadd{#1}{#2}{#4}{#5}}{#3}}
%%%%% giu xxx
\newcommand{\blogiuxxxlarge}[5]{\blogiubase{\midgiuxxxlarge{#1}{#2}{#3}{#4}}{#5}}
\newcommand{\blogiuxxx}[5]{\blogiubase{\midgiuxxx{#1}{#2}{#3}{#4}}{#5}}
\newcommand{\blovigiuxxx}[5]{\blovigiubase{\midgiuxxx{#1}{#2}{#3}{#4}}{#5}}
\newcommand{\bloivgiuxxx}[5]{\bloivgiubase{\midgiuivxxx{#1}{#2}{#3}{#4}}{#5}}
%%%%% giu xxx or
\newcommand{\blogiuxxxlargeor}[5]{\blogiuorbase{\midgiuxxxlargeadd{#1}{#2}{#3}{#4}}{#5}}
\newcommand{\blogiuxxxor}[5]{\blogiuorbase{\midgiuxxxadd{#1}{#2}{#3}{#4}}{#5}}
\newcommand{\blovigiuxxxor}[5]{\blovigiuorbase{\midgiuxxxadd{#1}{#2}{#3}{#4}}{#5}}
\newcommand{\bloivgiuxxxor}[5]{\bloivgiuorbase{\midgiuivxxxadd{#1}{#2}{#3}{#4}}{#5}} %%
%%%%% giu xxx aor
\newcommand{\blogiuxxxlargeaor}[5]{\blogiuaorbase{\midgiuxxxlargeadd{#1}{#2}{#3}{#4}}{#5}}
\newcommand{\blogiuxxxaor}[5]{\blogiuaorbase{\midgiuxxxadd{#1}{#2}{#3}{#4}}{#5}}
\newcommand{\blovigiuxxxaor}[5]{\blovigiuaorbase{\midgiuxxxadd{#1}{#2}{#3}{#4}}{#5}}
\newcommand{\bloivgiuxxxaor}[5]{\bloivgiuaorbase{\midgiuivxxxadd{#1}{#2}{#3}{#4}}{#5}}
%%%%% giu intmvuoto
\newcommand{\blogiuintmvuoto}[3]{\blogiubase{\midgiuintmvuoto{#1}{#2}}{#3}}
\newcommand{\blovigiuintmvuoto}[3]{\blovigiubase{\midgiuintmvuoto{#1}{#2}}{#3}}
\newcommand{\bloivgiuintmvuoto}[3]{\bloivgiubase{\midgiuintmvuoto{#1}{#2}}{#3}}
%%%%% giu dst
\newcommand{\blogiudst}[3]{\blogiudstbase{\midgiuadd{#1}{#2}}{#3}}
\newcommand{\bloivgiudst}[3]{\bloivgiudstbase{\midgiuivadd{#1}{#2}}{#3}}
\newcommand{\blovigiudst}[3]{\blovigiudstbase{\midgiuadd{#1}{#2}}{#3}}
%%%%% giu snt
\newcommand{\blogiusnt}[3]{\blogiusntbase{\midgiuadd{#1}{#2}}{#3}}
\newcommand{\bloivgiusnt}[3]{\bloivgiusntbase{\midgiuivadd{#1}{#2}}{#3}}
\newcommand{\blovigiusnt}[3]{\blovigiusntbase{\midgiuadd{#1}{#2}}{#3}}
%%%%% giu mxm dst
\newcommand{\blogiumxmdst}[5]{\blogiudstbase{\midgiumxmadd{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\bloivgiumxmdst}[5]{\bloivgiudstbase{\midgiuivmxmadd{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\blovigiumxmdst}[5]{\blovigiudstbase{\midgiumxmadd{#1}{#2}{#4}{#5}}{#3}}
%%%%% giu mxm snt
\newcommand{\blogiumxmsnt}[5]{\blogiusntbase{\midgiumxmadd{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\bloivgiumxmsnt}[5]{\bloivgiusntbase{\midgiuivmxmadd{#1}{#2}{#4}{#5}}{#3}}
\newcommand{\blovigiumxmsnt}[5]{\blovigiusntbase{\midgiumxmadd{#1}{#2}{#4}{#5}}{#3}}

%%%%%%%%%%%%%% sopra \`e aggiornato
%%%%%%%%%%%%%% sopra \`e aggiornato

%%%% kx

%%>>%%        'kxdst','{2}{2}{3}{4}',''
\newcommand{\kxdst}[4]{\begin{picture}(0,1)
   \put(0,0){\vector(1,0){1}}
   \psset{unit=0.5\unitlength}
   \rput[lb](2,-#1){\psset{unit=2.0\unitlength}
   \framebox(#1,#1){$#2$}}
   \psset{unit=2.0\unitlength}
   \put(#1,0){
   \put(1,0){\vector(1,0){1}}
   \put(2.25, 0.5){\makebox(0,0)[bl]{$#3$}}
   \put(2.25,-0.5){\makebox(0,0)[tl]{$#4$}}}
\end{picture}}

%%>>%%        'kxsnt','{2}{2}{3}{4}','\small kxdst,\\ kxsnt,\\(x,2,3,4): \\ \\ (x,x)=(2,2) dimensione del blocco.'
\newcommand{\kxsnt}[4]{\begin{picture}(0,1)
   \put(1,0){\vector(-1,0){1}}
   \put(-0.25, 0.5){\makebox(0,0)[br]{$#3$}}
   \put(-0.25,-0.5){\makebox(0,0)[tr]{$#4$}}
   \put(#1,0){
   \put(2,0){\vector(-1,0){1}}
   \psset{unit=0.5\unitlength}
   \rput[rb](2,-#1){\psset{unit=2.0\unitlength}
   \framebox(#1,#1){$#2$}}
   \psset{unit=2.0\unitlength}}
\end{picture}}

%%%% kxy

%%>>%%        'kxydst','{2}{3}{2}{3}{4}',''
\newcommand{\kxydst}[5]{\begin{picture}(0,1)
   \put(0,0){\vector(1,0){1}}
   \psset{unit=0.5\unitlength}
   \rput[lb](2,-#2){\psset{unit=2.0\unitlength}
   \framebox(#1,#2){$#3$}}
   \psset{unit=2.0\unitlength}
   \put(#1,0){
   \put(1,0){\vector(1,0){1}}
   \put(2.25, 0.5){\makebox(0,0)[bl]{$#4$}}
   \put(2.25,-0.5){\makebox(0,0)[tl]{$#5$}}}
\end{picture}}

%%>>%%        'kxysnt','{2}{3}{3}{4}{5}','\small kxydst,\\ kxysnt,\\(x,y,3,4,5): \\ \\ (x,y)=(2,3) \\dimensione del blocco'
\newcommand{\kxysnt}[5]{\begin{picture}(0,1)
   \put(1,0){\vector(-1,0){1}}
   \put(-0.25, 0.5){\makebox(0,0)[br]{$#4$}}
   \put(-0.25,-0.5){\makebox(0,0)[tr]{$#5$}}
   \put(#1,0){
   \put(2,0){\vector(-1,0){1}}
   \psset{unit=0.5\unitlength}
   \rput[rb](2,-#2){\psset{unit=2.0\unitlength}
   \framebox(#1,#2){$#3$}}
   \psset{unit=2.0\unitlength}}
\end{picture}}

\newcommand{\blokxbase}[3]{\begin{picture}(#1,10)
   \put(0, 0){\tratteggio}
   \put(0, 0){#2}
   \put(0,10){#3}
\end{picture}
\begin{picture}(2,10)\put(0, 0){}\end{picture}
}
%
%%>>%%      'blokxor','{2}{2}{3}{4}{5}',''
\newcommand{\blokxor}[5]{\blokxbase{#1}{\kxsnt{#1}{#3}{}{#5}}{\kxdst{#1}{#2}{#4}{}}}
%%>>%%      'blokxaor','{2}{2}{3}{4}{5}','\small blokxor,\\ blokxaor,\\(x,2,3,4,5): \\ \\ (x,x)=(2,2) \\dimensione del blocco'
\newcommand{\blokxaor}[5]{\blokxbase{#1}{\kxdst{#1}{#3}{}{#5}}{\kxsnt{#1}{#2}{#4}{}}}
%%>>%%      'blokxyor','{2}{3}{3}{4}{5}{6}',''
\newcommand{\blokxyor}[6]{\blokxbase{#1}{\kxysnt{#1}{#2}{#4}{}{#6}}{\kxydst{#1}{#2}{#3}{#5}{}}}
%%>>%%      'blokxyaor','{2}{3}{3}{4}{5}{6}','\small blokxyor,\\ blokxyaor,\\(x,y,3,4,5,6): \\ \\ (x,y)=(2,3) \\dimensione del blocco'
\newcommand{\blokxyaor}[6]{\blokxbase{#1}{\kxydst{#1}{#2}{#4}{}{#6}}{\kxysnt{#1}{#2}{#3}{#5}{}}}
%%>>%%      'blokxydst','{2}{3}{3}{4}{5}{6}',''
\newcommand{\blokxydst}[6]{\blokxbase{#1}{\kxydst{#1}{#2}{#4}{}{#6}}{\kxydst{#1}{#2}{#3}{#5}{}}}
%%>>%%      'blokxysnt','{2}{3}{3}{4}{5}{6}',''
\newcommand{\blokxysnt}[6]{\blokxbase{#1}{\kxysnt{#1}{#2}{#4}{}{#6}}{\kxysnt{#1}{#2}{#3}{#5}{}}}


%%%>>%%      'blokxyzor','{2}{3}{3}{4}{5}{6}',''
%\newcommand{\blokxyzor}[6]{\blokxbase{#1}{\kxysnt{#1}{#2}{#4}{}{#6}}{\kxydst{#1}{#2}{#3}{#5}{}}}
%%%>>%%      'blokxyzaor','{2}{3}{3}{4}{5}{6}','\small blokxyzor,\\ blokxyaor,\\(x,y,3,4,5,6): \\ \\ (x,y)=(2,3) \\dimensione del blocco'
%\newcommand{\blokxyzaor}[6]{\blokxbase{#1}{\kxydst{#1}{#2}{#4}{}{#6}}{\kxysnt{#1}{#2}{#3}{#5}{}}}
%
%
%%%>>%%        'kxyzdst','{2}{3}{2}{3}{4}',''
%\newcommand{\kxyzdst}[6]{\begin{picture}(0,1)
%   \put(0,0){\vector(1,0){#6}}
%   \psset{unit=0.5\unitlength}
%   \rput[lb](2,-#2){\psset{unit=2.0\unitlength}
%   \framebox(#1,#2){$#3$}}
%   \psset{unit=2.0\unitlength}
%   \put(#1,0){
%   \put(1,0){\vector(1,0){1}}
%   \put(2.25, 0.5){\makebox(0,0)[bl]{$#4$}}
%   \put(2.25,-0.5){\makebox(0,0)[tl]{$#5$}}}
%\end{picture}}
%
%%%>>%%        'kxyzsnt','{2}{3}{3}{4}{5}','\small kxyzdst,\\ kxyzsnt,\\(x,y,3,4,5): \\ \\ (x,y)=(2,3) \\dimensione del blocco'
%\newcommand{\kxyzsnt}[5]{\begin{picture}(0,1)
%   \put(1,0){\vector(-1,0){1}}
%   \put(-0.25, 0.5){\makebox(0,0)[br]{$#4$}}
%   \put(-0.25,-0.5){\makebox(0,0)[tr]{$#5$}}
%   \put(#1,0){
%   \put(2,0){\vector(-1,0){1}}
%   \psset{unit=0.5\unitlength}
%   \rput[rb](2,-#2){\psset{unit=2.0\unitlength}
%   \framebox(#1,#2){$#3$}}
%   \psset{unit=2.0\unitlength}}
%\end{picture}}
%


%%%%% kdue
\newcommand{\kduedst}[3]{\kxdst{2}{#1}{#2}{#3}}
\newcommand{\kduesnt}[3]{\kxsnt{2}{#1}{#2}{#3}}
%%%%% ktre
\newcommand{\ktredst}[3]{\kxdst{4}{#1}{#2}{#3}}
\newcommand{\ktresnt}[3]{\kxsnt{4}{#1}{#2}{#3}}
%%%%% kqua
\newcommand{\kquadst}[3]{\kxydst{4}{3}{#1}{#2}{#3}}
\newcommand{\kquasnt}[3]{\kxysnt{4}{3}{#1}{#2}{#3}}
%%%%% kcin
\newcommand{\kcindst}[3]{\kxydst{8}{4}{#1}{#2}{#3}}
\newcommand{\kcinsnt}[3]{\kxysnt{8}{4}{#1}{#2}{#3}}
%%%%% kbase
\newcommand{\blokbase}[2]{\blokxbase{2}{#1}{#2}}
%%%%% blocchi k
\newcommand{\bloko}[4]{\blokxbase{2}{\kduesnt{#2}{}{#4}}{\kduedst{#1}{#3}{}}}
\newcommand{\blokao}[4]{\blokxbase{2}{\kduedst{#2}{}{#4}}{\kduesnt{#1}{#3}{}}}
\newcommand{\bloktreo}[4]{\blokxbase{4}{\ktresnt{#2}{}{#4}}{\ktredst{#1}{#3}{}}}
\newcommand{\bloktreao}[4]{\blokxbase{4}{\ktredst{#2}{}{#4}}{\ktresnt{#1}{#3}{}}}
\newcommand{\blokquao}[4]{\blokxbase{4}{\kquasnt{#2}{}{#4}}{\kquadst{#1}{#3}{}}}
\newcommand{\blokquaao}[4]{\blokxbase{4}{\kquadst{#2}{}{#4}}{\kquasnt{#1}{#3}{}}}
\newcommand{\blokcino}[4]{\blokxbase{8}{\kcinsnt{#2}{}{#4}}{\kcindst{#1}{#3}{}}}
\newcommand{\blokcinao}[4]{\blokxbase{8}{\kcindst{#2}{}{#4}}{\kcinsnt{#1}{#3}{}}}


%%%%%

\newcommand{\blosuatt}[5]{\begin{picture}(8,10)
   \put(2.5,10.5){\makebox(0,0)[b]{$#4$}}
   \put(2,7.5){\makebox(0,0)[r]{$#3$}}
   \put(0,0){\tratteggio}
   \put(0,0){\vector(1,0){2}}
   \put(8,0){\vector(-1,0){5}}
   \put(2.5,0){\circle{1}}
   \put(2.5,0){\piu}
   \put(2.5,0){#5}
   \put(2.5,0.5){\vector(0,1){3}}
   \put(2.5, 2){\punto}
   \put(2.5, 2){\line(1,0){3.5}}
   \put(  6, 2){\vector(0,1){2}}
   \put(  5, 4){\framebox(2,2){$#2$}}
   \put(  1, 3.5){\framebox(3,3){$#1$}}
   \put(2.5, 6.5){\vector(0,1){1.5}}
   \put(  6, 6){\line(0,1){2.5}}
   \put(  6, 8.5){\vector(-1,0){3}}
   \put(2.5,8.5){\circle{1}}
   \put(2.5,8.5){\piu}
   \put(2.5,  9){\vector(0,1){1}}
   \put(2.5, 10){\vector(-1,0){2.5}}
   \put(2.5, 10){\vector(1,0){5.5}}
   \end{picture}}

\newcommand{\blogiuattraor}[5]{\begin{picture}(8,10)
   \put(2,2){\makebox(0,0)[r]{$#3$}}
   \put(0,0){\tratteggio}
   \put(0,0){\vector(1,0){2}}
   \put(3,0){\vector(1,0){5}}
   \put(2.5,0){\circle{1}}
   \put(2.5,0){\piu}
   \put(2.5,0){#5}
   \put(2.5,3.5){\vector(0,-1){3}}
   \put(2.5, 2){\punto}
   \put(2.5, 2){\line(1,0){3.5}}
   \put(  6, 2){\vector(0,1){2}}
   \put(  5, 4){\framebox(2,2){$#2$}}
   \put(  1, 3.5){\framebox(3,3){$#1$}}
   \put(2.5, 8){\vector(0,-1){1.5}}
   \put(  6, 6){\line(0,1){2.5}}
   \put(  6, 8.5){\vector(-1,0){3}}
   \put(2.5,8.5){\circle{1}}
   \put(2.5,8.5){\piu}
   \put(2.5,8.5){#4}
   \put(2.5, 10){\vector(0,-1){1}}
   \put(2.5, 10){\vector(-1,0){2.5}}
   \put(8, 10){\vector(-1,0){5.5}}
   \end{picture}}

\newcommand{\blogiuattror}[5]{\begin{picture}(8,10)
   \put(2,2){\makebox(0,0)[r]{$#3$}}
   \put(0,0){\tratteggio}
   \put(2,0){\vector(-1,0){2}}
   \put(8,0){\vector(-1,0){5}}
   \put(2.5,0){\circle{1}}
   \put(2.5,0){\piu}
   \put(2.5,0){#5}
   \put(2.5,3.5){\vector(0,-1){3}}
   \put(2.5, 2){\punto}
   \put(2.5, 2){\line(1,0){3.5}}
   \put(  6, 2){\vector(0,1){2}}
   \put(  5, 4){\framebox(2,2){$#2$}}
   \put(  1, 3.5){\framebox(3,3){$#1$}}
   \put(2.5, 8){\vector(0,-1){1.5}}
   \put(  6, 6){\line(0,1){2.5}}
   \put(  6, 8.5){\vector(-1,0){3}}
   \put(2.5,8.5){\circle{1}}
   \put(2.5,8.5){\piu}
   \put(2.5,8.5){#4}
   \put(2.5, 10){\vector(0,-1){1}}
   \put(0, 10){\vector(1,0){2.5}}
   \put(2.5, 10){\vector(1,0){5.5}}
   \end{picture}}

\newcommand{\blogiuatt}[5]{\begin{picture}(8,10)
   \put(2.5,-0.5){\makebox(0,0)[t]{$#4$}}
   \put(2,2.5){\makebox(0,0)[r]{$#3$}}
   \put(0,0){\tratteggio}
   \put(0,10){\vector(1,0){2}}
   \put(8,10){\vector(-1,0){5}}
   \put(2.5,10){\circle{1}}
   \put(2.5,10){\piu}
   \put(2.5,10){#5}
   \put(2.5,9.5){\vector(0,-1){3}}
   \put(2.5, 8){\punto}
   \put(2.5, 8){\line(1,0){3.5}}
   \put(  6, 8){\vector(0,-1){2}}
   \put(  5, 4){\framebox(2,2){$#2$}}
   \put(  1, 3.5){\framebox(3,3){$#1$}}
   \put(2.5, 3.5){\vector(0,-1){1.5}}
   \put(  6, 1.5){\line(0,1){2.5}}
   \put(  6, 1.5){\vector(-1,0){3}}
   \put(2.5,1.5){\circle{1}}
   \put(2.5,1.5){\piu}
   \put(2.5,  1){\vector(0,-1){1}}
   \put(2.5,  0){\vector(-1,0){2.5}}
   \put(2.5,  0){\vector(1,0){5.5}}
   \end{picture}}

\newcommand{\blosuattaor}[5]{\begin{picture}(8,10)
   \put(2.5,-0.5){\makebox(0,0)[t]{$#4$}}
   \put(2,2.5){\makebox(0,0)[r]{$#3$}}
   \put(0,0){\tratteggio}
   \put(2,10){\vector(-1,0){2}}
   \put(8,10){\vector(-1,0){5}}
   \put(2.5,10){\circle{1}}
   \put(2.5,10){\piu}
   \put(2.5,10){#5}
   \put(2.5,6.5){\vector(0,1){3}}
   \put(2.5, 8){\punto}
   \put(2.5, 8){\line(1,0){3.5}}
   \put(  6, 8){\vector(0,-1){2}}
   \put(  5, 4){\framebox(2,2){$#2$}}
   \put(  1, 3.5){\framebox(3,3){$#1$}}
   \put(2.5, 2.0){\vector(0,1){1.5}}
   \put(  6, 1.5){\line(0,1){2.5}}
   \put(  6, 1.5){\vector(-1,0){3}}
   \put(2.5,1.5){\circle{1}}
   \put(2.5,1.5){\piu}
   \put(2.5,  0){\vector(0,1){1}}
   \put(0,  0){\vector(1,0){2.5}}
   \put(2.5,  0){\vector(1,0){5.5}}
   \end{picture}}

\newcommand{\blosuattor}[5]{\begin{picture}(8,10)
   \put(2.5,-0.5){\makebox(0,0)[t]{$#4$}}
   \put(2,2.5){\makebox(0,0)[r]{$#3$}}
   \put(0,0){\tratteggio}
   \put(0,10){\vector(1,0){2}}
   \put(3,10){\vector(1,0){5}}
   \put(2.5,10){\circle{1}}
   \put(2.5,10){\piu}
   \put(2.5,10){#5}
   \put(2.5,6.5){\vector(0,1){3}}
   \put(2.5, 8){\punto}
   \put(2.5, 8){\line(1,0){3.5}}
   \put(  6, 8){\vector(0,-1){2}}
   \put(  5, 4){\framebox(2,2){$#2$}}
   \put(  1, 3.5){\framebox(3,3){$#1$}}
   \put(2.5, 2.0){\vector(0,1){1.5}}
   \put(  6, 1.5){\line(0,1){2.5}}
   \put(  6, 1.5){\vector(-1,0){3}}
   \put(2.5,1.5){\circle{1}}
   \put(2.5,1.5){\piu}
   \put(2.5,  0){\vector(0,1){1}}
   \put(2.5,  0){\vector(-1,0){2.5}}
   \put(8,  0){\vector(-1,0){5.5}}
   \end{picture}}

%%%%%%%%%%
%%%%%%%%%%

\newcommand{\blosufdk}[9]{\begin{picture}(8,10)
   \put(2.5,10.5){\makebox(0,0)[b]{$#7$}}
   \put(2.0,8.5){\makebox(0,0)[r]{$#4$}}
   \put(6.25,8){\makebox(0,0)[l]{$#5$}}
   \put(6.25,3.5){\makebox(0,0)[l]{$#6$}}
   \put(0,0){\tratteggio}
   \put(0,0){\vector(1,0){2}}
   \put(8,0){\vector(-1,0){5}}
   \put(2.5,0){\piu}
   \put(2.5,0){#8}
   \put(2.5,0.5){\vector(0,1){1}}
   \put(2.5,2){\piu}
   \put(2.5,2){#9}
   \put(2.5,2.5){\vector(0,1){1.5}}
   \put(2.0,3.5){\makebox(0,0)[rt]{$#3$}}
   \put(6, 2){\vector(-1,0){3}}
   \put(  6, 2){\line(0,1){2.5}}
   \put(  5, 4.5){\framebox(2,2){$#2$}}
   \put(  1, 4.0){\framebox(3,3){$#1$}}
   \put(2.5, 7.0){\vector(0,1){1.5}}
   \put(  6, 8.5){\vector(0,-1){2.0}}
   \put(  6, 8.5){\line(-1,0){3.5}}
   \put(2.5, 8.5){\punto}
   \put(2.5, 8.5){\vector(0,1){1.5}}
   \put(2.5, 10){\vector(-1,0){2.5}}
   \put(2.5, 10){\vector(1,0){5.5}}
   \end{picture}}

\newcommand{\blosuaorpar}[9]{\begin{picture}(8,10)
   \put(2.5,-0.5){\makebox(0,0)[t]{$#7$}}
   \put(2.0,1.5){\makebox(0,0)[r]{$#4$}}
   \put(6.25,2){\makebox(0,0)[l]{$#5$}}
   \put(6.25,6.5){\makebox(0,0)[l]{$#6$}}
   \put(0,0){\tratteggio}
   \put(2,10){\vector(-1,0){2}}
   \put(8,10){\vector(-1,0){5}}
   \put(2.5,10){\piu}
   \put(2.5,10){#8}
   \put(2.5,8.5){\vector(0,1){1}}
   \put(2.5,8){\piu}
   \put(2.5,8){#9}
   \put(2.5,6.0){\vector(0,1){1.5}}
   \put(2.0,6.5){\makebox(0,0)[rb]{$#3$}}
   \put(6, 8){\vector(-1,0){3}}
   \put(  6, 8){\line(0,-1){2.5}}
   \put(  5, 3.5){\framebox(2,2){$#2$}}
   \put(  1, 3.0){\framebox(3,3){$#1$}}
   \put(2.5, 1.5){\vector(0,1){1.5}}
   \put(  6, 1.5){\vector(0,1){2.0}}
   \put(  6, 1.5){\line(-1,0){3.5}}
   \put(2.5, 1.5){\punto}
   \put(2.5, 0.0){\vector(0,1){1.5}}
   \put(0, 0){\vector(1,0){2.5}}
   \put(2.5, 0){\vector(1,0){5.5}}
   \end{picture}}

\newcommand{\blosuorpar}[9]{\begin{picture}(8,10)
   \put(2.5,-0.5){\makebox(0,0)[t]{$#7$}}
   \put(2.0,1.5){\makebox(0,0)[r]{$#4$}}
   \put(6.25,2){\makebox(0,0)[l]{$#5$}}
   \put(6.25,6.5){\makebox(0,0)[l]{$#6$}}
   \put(0,0){\tratteggio}
   \put(0,10){\vector(1,0){2}}
   \put(3,10){\vector(1,0){5}}
   \put(2.5,10){\piu}
   \put(2.5,10){#8}
   \put(2.5,8.5){\vector(0,1){1}}
   \put(2.5,8){\piu}
   \put(2.5,8){#9}
   \put(2.5,6.0){\vector(0,1){1.5}}
   \put(2.0,6.5){\makebox(0,0)[rb]{$#3$}}
   \put(6, 8){\vector(-1,0){3}}
   \put(  6, 8){\line(0,-1){2.5}}
   \put(  5, 3.5){\framebox(2,2){$#2$}}
   \put(  1, 3.0){\framebox(3,3){$#1$}}
   \put(2.5, 1.5){\vector(0,1){1.5}}
   \put(  6, 1.5){\vector(0,1){2.0}}
   \put(  6, 1.5){\line(-1,0){3.5}}
   \put(2.5, 1.5){\punto}
   \put(2.5, 0.0){\vector(0,1){1.5}}
   \put(2.5, 0){\vector(-1,0){2.5}}
   \put(8.0, 0){\vector(-1,0){5.5}}
   \end{picture}}

\newcommand{\blogiufdk}[9]{\begin{picture}(8,10)
   \put(2.5,-0.5){\makebox(0,0)[t]{$#7$}}
   \put(2.0,1.5){\makebox(0,0)[r]{$#4$}}
   \put(6.25,2){\makebox(0,0)[l]{$#5$}}
   \put(6.25,6.5){\makebox(0,0)[l]{$#6$}}
   \put(0,0){\tratteggio}
   \put(0,10){\vector(1,0){2}}
   \put(8,10){\vector(-1,0){5}}
   \put(2.5,10){\piu}
   \put(2.5,10){#8}
   \put(2.5,9.5){\vector(0,-1){1}}
   \put(2.5,8){\piu}
   \put(2.5,8){#9}
   \put(2.5,7.5){\vector(0,-1){1.5}}
   \put(2.0,6.5){\makebox(0,0)[rb]{$#3$}}
   \put(6, 8){\vector(-1,0){3}}
   \put(  6, 8){\line(0,-1){2.5}}
   \put(  5, 3.5){\framebox(2,2){$#2$}}
   \put(  1, 3.0){\framebox(3,3){$#1$}}
   \put(2.5, 3.0){\vector(0,-1){1.5}}
   \put(  6, 1.5){\vector(0,1){2.0}}
   \put(  6, 1.5){\line(-1,0){3.5}}
   \put(2.5, 1.5){\punto}
   \put(2.5, 1.5){\vector(0,-1){1.5}}
   \put(2.5, 0){\vector(-1,0){2.5}}
   \put(2.5, 0){\vector(1,0){5.5}}
   \end{picture}}

\newcommand{\blogiuaorpar}[9]{\begin{picture}(8,10)
   \put(2.5,10.5){\makebox(0,0)[b]{$#7$}}
   \put(2.0,8.5){\makebox(0,0)[r]{$#4$}}
   \put(6.25,8){\makebox(0,0)[l]{$#5$}}
   \put(6.25,3.5){\makebox(0,0)[l]{$#6$}}
   \put(0,0){\tratteggio}
   \put(0,0){\vector(1,0){2}}
   \put(3,0){\vector(1,0){5}}
   \put(2.5,0){\piu}
   \put(2.5,0){#8}
   \put(2.5,1.5){\vector(0,-1){1}}
   \put(2.5,2){\piu}
   \put(2.5,2){#9}
   \put(2.5,4.0){\vector(0,-1){1.5}}
   \put(2.0,3.5){\makebox(0,0)[rt]{$#3$}}
   \put(6, 2){\vector(-1,0){3}}
   \put(  6, 2){\line(0,1){2.5}}
   \put(  5, 4.5){\framebox(2,2){$#2$}}
   \put(  1, 4.0){\framebox(3,3){$#1$}}
   \put(2.5, 8.5){\vector(0,-1){1.5}}
   \put(  6, 8.5){\vector(0,-1){2.0}}
   \put(  6, 8.5){\line(-1,0){3.5}}
   \put(2.5, 8.5){\punto}
   \put(2.5, 10){\vector(0,-1){1.5}}
   \put(2.5, 10){\vector(-1,0){2.5}}
   \put(8, 10){\vector(-1,0){5.5}}
   \end{picture}}


\newcommand{\blogiuorpar}[9]{\begin{picture}(8,10)
   \put(2.5,10.5){\makebox(0,0)[b]{$#7$}}
   \put(2.0,8.5){\makebox(0,0)[r]{$#4$}}
   \put(6.25,8){\makebox(0,0)[l]{$#5$}}
   \put(6.25,3.5){\makebox(0,0)[l]{$#6$}}
   \put(0,0){\tratteggio}
   \put(2,0){\vector(-1,0){2}}
   \put(8,0){\vector(-1,0){5}}
   \put(2.5,0){\piu}
   \put(2.5,0){#8}
   \put(2.5,1.5){\vector(0,-1){1}}
   \put(2.5,2){\piu}
   \put(2.5,2){#9}
   \put(2.5,4.0){\vector(0,-1){1.5}}
   \put(2.0,3.5){\makebox(0,0)[rt]{$#3$}}
   \put(6, 2){\vector(-1,0){3}}
   \put(  6, 2){\line(0,1){2.5}}
   \put(  5, 4.5){\framebox(2,2){$#2$}}
   \put(  1, 4.0){\framebox(3,3){$#1$}}
   \put(2.5, 8.5){\vector(0,-1){1.5}}
   \put(  6, 8.5){\vector(0,-1){2.0}}
   \put(  6, 8.5){\line(-1,0){3.5}}
   \put(2.5, 8.5){\punto}
   \put(2.5, 10){\vector(0,-1){1.5}}
   \put(0, 10){\vector(1,0){2.5}}
   \put(2.5, 10){\vector(1,0){5.5}}
   \end{picture}}


%%%%%%%%%%
%%%%%%%%%%

\newcommand{\blogiupar}[9]{\begin{picture}(8,10)
   \put(2.5,-0.5){\makebox(0,0)[t]{$#7$}}
   \put(2,2.5){\makebox(0,0)[r]{$#4$}}
   \put(2,8.0){\makebox(0,0)[r]{$#3$}}
   \put(6.25,2.5){\makebox(0,0)[l]{$#6$}}
   \put(6.25,7.5){\makebox(0,0)[l]{$#5$}}
   \put(0,0){\tratteggio}
   \put(0,10){\vector(1,0){2}}
   \put(8,10){\vector(-1,0){5}}
   \put(2.5,10){\circle{1}}
   \put(2.5,10){\piu}
   \put(2.5,10){#8}
   \put(2.5,9.5){\vector(0,-1){1.5}}
   \put(2.5, 8){\punto}
   \put(2.5, 8){\vector(0,-1){1.5}}
   \put(2.5, 8){\line(1,0){3.5}}
   \put(  6, 8){\vector(0,-1){2}}
   \put(  5, 4){\framebox(2,2){$#2$}}
   \put(  1, 3.5){\framebox(3,3){$#1$}}
   \put(2.5, 3.5){\vector(0,-1){1.5}}
   \put(  6, 1.5){\line(0,1){2.5}}
   \put(  6, 1.5){\vector(-1,0){3}}
   \put(2.5,1.5){\piu}
   \put(2.5,1.5){#9}
   \put(2.5,  1){\vector(0,-1){1}}
   \put(2.5,  0){\vector(-1,0){2.5}}
   \put(2.5,  0){\vector(1,0){5.5}}
   \end{picture}}

\newcommand{\blogiuorfdk}[9]{\begin{picture}(8,10)
   \put(2.5,10.5){\makebox(0,0)[b]{$#7$}}
   \put(2,7.5){\makebox(0,0)[r]{$#4$}}
   \put(2,2.0){\makebox(0,0)[r]{$#3$}}
   \put(6.25,2.5){\makebox(0,0)[l]{$#5$}}
   \put(6.25,7.5){\makebox(0,0)[l]{$#6$}}
   \put(0,0){\tratteggio}
   \put(2,0){\vector(-1,0){2}}
   \put(8,0){\vector(-1,0){5}}
   \put(2.5,0){\circle{1}}
   \put(2.5,2.0){\vector(0,-1){1.5}}
   \put(2.5,0){\piu}
   \put(2.5,0){#8}
   \put(2.5,3.5){\vector(0,-1){1.5}}
   \put(2.5, 2){\punto}
   \put(2.5, 2){\line(1,0){3.5}}
   \put(  6, 2){\vector(0,1){2}}
   \put(  5, 4){\framebox(2,2){$#2$}}
   \put(  1, 3.5){\framebox(3,3){$#1$}}
   \put(2.5, 8.0){\vector(0,-1){1.5}}
   \put(  6, 6){\line(0,1){2.5}}
   \put(  6, 8.5){\vector(-1,0){3}}
   \put(2.5,8.5){\piu}
   \put(2.5,8.5){#9}
   \put(2.5, 10){\vector(0,-1){1}}
   \put(0, 10){\vector(1,0){2.5}}
   \put(2.5, 10){\vector(1,0){5.5}}
   \end{picture}}

\newcommand{\blogiuaorfdk}[9]{\begin{picture}(8,10)
   \put(2.5,10.5){\makebox(0,0)[b]{$#7$}}
   \put(2,7.5){\makebox(0,0)[r]{$#4$}}
   \put(2,2.0){\makebox(0,0)[r]{$#3$}}
   \put(6.25,2.5){\makebox(0,0)[l]{$#5$}}
   \put(6.25,7.5){\makebox(0,0)[l]{$#6$}}
   \put(0,0){\tratteggio}
   \put(0,0){\vector(1,0){2}}
   \put(3,0){\vector(1,0){5}}
   \put(2.5,0){\circle{1}}
   \put(2.5,2.0){\vector(0,-1){1.5}}
   \put(2.5,0){\piu}
   \put(2.5,0){#8}
   \put(2.5,3.5){\vector(0,-1){1.5}}
   \put(2.5, 2){\punto}
   \put(2.5, 2){\line(1,0){3.5}}
   \put(  6, 2){\vector(0,1){2}}
   \put(  5, 4){\framebox(2,2){$#2$}}
   \put(  1, 3.5){\framebox(3,3){$#1$}}
   \put(2.5, 8.0){\vector(0,-1){1.5}}
   \put(  6, 6){\line(0,1){2.5}}
   \put(  6, 8.5){\vector(-1,0){3}}
   \put(2.5,8.5){\piu}
   \put(2.5,8.5){#9}
   \put(2.5, 10){\vector(0,-1){1}}
   \put(2.5, 10){\vector(-1,0){2.5}}
   \put(8, 10){\vector(-1,0){5.5}}
   \end{picture}}

\newcommand{\blosupar}[9]{\begin{picture}(8,10)
   \put(2.5,10.5){\makebox(0,0)[b]{$#7$}}
   \put(2,7.5){\makebox(0,0)[r]{$#4$}}
   \put(2,2.0){\makebox(0,0)[r]{$#3$}}
   \put(6.25,2.5){\makebox(0,0)[l]{$#5$}}
   \put(6.25,7.5){\makebox(0,0)[l]{$#6$}}
   \put(0,0){\tratteggio}
   \put(0,0){\vector(1,0){2}}
   \put(8,0){\vector(-1,0){5}}
   \put(2.5,2.0){\vector(0,1){1.5}}
   \put(2.5,0){\piu}
   \put(2.5,0){#8}
   \put(2.5,0.5){\vector(0,1){1.5}}
   \put(2.5, 2){\punto}
   \put(2.5, 2){\line(1,0){3.5}}
   \put(  6, 2){\vector(0,1){2}}
   \put(  5, 4){\framebox(2,2){$#2$}}
   \put(  1, 3.5){\framebox(3,3){$#1$}}
   \put(2.5, 6.5){\vector(0,1){1.5}}
   \put(  6, 6){\line(0,1){2.5}}
   \put(  6, 8.5){\vector(-1,0){3}}
   \put(2.5,8.5){\circle{1}}
   \put(2.5,8.5){\piu}
   \put(2.5,8.5){#9}
   \put(2.5,  9){\vector(0,1){1}}
   \put(2.5, 10){\vector(-1,0){2.5}}
   \put(2.5, 10){\vector(1,0){5.5}}
   \end{picture}}


\newcommand{\blosuorfdk}[9]{\begin{picture}(8,10)
   \put(2.5,-0.5){\makebox(0,0)[t]{$#7$}}
   \put(2,2.5){\makebox(0,0)[r]{$#4$}}
   \put(2,8.0){\makebox(0,0)[r]{$#3$}}
   \put(6.25,2.5){\makebox(0,0)[l]{$#6$}}
   \put(6.25,7.5){\makebox(0,0)[l]{$#5$}}
   \put(0,0){\tratteggio}
   \put(0,10){\vector(1,0){2}}
   \put(3,10){\vector(1,0){5}}
   \put(2.5,10){\piu}
   \put(2.5,10){#8}
   \put(2.5,8.0){\vector(0,1){1.5}}
   \put(2.5,6.5){\vector(0,1){1.5}}
   \put(2.5, 8){\punto}
   \put(2.5, 8){\line(1,0){3.5}}
   \put(  6, 8){\vector(0,-1){2}}
   \put(  5, 4){\framebox(2,2){$#2$}}
   \put(  1, 3.5){\framebox(3,3){$#1$}}
   \put(2.5, 2.0){\vector(0,1){1.5}}
   \put(  6, 1.5){\line(0,1){2.5}}
   \put(  6, 1.5){\vector(-1,0){3}}
   \put(2.5,1.5){\piu}
   \put(2.5,1.5){#9}
   \put(2.5,  0){\vector(0,1){1}}
   \put(2.5,  0){\vector(-1,0){2.5}}
   \put(8,  0){\vector(-1,0){5.5}}
   \end{picture}}


\newcommand{\blosuaorfdk}[9]{\begin{picture}(8,10)
   \put(2.5,-0.5){\makebox(0,0)[t]{$#7$}}
   \put(2,2.5){\makebox(0,0)[r]{$#4$}}
   \put(2,8.0){\makebox(0,0)[r]{$#3$}}
   \put(6.25,2.5){\makebox(0,0)[l]{$#6$}}
   \put(6.25,7.5){\makebox(0,0)[l]{$#5$}}
   \put(0,0){\tratteggio}
   \put(2,10){\vector(-1,0){2}}
   \put(8,10){\vector(-1,0){5}}
   \put(2.5,10){\piu}
   \put(2.5,10){#8}
   \put(2.5,8.0){\vector(0,1){1.5}}
   \put(2.5,6.5){\vector(0,1){1.5}}
   \put(2.5, 8){\punto}
   \put(2.5, 8){\line(1,0){3.5}}
   \put(  6, 8){\vector(0,-1){2}}
   \put(  5, 4){\framebox(2,2){$#2$}}
   \put(  1, 3.5){\framebox(3,3){$#1$}}
   \put(2.5, 2.0){\vector(0,1){1.5}}
   \put(  6, 1.5){\line(0,1){2.5}}
   \put(  6, 1.5){\vector(-1,0){3}}
   \put(2.5,1.5){\piu}
   \put(2.5,1.5){#9}
   \put(2.5,  0){\vector(0,1){1}}
   \put(0,  0){\vector(1,0){2.5}}
   \put(2.5,  0){\vector(1,0){5.5}}
   \end{picture}}


%%%%%%%%%
%%%%%%%%%

\newcommand{\blovigiuattror}[5]{\begin{picture}(6,10)
   \put(1.25,2){\makebox(0,0)[r]{$#3$}}
   \put(0,0){\tratteggio}
   \put(1,0){\vector(-1,0){1}}
   \put(6,0){\vector(-1,0){4}}
   \put(1.5,0){\circle{1}}
   \put(1.5,0){\piu}
   \put(1.5,0){#5}
   \put(1.5,4){\vector(0,-1){3.5}}
   \put(1.5, 2){\punto}
   \put(1.5, 2){\line(1,0){3}}
   \put(4.5, 2){\vector(0,1){2}}
   \put(3.5, 4){\framebox(2,2){$#2$}}
   \put(0.5, 4){\framebox(2,2){$#1$}}
   \put(1.5, 7.5){\vector(0,-1){1.5}}
   \put(4.5, 6){\line(0,1){2}}
   \put(4.5, 8){\vector(-1,0){2.5}}
   \put(1.5,8){\circle{1}}
   \put(1.5,8){\piu}
   \put(1.5,8){#4}
   \put(1.5, 10){\vector(0,-1){1.5}}
   \put(0, 10){\vector(1,0){1.5}}
   \put(1.5, 10){\vector(1,0){4.5}}
   \end{picture}}

\newcommand{\blovigiuattr}[5]{\begin{picture}(6,10)
   \put(1.5,-0.5){\makebox(0,0)[t]{$#3$}}
   \put(0,0){\tratteggio}
   \put(1.5,0){\vector(-1,0){1.5}}
   \put(1.5,0){\vector(1,0){4.5}}
   \put(1.5,4){\vector(0,-1){4}}
   \put(1.5, 2){\punto}
   \put(1.5, 2){\line(1,0){3}}
   \put(4.5, 2){\vector(0,1){2}}
   \put(3.5, 4){\framebox(2,2){$#2$}}
   \put(0.5, 4){\framebox(2,2){$#1$}}
   \put(1.5, 7.5){\vector(0,-1){1.5}}
   \put(4.5, 6){\line(0,1){2}}
   \put(4.5, 8){\vector(-1,0){2.5}}
   \put(1.5,8){\circle{1}}
   \put(1.5,8){\piu}
   \put(1.5,8){#4}
   \put(1.5, 9.5){\vector(0,-1){1}}
   \put(1.5,10){\circle{1}}
   \put(1.5,10){\piu}
   \put(1.5,10){#5}
   \put(0, 10){\vector(1,0){1}}
   \put(6, 10){\vector(-1,0){4}}
   \end{picture}}

\newcommand{\blosuintpium}[6]{\blosubase{\midsuintpium{#1}{#2}{#4}{#5}{#6}}{#3}}
\newcommand{\blovisuintpium}[6]{\blovisubase{\midsuintpium{#1}{#2}{#4}{#5}{#6}}{#3}}

\newcommand{\blosuattdue}[6]{\begin{picture}(8,10)
   \put(2.5,10.5){\makebox(0,0)[b]{$#5$}}
   \put(3.5,9){\makebox(0,0)[bl]{$#4$}}
   \put(0,0){\tratteggio}
   \put(0,0){\vector(1,0){2}}
   \put(8,0){\vector(-1,0){5}}
   \put(2.5,0){\circle{1}}
   \put(2.5,0){\piu}
   \put(2.5,0){#6}
   \put(2.5,0.5){\vector(0,1){1.5}}
   \put(2.5, 1){\punto}
   \put(2.5, 1){\line(1,0){3.5}}
   \put(  6, 1){\vector(0,1){3}}
   \put( 4.5, 4){\framebox(3,2){$#3$}}
   \put(  1.5, 2){\framebox(2,2){$\frac{1}{s}$}}
   \put(2.5, 4){\vector(0,1){1.5}}
   \put(2.25 ,4.75){\makebox(0,0)[r]{$#1$}}
   \put( 1.5, 5.5){\framebox(2,2){$#2$}}
   \put(2.5, 7.5){\vector(0,1){0.75}}
   \put(  6, 6){\line(0,1){2.75}}
   \put(  6, 8.75){\vector(-1,0){3}}
   \put(2.5,8.75){\circle{1}}
   \put(2.5,8.75){\piu}
   \put(2.5,  9.25){\vector(0,1){.75}}
   \put(2.5, 10){\vector(-1,0){2.5}}
   \put(2.5, 10){\vector(1,0){5.5}}
   \end{picture}}

\newcommand{\blosuatttre}[6]{\begin{picture}(8,10)
   \put(2.5,10.5){\makebox(0,0)[b]{$#5$}}
   \put(3.5,9){\makebox(0,0)[bl]{$#4$}}
   \put(0,0){\tratteggio}
   \put(0,0){\vector(1,0){2}}
   \put(8,0){\vector(-1,0){5}}
   \put(2.5,0){\circle{1}}
   \put(2.5,0){\piu}
   \put(2.5,0){#6}
   \put(2.5,0.5){\vector(0,1){1.5}}
   \put(2.5, 1){\punto}
   \put(2.5, 1){\line(1,0){3.5}}
   \put(  6, 1){\vector(0,1){2.5}}
   \put( 4.5,3.5){\framebox(3,2){$#3$}}
   \put(  1.5, 2){\framebox(2,2){$\frac{1}{s}$}}
   \put(2.5, 4){\vector(0,1){1.5}}
   \put(2.25 ,4.75){\makebox(0,0)[r]{$#1$}}
   \put(1, 5.5){\framebox(3,2){$#2$}}
   \put(2.5, 7.5){\vector(0,1){0.75}}
   \put(  6, 5.5){\line(0,1){3.25}}
   \put(  6, 8.75){\vector(-1,0){3}}
   \put(2.5,8.75){\circle{1}}
   \put(2.5,8.75){\piu}
   \put(2.5,  9.25){\vector(0,1){.75}}
   \put(2.5, 10){\vector(-1,0){2.5}}
   \put(2.5, 10){\vector(1,0){5.5}}
   \end{picture}}

\newcommand{\blogiuatttre}[6]{\begin{picture}(8,10)
   \put(2.5,-0.5){\makebox(0,0)[t]{$#5$}}
   \put(3.5,1){\makebox(0,0)[tl]{$#4$}}
   \put(0,0){\tratteggio}
   \put(0,10){\vector(1,0){2}}
   \put(8,10){\vector(-1,0){5}}
   \put(2.5,10){\circle{1}}
   \put(2.5,10){\piu}
   \put(2.5,10){#6}
   \put(2.5,9.5){\vector(0,-1){1.5}}
   \put(2.5, 9){\punto}
   \put(2.5, 9){\line(1,0){3.5}}
   \put(  6, 9){\vector(0,-1){2.5}}
   \put( 4.5,4.5){\framebox(3,2){$#3$}}
   \put(  1.5, 6){\framebox(2,2){$\frac{1}{s}$}}
   \put(2.5, 6){\vector(0,-1){1.5}}
   \put(2.25 ,5.25){\makebox(0,0)[r]{$#1$}}
   \put(1, 2.5){\framebox(3,2){$#2$}}
   \put(2.5, 2.5){\vector(0,-1){0.75}}
   \put(  6, 4.5){\line(0,-1){3.25}}
   \put(  6, 1.25){\vector(-1,0){3}}
   \put(2.5,1.25){\circle{1}}
   \put(2.5,1.25){\piu}
   \put(2.5,  0.75){\vector(0,-1){.75}}
   \put(2.5,  0){\vector(-1,0){2.5}}
   \put(2.5,  0){\vector(1,0){5.5}}
   \end{picture}}

\newcommand{\tratteggiogiu}[1]{\begin{picture}(0,10)
   \put(0,-1.125){\psline[linestyle=dashed,linewidth=0.2pt](0,0)(0,-#1)}
   \end{picture}}

\newcommand{\scrivigiu}[3]{\begin{picture}(0,10)
   \put(0,0){\tratteggiogiu{#2}}
   \put(0,-1){
   \put(0,-#2){\begin{minipage}[t]{#1\unitlength} \centering #3 \end{minipage}}
   % era \put(0,-4){\begin{minipage}[t]{#1\unitlength} \centering #3 \end{minipage}}
   }
   \end{picture}}

\newcommand{\tratteggiosu}[1]{\begin{picture}(0,10)
   \put(0, 11.125){\psline[linestyle=dashed,linewidth=0.2pt](0,0)(0,#1)}
   \end{picture}}

\newcommand{\scrivisu}[3]{\begin{picture}(0,10)
   \put(0,0){\tratteggiosu{#2}}
   \put(0,10){\put(0,#2){\begin{minipage}[b]{#1\unitlength} \centering #3 \end{minipage}}}
   \end{picture}}


\newcommand{\nrsezsu}[2]{\begin{picture}(0,10)
   \put(0,#2){\small\cput[linewidth=0.3pt,framesep=1pt](0,11.75){\tiny #1}}
  \end{picture}}

\newcommand{\nrsezxsu}[3]{\begin{picture}(0,10)
   \put(0,#3){\pscircle[linewidth=0.3pt](0,11.75){#1}\rput(0,11.75){\tiny #2}}
  \end{picture}}


\newcommand{\nrsezgiu}[2]{\begin{picture}(0,10)
   \put(0,#2){\small\cput[linewidth=0.3pt,framesep=1pt](0,-2){\tiny #1}}
  \end{picture}}

\newcommand{\nrsezxgiu}[3]{\begin{picture}(0,10)
   \put(0,#3){\pscircle[linewidth=0.3pt](0,-2){#1}\rput(0,-2){\tiny #2}}
  \end{picture}}


%%%%%%%%%%%%%%%
\newcommand{\blogiogiu}[3]{\begin{picture}(8,10)
   \put(0,0){\tratteggio}
   \put(2,1){\framebox(4,4){}}
   \put(3,6){\framebox(2,2){{\bf $1/s$}}}
   \put(2.5,3){\line(1,0){3}}
   \put(4,1.5){\line(0,1){3}}
   \put(4.75,3){\line(2,3){1}}
   \put(3.25,3){\line(-2,-3){1}}
   \put(4,10){\piu\dst}
   \put(0,10){\vector(1,0){3.5}}
   \put(8,10){\vector(-1,0){3.5}}
   \put(4,0){\vector(1,0){4}}
   \put(4,0){\vector(-1,0){4}}
   \put(4,0){\punto}
   \put(4,1){\vector(0,-1){1}}
   \put(4,6){\vector(0,-1){1}}
   \put(4,9.5){\vector(0,-1){1.5}}
   \put(3,-2){\makebox(2,2){{\bf $#3$}}}
   \put(4,1.5){\makebox(1.5,1.5){{\bf $#1$}}}
   \put(4,3.5){\makebox(1.5,1.5){{\bf $#2$}}}
\end{picture}}


%%%%%%%%%
%%%%%%%%% Comandi vecchi o poco usati
%%%%%%%%%

\newcommand{\flowrightgiu}[1]{\begin{picture}(0,10)
 %  \put(0,-1){\makebox(0,0)[t]{$\rightarrow$}}
   \psline[linewidth=0.4pt]{->}(-0.5,-1)(0.5,-1)
   \put(0,-1.5){\makebox(0,0)[t]{$#1$}}
\end{picture}}

\newcommand{\flowleftgiu}[1]{\begin{picture}(0,10)
%   \put(0,-1){\makebox(0,0)[t]{$\leftarrow$}}
   \Psline[linewidth=0.4pt]{<-}(-0.5,-1)(0.5,-1)
   \put(0,-1.5){\makebox(0,0)[t]{$#1$}}
\end{picture}}

\newcommand{\flowrightsu}[1]{\begin{picture}(0,10)
%   \put(0,11){\makebox(0,0)[b]{$\rightarrow$}}
   \psline[linewidth=0.4pt]{->}(-0.5,11.5)(0.5,11.5)
   \put(0,11.75){\makebox(0,0)[b]{$#1$}}
\end{picture}}

\newcommand{\flowleftsu}[1]{\begin{picture}(0,10)
%   \put(0,11){\makebox(0,0)[b]{$\leftarrow$}}
   \psline[linewidth=0.4pt]{<-}(-0.5,11.5)(0.5,11.5)
   \put(0,11.75){\makebox(0,0)[b]{$#1$}}
\end{picture}}

%%%%%%

\newcommand{\flowright}[1]{\begin{picture}(0,12)
   \put(0,-1){\makebox(0,0)[t]{$\Rightarrow$}}
\end{picture}}

\newcommand{\flowleft}[1]{\begin{picture}(0,12)
   \put(0,-1){\makebox(0,0)[t]{$\leftarrow$}}
\end{picture}}

\newcommand{\downdot}[1]{\begin{picture}(0,12)
   \put(0,-1){\makebox(0,0)[t]{$#1$}}
\end{picture}}

\newcommand{\updot}[1]{\begin{picture}(0,12)
   \put(0,11){\makebox(0,0)[b]{$#1$}}
\end{picture}}

\newcommand{\attdstsnt}[1]{\begin{picture}(0,1)
   \put(2.5,-1.5){\framebox(3,3){#1}}
   \put(0,0){\vector(1,0){2.5}}
   \put(8,0){\vector(-1,0){2.5}}
\end{picture}}

\newcommand{\midgiuadd}[2]{\begin{picture}(0,1)
   \put( 0, 10){\vector(0,-1){3}}
   \put(-2,  3){\framebox(4,4){$#1$}}
   \put( 0,  3){\vector(0,-1){2.5}}
   \put( 0,1.5){\makebox(0,0)[l]{$#2$}}
\end{picture}}

\newcommand{\midgiuvipiu}[2]{\begin{picture}(0,1)
   \put(   0, 10){\vector(0,-1){3.5}}
   \put(-1.5,3.5){\framebox(3,3){$#1$}}
   \put(   0, 3.5){\vector(0,-1){3}}
   \put(   0,1.5){\makebox(0,0)[l]{$#2$}}
\end{picture}}

\newcommand{\midsuvipiu}[2]{\begin{picture}(0,1)
   \put(   0,  0){\vector(0,1){3.5}}
   \put(-1.5,3.5){\framebox(3,3){$#1$}}
   \put(   0,6.5){\vector(0,1){3}}
   \put(   0,8.5){\makebox(0,0)[l]{$#2$}}
\end{picture}}



\newcommand{\midsutrelarge}[2]{\begin{picture}(0,1)
   \put(-2,3.5){\framebox(4,3){$#1$}}
   \put(0,6.5){\vector(0,1){3.5}}
   \put(0,  0){\vector(0,1){3.5}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}


\newcommand{\midsuintpium}[5]{\begin{picture}(0,1)
   \put(    0,0.5){\vector(0,1){0.5}}
   \put(-1.25,  1){\framebox(2.5,2.5){{\bf $\frac{1}{s}$}}}
   \put(    0,3.5){\vector(0,1){1}}
   \put(    0,  5){\piu}
   \put(    0,5.5){\vector(0,1){0.5}}
   \put(    2, 5){\vector(-1,0){1.5}}
   \put(    2, 5){\punto}
   \put(   -1.5,  6){\framebox(3,3){$#1$}}
   \put(    0,  9){\vector(0,1){1}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
   \put(  2.25,5){\makebox(0,0)[l]{$#3$}}
   \put(    0, 5){\makebox(0,0)[c]{$#4$}}
   \put(-0.25, 3.75){\makebox(0,0)[rb]{$#5$}}
\end{picture}}

%\newcommand{\midsupiu}[2]{\begin{picture}(0,1)
%   \put( 0,  7){\vector(0,1){2.5}}
%   \put(-2,  3){\framebox(4,4){$#1$}}
%   \put( 0,  0){\vector(0,1){3}}
%   \put( 0,8.5){\makebox(0,0)[l]{$#2$}}
%\end{picture}}




\newcommand{\bloseiretaor}[2]{\begin{picture}(8,10)
   \put(0,0){\tratteggio}
   \put(3,10){\vector(-1,0){3}}
   \put(3, 0){\midsutre{#1}{#2}}
   \put(0, 0){\vector( 1,0){3}}
\end{picture}}

\newcommand{\bloseiretaorlarge}[2]{\begin{picture}(8,10)
   \put(0,0){\tratteggio}
   \put(3,10){\vector(-1,0){3}}
   \put(3, 0){\midsutrelarge{#1}{#2}}
   \put(0, 0){\vector( 1,0){3}}
\end{picture}}

\newcommand{\bloseiretor}[2]{\begin{picture}(8,10)
   \put(0,0){\bloseiintgiu{#1}{#2}}
   \put(3,0){\vector(-1,0){3}}
\end{picture}}

\newcommand{\bloseigiuao}[2]{\begin{picture}(6,10)
   \put(6,10){\vector(-1,0){3}}
   \put(3,0){\midgiutre{#1}{#2}}
   \put(3,0){\vector(1,0){3}}
\end{picture}}

\newcommand{\bloseiintgiu}[2]{\begin{picture}(8,10)
   \put(0,0){\tratteggio}
   \put(0,10){\vector(1,0){3}}
   \put(3,0){\midgiutre{#1}{#2}}
\end{picture}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\blogiuretor}[3]{\begin{picture}(8,10)
   \put(0,0){\tratteggio}
   \put(4.5,8.0){\makebox(0,0)[lb]{$#2$}}
   \put(0,10){\line(1,0){4}}
   \put(4,10){\vector(0,-1){3}}
   \put(2,3){\framebox(4,4){$#1$}}
   \put(4,3){\line(0,-1){3}}
   \put(4,0){\vector(-1,0){4}}
   \put(4.5,2.0){\makebox(0,0)[lt]{$#3$}}
\end{picture}}

\newcommand{\blogiuretao}[3]{\begin{picture}(0,10)
   \put(8,0){\tratteggio}
   \put(3.5,8.0){\makebox(0,0)[rb]{$#2$}}
   \put(8,10){\line(-1,0){4}}
   \put(4,10){\vector(0,-1){3}}
   \put(2,3){\framebox(4,4){$#1$}}
   \put(4,3){\line(0,-1){3}}
   \put(4,0){\vector(1,0){4}}
   \put(3.5,2.0){\makebox(0,0)[rt]{$#3$}}
\end{picture}}

\newcommand{\blosuretor}[3]{\begin{picture}(8,10)
   \put(8,0){\tratteggio}
   \put(3.5,8.0){\makebox(0,0)[rb]{$#2$}}
   \put(4,10){\vector(1,0){4}}
   \put(4,7){\line(0,1){3}}
   \put(2,3){\framebox(4,4){$#1$}}
   \put(4,0){\vector(0,1){3}}
   \put(8,0){\line(-1,0){4}}
   \put(3.5,2.0){\makebox(0,0)[rt]{$#3$}}
\end{picture}}

\newcommand{\blosuretao}[3]{\begin{picture}(8,10)
   \put(0,0){\tratteggio}
   \put(4.5,8.0){\makebox(0,0)[lb]{$#2$}}
   \put(4,10){\vector(-1,0){4}}
   \put(4,7){\line(0,1){3}}
   \put(2,3){\framebox(4,4){$#1$}}
   \put(4,0){\vector(0,1){3}}
   \put(0,0){\line(1,0){4}}
   \put(4.5,2.0){\makebox(0,0)[lt]{$#3$}}
\end{picture}}

%%%%%%%%%%%%%%%%

\newcommand{\blovigiuretor}[3]{\begin{picture}(8,10)
   \put(0,0){\tratteggio}
   \put(3.5,8.0){\makebox(0,0)[lb]{$#2$}}
   \put(0,10){\line(1,0){3}}
   \put(3,10){\vector(0,-1){3}}
   \put(1,3){\framebox(4,4){$#1$}}
   \put(3,3){\line(0,-1){3}}
   \put(3,0){\vector(-1,0){3}}
   \put(3.5,2.0){\makebox(0,0)[lt]{$#3$}}
\end{picture}}

\newcommand{\blovigiuretao}[3]{\begin{picture}(6,10)
   \put(6,0){\tratteggio}
   \put(2.5,8.0){\makebox(0,0)[rb]{$#2$}}
   \put(6,10){\line(-1,0){3}}
   \put(3,10){\vector(0,-1){3}}
   \put(1,3){\framebox(4,4){$#1$}}
   \put(3,3){\line(0,-1){3}}
   \put(3,0){\vector(1,0){3}}
   \put(2.5,2.0){\makebox(0,0)[rt]{$#3$}}
\end{picture}}

\newcommand{\blovisuretor}[3]{\begin{picture}(6,10)
   \put(6,0){\tratteggio}
   \put(2.5,8.0){\makebox(0,0)[rb]{$#2$}}
   \put(3,10){\vector(1,0){3}}
   \put(3,7){\line(0,1){3}}
   \put(1,3){\framebox(4,4){$#1$}}
   \put(3,0){\vector(0,1){3}}
   \put(6,0){\line(-1,0){3}}
   \put(2.5,2.0){\makebox(0,0)[rt]{$#3$}}
\end{picture}}

\newcommand{\blovisuretao}[3]{\begin{picture}(6,10)
   \put(0,0){\tratteggio}
   \put(3.5,8.0){\makebox(0,0)[lb]{$#2$}}
   \put(3,10){\vector(-1,0){3}}
   \put(3,7){\line(0,1){3}}
   \put(1,3){\framebox(4,4){$#1$}}
   \put(3,0){\vector(0,1){3}}
   \put(0,0){\line(1,0){3}}
   \put(3.5,2.0){\makebox(0,0)[lt]{$#3$}}
\end{picture}}

%%%%%%%%%%%%%%%%

\newcommand{\bloivgiuretor}[3]{\begin{picture}(4,10)
   \put(0,0){\tratteggio}
   \put(2.5,8.0){\makebox(0,0)[lb]{$#2$}}
   \put(0,10){\line(1,0){2}}
   \put(2,10){\vector(0,-1){3.5}}
   \put(0.5,3.5){\framebox(3,3){$#1$}}
   \put(2,3.5){\line(0,-1){3.5}}
   \put(2,0){\vector(-1,0){2}}
   \put(2.5,2.0){\makebox(0,0)[lt]{$#3$}}
\end{picture}}

\newcommand{\bloivgiuretao}[3]{\begin{picture}(4,10)
   \put(4,0){\tratteggio}
   \put(1.5,8.0){\makebox(0,0)[rb]{$#2$}}
   \put(4,10){\line(-1,0){2}}
   \put(2,10){\vector(0,-1){3.5}}
   \put(0.5,3.5){\framebox(3,3){$#1$}}
   \put(2,3.5){\line(0,-1){3.5}}
   \put(2,0){\vector(1,0){2}}
   \put(1.5,2.0){\makebox(0,0)[rt]{$#3$}}
\end{picture}}

\newcommand{\bloivsuretor}[3]{\begin{picture}(4,10)
   \put(4,0){\tratteggio}
   \put(1.5,8.0){\makebox(0,0)[rb]{$#2$}}
   \put(2,10){\vector(1,0){2}}
   \put(2,6.5){\line(0,1){3.5}}
   \put(0.5,3.5){\framebox(3,3){$#1$}}
   \put(2,0){\vector(0,1){3.5}}
   \put(4,0){\line(-1,0){2}}
   \put(1.5,2.0){\makebox(0,0)[rt]{$#3$}}
\end{picture}}

\newcommand{\bloivsuretao}[3]{\begin{picture}(4,10)
   \put(0,0){\tratteggio}
   \put(2.5,8.0){\makebox(0,0)[lb]{$#2$}}
   \put(2,10){\vector(-1,0){2}}
   \put(2,6.5){\line(0,1){3.5}}
   \put(0.5,3.5){\framebox(3,3){$#1$}}
   \put(2,0){\vector(0,1){3.5}}
   \put(0,0){\line(1,0){2}}
   \put(2.5,2.0){\makebox(0,0)[lt]{$#3$}}
\end{picture}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\addgiu}[3]{\begin{picture}(4,10)
   \put(0,0){\tratteggio}
   \put(0,0){\vector( 1,0){1.5}}
   \put(2,0){\piu}
   \put(2,0){\makebox(0,0){$#2$}}
   \put(2.5,-2){\makebox(0,0)[l]{$#3$}}
   \put(4,0){\vector(-1,0){1.5}}
   \put(2,-0.5){\vector(0,-1){1}}
   \put(2,10){\vector(-1,0){2}}
   \put(2,10){\vector( 1,0){2}}
   \put(2,10){\punto}
   \put(2,12){\vector(0,-1){2}}
   \put(2,12){\punto}
   \put(2.5,12){\makebox(0,0)[l]{$#1$}}
\end{picture}}


\newcommand{\addsu}[3]{\begin{picture}(4,10)
   \put(0,0){\tratteggio}
   \put(0,10){\vector( 1,0){1.5}}
   \put(2,10){\piu}
   \put(2,10){\makebox(0,0){$#2$}}
   \put(2.5,12){\makebox(0,0)[l]{$#3$}}
   \put(4,10){\vector(-1,0){1.5}}
   \put(2,10.5){\vector(0,1){1}}
   \put(2,0){\vector(-1,0){2}}
   \put(2,0){\vector( 1,0){2}}
   \put(2,0){\punto}
   \put(2,-2){\vector(0,1){2}}
   \put(2,-2){\punto}
   \put(2.5,-2){\makebox(0,0)[l]{$#1$}}
\end{picture}}


\newcommand{\blopiugiuor}[5]{\begin{picture}(8,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\dotdstdst}
   \put(4,10){\vector(0,-1){1.5}}
   \put(4,8){\piu}
   \put(6,8){\vector(-1,0){1.5}}
   \put(6,8){\punto}
   \put(6.25,8){\makebox(0,0)[l]{$#4$}}
   \put(4,8){\makebox(0,0){$#5$}}
   \put(4,7.5){\vector(0,-1){1}}
   \put(4,2.5){\vector(0,-1){2}}
   \put(1.5,2.5){\framebox(5,4){$#1$}}
   \put(4.5,1.5){\makebox(0,0)[l]{$#2$}}
   \put(0, 0){\sumsntsnt{#3}}
\end{picture}}

\newcommand{\blopiugiuorlarge}[5]{\begin{picture}(8,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\dotdstdst}
   \put(4,10){\vector(0,-1){1.5}}
   \put(4,8){\piu}
   \put(6,8){\vector(-1,0){1.5}}
   \put(6,8){\punto}
   \put(6.25,8){\makebox(0,0)[l]{$#4$}}
   \put(4,8){\makebox(0,0){$#5$}}
   \put(4,7.5){\vector(0,-1){1}}
   \put(4,2.5){\vector(0,-1){2}}
   \put(0.5,2.5){\framebox(7,4){$#1$}}
   \put(4.5,1.5){\makebox(0,0)[l]{$#2$}}
   \put(0, 0){\sumsntsnt{#3}}
\end{picture}}

\newcommand{\blopiugiuaor}[5]{\begin{picture}(8,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\dotsntsnt}
   \put(4,10){\vector(0,-1){1.5}}
   \put(4,8){\piu}
   \put(6,8){\vector(-1,0){1.5}}
   \put(6,8){\punto}
   \put(6.25,8){\makebox(0,0)[l]{$#4$}}
   \put(4,8){\makebox(0,0){$#5$}}
   \put(4,7.5){\vector(0,-1){1}}
   \put(4,2.5){\vector(0,-1){2}}
   \put(1.5,2.5){\framebox(5,4){$#1$}}
   \put(4.5,1.5){\makebox(0,0)[l]{$#2$}}
   \put(0, 0){\sumdstdst{#3}}
\end{picture}}

\newcommand{\blopiugiuaorlarge}[5]{\begin{picture}(8,10)
   \put(0, 0){\tratteggio}
   \put(0,10){\dotsntsnt}
   \put(4,10){\vector(0,-1){1.5}}
   \put(4,8){\piu}
   \put(6,8){\vector(-1,0){1.5}}
   \put(6,8){\punto}
   \put(6.25,8){\makebox(0,0)[l]{$#4$}}
   \put(4,8){\makebox(0,0){$#5$}}
   \put(4,7.5){\vector(0,-1){1}}
   \put(4,2.5){\vector(0,-1){2}}
   \put(0.5,2.5){\framebox(7,4){$#1$}}
   \put(4.5,1.5){\makebox(0,0)[l]{$#2$}}
   \put(0, 0){\sumdstdst{#3}}
\end{picture}}

\newcommand{\midgiutre}[2]{\begin{picture}(0,1)
   \put(-1.5,3.5){\framebox(3,3){$#1$}}
   \put(0,10){\vector(0,-1){3.5}}
   \put(0,3.5){\vector(0,-1){3.5}}
   \put(0,-0.5){\makebox(0,0)[t]{$#2$}}
\end{picture}}

\newcommand{\midgiutreadd}[2]{\midgiuaddbase{\midgiutre{#1}{}}{#2}}

\newcommand{\midsutre}[2]{\begin{picture}(0,1)
   \put(-1.5,3.5){\framebox(3,3){$#1$}}
   \put(0,6.5){\vector(0,1){3.5}}
   \put(0,  0){\vector(0,1){3.5}}
   \put(0,10.5){\makebox(0,0)[b]{$#2$}}
\end{picture}}

\newcommand{\midsutreadd}[2]{\midsuaddbase{\midsutre{#1}{}}{#2}}


\newcommand{\blokcindst}[1]{\begin{picture}(0,1)
   \put(1,-2){\framebox(8,4){$#1$}}
   \put(0,0){\vector(1,0){1}}
   \put(9,0){\vector(1,0){1}}
\end{picture}}

\newcommand{\blokcinsnt}[1]{\begin{picture}(0,1)
   \put(1,-2){\framebox(8,4){$#1$}}
   \put(1,0){\vector(-1,0){1}}
   \put(10,0){\vector(-1,0){1}}
\end{picture}}

\newcommand{\blokaocin}[4]{\begin{picture}(8,10)
   \put(0, 0){\tratteggio}
   \put(0, 0){\blokcindst{#2}}
   \put(0,10){\blokcinsnt{#1}}
   \put(0,10.5){\makebox(0,0)[br]{$#3$}}
   \put(10,-0.5){\makebox(0,0)[tl]{$#4$}}
\end{picture}}

\newcommand{\blokocin}[4]{\begin{picture}(6,10)
   \put(0,0){\tratteggio}
   \put(0,10){\blokcindst{#1}}
   \put(0, 0){\blokcinsnt{#2}}
   \put(10,10.5){\makebox(0,0)[bl]{$#3$}}
   \put(0,-0.5){\makebox(0,0)[tr]{$#4$}}
\end{picture}}


\newcommand{\piudst}{\begin{picture}(1,1)
 \put(0,0){\piu}
 \put(0,0){\dst}
\end{picture}}

%%%%%% kdue
%
%\newcommand{\kduedst}[3]{\begin{picture}(0,1)
%   \put(0,0){\vector(1,0){1}}
%   \put(1,-1){\framebox(2,2){$#1$}}
%   \put(3,0){\vector(1,0){1}}
%   \put(4.25, 0.5){\makebox(0,0)[bl]{$#2$}}
%   \put(4.25,-0.5){\makebox(0,0)[tl]{$#3$}}
%\end{picture}}
%
%\newcommand{\kduesnt}[3]{\begin{picture}(0,1)
%   \put(1,-1){\framebox(2,2){$#1$}}
%   \put(1,0){\vector(-1,0){1}}
%   \put(4,0){\vector(-1,0){1}}
%   \put(-0.25, 0.5){\makebox(0,0)[br]{$#2$}}
%   \put(-0.25,-0.5){\makebox(0,0)[tr]{$#3$}}
%\end{picture}}
%
%%%%%% ktre
%
%\newcommand{\ktredst}[3]{\begin{picture}(0,1)
%   \put(0,0){\vector(1,0){1}}
%   \put(1,-2){\framebox(4,4){$#1$}}
%   \put(5,0){\vector(1,0){1}}
%   \put(6.25, 0.5){\makebox(0,0)[bl]{$#2$}}
%   \put(6.25,-0.5){\makebox(0,0)[tl]{$#3$}}
%\end{picture}}
%
%\newcommand{\ktresnt}[3]{\begin{picture}(0,1)
%   \put(6,0){\vector(-1,0){1}}
%   \put(1,-2){\framebox(4,4){$#1$}}
%   \put(1,0){\vector(-1,0){1}}
%   \put(-0.25, 0.5){\makebox(0,0)[br]{$#2$}}
%   \put(-0.25,-0.5){\makebox(0,0)[tr]{$#3$}}
%\end{picture}}
%
%%%%%% kqua
%
%\newcommand{\kquadst}[3]{\begin{picture}(0,1)
%   \put(0,0){\vector(1,0){1}}
%   \put(1,-1.5){\framebox(4,3){$#1$}}
%   \put(5,0){\vector(1,0){1}}
%   \put(6.25, 0.5){\makebox(0,0)[bl]{$#2$}}
%   \put(6.25,-0.5){\makebox(0,0)[tl]{$#3$}}
%\end{picture}}
%
%\newcommand{\kquasnt}[3]{\begin{picture}(0,1)
%   \put(6,0){\vector(-1,0){1}}
%   \put(1,-1.5){\framebox(4,3){$#1$}}
%   \put(1,0){\vector(-1,0){1}}
%   \put(-0.25, 0.5){\makebox(0,0)[br]{$#2$}}
%   \put(-0.25,-0.5){\makebox(0,0)[tr]{$#3$}}
%\end{picture}}
%
% %%%%% kcin
%
%\newcommand{\kcindst}[3]{\begin{picture}(0,1)
%   \put(0,0){\vector(1,0){1}}
%   \put(1,-2){\framebox(8,4){$#1$}}
%   \put(9,0){\vector(1,0){1}}
%   \put(10.25, 0.5){\makebox(0,0)[bl]{$#2$}}
%   \put(10.25,-0.5){\makebox(0,0)[tl]{$#3$}}
%\end{picture}}
%
%\newcommand{\kcinsnt}[3]{\begin{picture}(0,1)
%   \put(1,0){\vector(-1,0){1}}
%   \put(1,-2){\framebox(8,4){$#1$}}
%   \put(10,0){\vector(-1,0){1}}
%   \put(-0.25, 0.5){\makebox(0,0)[br]{$#2$}}
%   \put(-0.25,-0.5){\makebox(0,0)[tr]{$#3$}}
%\end{picture}}
%
%
% %%%%% Blocchi k
%
%\newcommand{\blokbase}[2]{\begin{picture}(4,10)
%   \put(0, 0){\tratteggio}
%   \put(0, 0){#1}
%   \put(0,10){#2}
%\end{picture}}
%
%
%\newcommand{\bloko}[4]{\blokbase{\kduesnt{#2}{}{#4}}{\kduedst{#1}{#3}{}}}
%\newcommand{\blokao}[4]{\blokbase{\kduedst{#2}{}{#4}}{\kduesnt{#1}{#3}{}}}
%\newcommand{\bloktreo}[4]{\blokbase{\ktresnt{#2}{}{#4}}{\ktredst{#1}{#3}{}}}
%\newcommand{\bloktreao}[4]{\blokbase{\ktredst{#2}{}{#4}}{\ktresnt{#1}{#3}{}}}
%\newcommand{\blokquao}[4]{\blokbase{\kquasnt{#2}{}{#4}}{\kquadst{#1}{#3}{}}}
%\newcommand{\blokquaao}[4]{\blokbase{\kquadst{#2}{}{#4}}{\kquasnt{#1}{#3}{}}}
%\newcommand{\blokcino}[4]{\blokbase{\kcinsnt{#2}{}{#4}}{\kcindst{#1}{#3}{}}}
%\newcommand{\blokcinao}[4]{\blokbase{\kcindst{#2}{}{#4}}{\kcinsnt{#1}{#3}{}}}
%

\newcommand{\midgiupiu}[2]{\begin{picture}(0,1)
   \put( 0, 10){\vector(0,-1){3}}
   \put(-2,  3){\framebox(4,4){$#1$}}
   \put( 0,  3){\vector(0,-1){2.5}}
   \put( 0,1.5){\makebox(0,0)[l]{$#2$}}
\end{picture}}

\newcommand{\addsuaoriv}[2]{\begin{picture}(4,10)
   \put(0,0){\tratteggio}
   \put(1.5,10){\vector(-1,0){1.5}}
   \put(2,10){\piu}
   \put(2,11.5){\punto}
   \put(2,10){\makebox(0,0){$#2$}}
   \put(2.5,12){\makebox(0,0)[l]{$#1$}}
   \put(4,10){\vector(-1,0){1.5}}
   \put(2,11.5){\vector(0,-1){1}}
   \put(0,0){\vector(1,0){4}}
\end{picture}}

\newcommand{\blosuintmp}[5]{\blosubase{\midsuintmp{#1}{#2}{#3}{#4}}{#5}}

\newcommand{\midsuintmp}[4]{\begin{picture}(0,1)
   \put(0,0.5){\vector(0,1){1}}
   \put(-1,1.5){\framebox(2,2){{\bf $\frac{1}{s}$}}}
   \put(0,3.5){\vector(0,1){1}}
   \put(0,5){\piu}
   \put(0,5){\makebox(0,0){$#4$}}
   \put(2,5){\vector(-1,0){1.5}}
   \put(2,5){\punto}
   \put(2.25,5){\makebox(0,0)[l]{$#2$}}
%   \put(0.7,4){\makebox(0,0){$#3$}}
   \put(0,10.5){\makebox(0,0)[b]{$#3$}}
   \put(0,5.5){\vector(0,1){0.75}}
   \put(0,9.25){\vector(0,1){0.75}}
   \put(-2,6.25){\framebox(4,3){$#1$}}
\end{picture}}

\newcommand{\blokodueuno}[8]{\begin{picture}(10,10)
   \put(0,0){\tratteggio}
   \put(0,2.5){\tratteggio}
    \rput(0,10){\punto}
   \psline[linewidth=0.4pt]{->}(1.5,0)(0,0)
   \psline[linewidth=0.4pt]{->}(1.5,2)(0,2)
   \psframe[linewidth=0.4pt](1.5,-1)(6.5,3)
   \put(3.95,1){\makebox(0,0){$#7$}}
   \put(-0.75,3){\makebox(0,0){$#3$}}
   \put(-0.75,-1){\makebox(0,0){$#4$}}
   \psline[linewidth=0.4pt]{->}(8,1)(6.5,1)
   \put(8.65,1.85){\makebox(0,0){$#6$}}
   \rput(8,1){\punto}
   \psline[linewidth=0.4pt]{->}(0,10)(1.5,10)
   \psline[linewidth=0.4pt]{->}(0,12)(1.5,12)
   \psframe[linewidth=0.4pt](1.5,9)(6.6,13)
   \put(3.9,10.8){\makebox(0,0){$#8$}}
   \put(-0.75,9){\makebox(0,0){$#2$}}
   \rput(0,12){\punto}
   \put(-0.75,12.5){\makebox(0,0){$#1$}}
   \psline[linewidth=0.4pt]{->}(6.5,11)(8,11)
   \put(8.65,11.95){\makebox(0,0){$#5$}}
\end{picture}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\POGgiularge}[4]{\begin{picture}(8,10)
   \put(0, 0){\blogiularge{#1}{#3}{#4}}
   \rput[lb](3.25,8.25){$#2$}
\end{picture}}

\newcommand{\POGvigiuaor}[4]{\begin{picture}(6,10)
   \put(0, 0){\blovigiuaor{#1}{#3}{#4}}
   \rput[lb](3.25,8.25){$#2$}
\end{picture}}

\newcommand{\POGvigiuor}[4]{\begin{picture}(6,10)
   \put(0, 0){\blovigiuor{#1}{#3}{#4}}
   \rput[lb](3.25,8.25){$#2$}
\end{picture}}

\newcommand{\POGvisu}[4]{\begin{picture}(6,10)
   \put(0, 0){\blovisu{#1}{}{#4}}
   \rput[lb](3.25,8.25){$#2$}
   \rput[lb](3.25,1.25){$#3$}
\end{picture}}

\newcommand{\POGvisuaor}[4]{\begin{picture}(6,10)
   \put(0, 0){\blovisuaor{#1}{#3}{#4}}
   \rput[lb](3.25,0.75){$#2$}
\end{picture}}

\newcommand{\POGvisuor}[4]{\begin{picture}(6,10)
   \put(0, 0){\blovisuor{#1}{#3}{#4}}
   \rput[lb](3.25,0.75){$#2$}
\end{picture}}

\newcommand{\POGvigiu}[4]{\begin{picture}(6,10)
   \put(0, 0){\blovigiu{#1}{}{#4}}
   \rput[lb](3.25,8.00){$#2$}
   \rput[lb](3.25,1.00){$#3$}
\end{picture}}

\newcommand{\POGsugiu}[2]{\begin{picture}(0,10)
   \rput[b](0,10.95){$#1$}
   \rput[t](0,-0.95){$#2$}
\end{picture}}

\newcommand{\POGsuatt}[9]{\begin{picture}(8,10)
   \put(0, 0){\blosuatt{#1}{#2}{#4}{#8}{#9}}
   \rput[rt](2.25,3.25){$#3$}
   \rput[l](6.25,2.75){$#5$}
   \rput[l](6.25,7.25){$#6$}
   \rput[lb](2.75,0.75){$#7$}
\end{picture}}

\newcommand{\POGgiuattor}[8]{\begin{picture}(8,10)
   \put(0, 0){\blogiuattror{#1}{#2}{#4}{#7}{#8}}
   \rput[rb](2.25,6.75){$#3$}
   \rput[l](6.25,7.25){$#5$}
   \rput[l](6.25,2.75){$#6$}
\end{picture}}

\newcommand{\POGgiuattaor}[8]{\begin{picture}(8,10)
   \put(0, 0){\blogiuattraor{#1}{#2}{#4}{#7}{#8}}
   \rput[rb](2.25,6.75){$#3$}
   \rput[l](6.25,7.25){$#5$}
   \rput[l](6.25,2.75){$#6$}
\end{picture}}

\newcommand{\POGgiuatt}[9]{\begin{picture}(8,10)
   \put(0, 0){\blogiuatt{#1}{#2}{#4}{#8}{#9}}
   \rput[rb](2.25,6.75){$#3$}
   \rput[l](6.25,7.25){$#5$}
   \rput[l](6.25,2.75){$#6$}
   \rput[lt](2.75,9.25){$#7$}
\end{picture}}


\newcommand{\POGgiupar}[9]{\blogiupar{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}
\newcommand{\POGgiuorpar}[9]{\blogiuorpar{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}
\newcommand{\POGgiuaorpar}[9]{\blogiuaorpar{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}
\newcommand{\POGgiufdk}[9]{\blogiufdk{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}
\newcommand{\POGgiuorfdk}[9]{\blogiuorfdk{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}
\newcommand{\POGgiuaorfdk}[9]{\blogiuaorfdk{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}
%
\newcommand{\POGsupar}[9]{\blosupar{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}
\newcommand{\POGsuorpar}[9]{\blosuorpar{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}
\newcommand{\POGsuaorpar}[9]{\blosuaorpar{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}
\newcommand{\POGsufdk}[9]{\blosufdk{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}
\newcommand{\POGsuorfdk}[9]{\blosuorfdk{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}
\newcommand{\POGsuaorfdk}[9]{\blosuaorfdk{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}{#9}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%  IN IN IN

%%%%%  SU SU SU


%%>>%%      'bloivparingiubase','(0,-10)(8,22)B','Commento'
\newcommand{\bloivparingiubase}[9]{\begin{picture}(4,10)
   \put(0,0){\tratteggio}
   \put(0,10){\psline{#1}(1.5,0)}
   \put(1.5,10){\punto}
   \put(1.5,10){\psline{#2}(2,8)}
   \put(1.5,10){\psline{#3}(2,-8)}
   \psline(3.5,-8)(4,-8)
   \psline(3.5,8)(4,8)
   \psline(3.5,2)(4,2)
   \psline(3.5,18)(4,18)
   \put(1.5,0){
   \put(0,0){\pscircle[linewidth=0.4pt]{0.5}}
   \psline{#5}(0.5;58)(2,8)
   \psline{#6}(0.5;-58)(2,-8)
   \psline(0.5; 0)(0;0)
   \psline(0.5; 120)(0;0)
   \psline(0.5; 240)(0;0)
   \psline{#4}(-1.5,0)(-0.5,0)
    #9
    }
    \put(4,8){$#7$}
    \put(4,-8){$#8$}
\end{picture}}


\newcommand{\bloivparingiulab}[4]{\begin{picture}(0,10)
   \put(1.25,10.25){\makebox(0,0)[rb]{$#1$}}
   \put(0.75,0.25){\makebox(0,0)[rb]{$#2$}}
   \put(2.25,3){\makebox(0,0)[rb]{$#3$}}
   \put(2.25,-3){\makebox(0,0)[rt]{$#4$}}
\end{picture}}


\newcommand{\bloivparingiu}[7]{\bloivparingiulab{#4}{#5}{#6}{#7}\bloivparingiubase{->}{->}{->}{<-}{<-}{<-}{#1}{#2}{#3}}
\newcommand{\bloivparingiuuno}[7]{\bloivparingiulab{#4}{#5}{#6}{#7}\bloivparingiubase{<-}{<-}{->}{->}{->}{<-}{#1}{#2}{#3}}
\newcommand{\bloivparingiudue}[7]{\bloivparingiulab{#4}{#5}{#6}{#7}\bloivparingiubase{<-}{->}{<-}{->}{<-}{->}{#1}{#2}{#3}}

%%%%%  SU SU SU

%%>>%%      'bloivparinsubase','','Commento'
\newcommand{\bloivparinsubase}[9]{\begin{picture}(4,10)
   \put(0,0){\tratteggio}
   \put(0,0){\psline{#1}(1.5,0)}
   \put(1.5,0){\punto}
   \put(1.5,0){\psline{#2}(2,8)}
   \put(1.5,0){\psline{#3}(2,-8)}
   \psline(3.5,-8)(4,-8)
   \psline(3.5,8)(4,8)
   \psline(3.5,2)(4,2)
   \psline(3.5,18)(4,18)
   \put(1.5,10){
   \put(0,0){\pscircle[linewidth=0.4pt]{0.5}}
   \psline{#5}(0.5;58)(2,8)
   \psline{#6}(0.5;-58)(2,-8)
   \psline(0.5; 0)(0;0)
   \psline(0.5; 120)(0;0)
   \psline(0.5; 240)(0;0)
   \psline{#4}(-1.5,0)(-0.5,0)
    #9
    }
    \put(4,8){$#7$}
    \put(4,-8){$#8$}
\end{picture}}

\newcommand{\bloivparinsulab}[4]{\begin{picture}(0,10)
   \put(0.75,10.25){\makebox(0,0)[rb]{$#1$}}
   \put(1.25,0.25){\makebox(0,0)[rb]{$#2$}}
   \put(2.25,13){\makebox(0,0)[rb]{$#3$}}
   \put(2.25,7){\makebox(0,0)[rt]{$#4$}}
\end{picture}}


\newcommand{\bloivparinsu}[7]{\bloivparinsulab{#4}{#5}{#6}{#7}\bloivparinsubase{->}{->}{->}{<-}{<-}{<-}{#1}{#2}{#3}}
\newcommand{\bloivparinsuuno}[7]{\bloivparinsulab{#4}{#5}{#6}{#7}\bloivparinsubase{<-}{<-}{->}{->}{->}{<-}{#1}{#2}{#3}}
\newcommand{\bloivparinsudue}[7]{\bloivparinsulab{#4}{#5}{#6}{#7}\bloivparinsubase{<-}{->}{<-}{->}{<-}{->}{#1}{#2}{#3}}

%%%%%%%%%%%%%%%%%% OUT OUT

%%>>%%      'bloivparoutgiubase','','Commento'
\newcommand{\bloivparoutgiubase}[7]{\begin{picture}(4,10)
   \put(0,8){\tratteggio}
   \put(0,-8){\tratteggio}
   \put(2.5,10){\psline{#2}(1.5,0)}
   \put(2.5,10){\punto}
   \put(2.5,10){\psline{#1}(-2,8)}
   \put(2.5,10){\psline{#3}(-2,-8)}
   \put(2.5,0){\psline{#4}(-2,8)(0.5;120)}
   \put(2.5,0){\psline{#6}(-2,-8)(0.5;-120)}
   \psline(0.5,-8)(0,-8)
   \psline(0.5,8)(0,8)
   \psline(0.5,2)(0,2)
   \psline(0.5,18)(0,18)
   \put(2.5,0){
   \put(0,0){\pscircle[linewidth=0.4pt]{0.5}}
   \psline(0.5;180)(0;0)
   \psline(0.5; 60)(0;0)
   \psline(0.5;-60)(0;0)
   \psline{#5}(0.5,0)(1.5,0)
    #7
    }
\end{picture}}


\newcommand{\bloivparoutgiulab}[4]{\begin{picture}(0,10)
   \put(2.75,10.25){\makebox(0,0)[lb]{$#1$}}
   \put(3.25,0.25){\makebox(0,0)[lb]{$#2$}}
   \put(1.75,3){\makebox(0,0)[lb]{$#3$}}
   \put(1.75,-3){\makebox(0,0)[lt]{$#4$}}
\end{picture}}


\newcommand{\bloivparoutgiu}[5]{\bloivparoutgiulab{#2}{#3}{#4}{#5}\bloivparoutgiubase{->}{<-}{->}{->}{->}{->}{#1}}
\newcommand{\bloivparoutgiuuno}[5]{\bloivparoutgiulab{#2}{#3}{#4}{#5}\bloivparoutgiubase{<-}{->}{->}{<-}{<-}{->}{#1}}
\newcommand{\bloivparoutgiudue}[5]{\bloivparoutgiulab{#2}{#3}{#4}{#5}\bloivparoutgiubase{->}{->}{<-}{->}{<-}{<-}{#1}}


%%%%%% SU SU SU


%%>>%%      'bloivparoutsubase','','Commento'
\newcommand{\bloivparoutsubase}[7]{\begin{picture}(4,10)
   \put(0,8){\tratteggio}
   \put(0,-8){\tratteggio}
   \put(2.5,0){\psline{#2}(1.5,0)}
   \put(2.5,0){\punto}
   \put(2.5,0){\psline{#1}(-2,8)}
   \put(2.5,0){\psline{#3}(-2,-8)}
   \put(2.5,10){\psline{#4}(-2,8)(0.5;120)}
   \put(2.5,10){\psline{#6}(-2,-8)(0.5;-120)}
   \psline(0.5,-8)(0,-8)
   \psline(0.5,8)(0,8)
   \psline(0.5,2)(0,2)
   \psline(0.5,18)(0,18)
   \put(2.5,10){
   \put(0,0){\pscircle[linewidth=0.4pt]{0.5}}
   \psline(0.5;180)(0;0)
   \psline(0.5; 60)(0;0)
   \psline(0.5;-60)(0;0)
   \psline{#5}(0.5,0)(1.5,0)
    #7
    }
\end{picture}}

\newcommand{\bloivparoutsulab}[4]{\begin{picture}(0,10)
   \put(3.25,10.25){\makebox(0,0)[lb]{$#1$}}
   \put(2.75,0.25){\makebox(0,0)[lb]{$#2$}}
   \put(1.75,13){\makebox(0,0)[lb]{$#3$}}
   \put(1.75,7){\makebox(0,0)[lt]{$#4$}}
\end{picture}}


\newcommand{\bloivparoutsu}[5]{\bloivparoutsulab{#2}{#3}{#4}{#5}\bloivparoutsubase{->}{<-}{->}{->}{->}{->}{#1}}
\newcommand{\bloivparoutsuuno}[5]{\bloivparoutsulab{#2}{#3}{#4}{#5}\bloivparoutsubase{<-}{->}{->}{<-}{<-}{->}{#1}}
\newcommand{\bloivparoutsudue}[5]{\bloivparoutsulab{#2}{#3}{#4}{#5}\bloivparoutsubase{->}{->}{<-}{->}{<-}{<-}{#1}}


%%%%%% thdot thdot

%%>>%%      'thdot','{30}(0,-2.5)(8,15)B',''
\newcommand{\thdot}[1]{\begin{picture}(0,0)
 \pscircle*(0.25;#1){0.25}
\end{picture}}


\newcommand{\linex}[1]{\begin{picture}(#1,10)
 \psline(#1,0)
 \psline(0,10)(#1,10)
\end{picture}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% 1111

%%>>%%      'bloivquaingiubase','(0,-20)(8,15)B','Commento'
\newcommand{\bloivquaingiubase}[9]{\begin{picture}(4,10)
   \put(0,0){\tratteggio}
   \put(0,10){\psline{#1}(3.0,0)}
   \put(3.0,10){\punto}
   \psline{#2}(3,10)(4,10)
%   \psline{#3}(3,10)(3,0.3)
%   \put(3,0){\psarc{-}{0.3}{-90}{90}}
%   \psline{#3}(3,-0.3)(3,-6)(4,-6)
   \put(3,0){\psline{#3}(0,10)(0,0.3)(0.3;80)(0.3;60)(0.3;40)(0.3;20)(0.3;0)(0.3;-20)(0.3;-40)(0.3;-60)(0.3;-80)(0,-0.3)(0,-6)(1,-6)}
   \put(1.5,0){\piu}
   \put(1.5,0){#9}
   \psline{#5}(2,0)(4,0)
   \psline{#6}(1.5,-0.5)(1.5,-16)(4,-16)
   \psline{#4}(0,0)(1,0)
   \put(4,0){$#7$}
   \put(4,-16){$#8$}
\end{picture}}


\newcommand{\bloivquaingiulab}[4]{\begin{picture}(0,10)
   \put(2.0,10.25){\makebox(0,0)[b]{$#1$}}
   \put(0.75,0.25){\makebox(0,0)[rb]{$#2$}}
   \put(2.5,5){\makebox(0,0)[r]{$#3$}}
   \put(2.0,-11){\makebox(0,0)[l]{$#4$}}
\end{picture}}


\newcommand{\bloivquaingiu}[7]{\bloivquaingiulab{#4}{#5}{#6}{#7}\bloivquaingiubase{->}{->}{->}{<-}{<-}{<-}{#1}{#2}{#3}}
\newcommand{\bloivquaingiuuno}[7]{\bloivquaingiulab{#4}{#5}{#6}{#7}\bloivquaingiubase{<-}{<-}{->}{->}{->}{<-}{#1}{#2}{#3}}
\newcommand{\bloivquaingiudue}[7]{\bloivquaingiulab{#4}{#5}{#6}{#7}\bloivquaingiubase{<-}{->}{<-}{->}{<-}{->}{#1}{#2}{#3}}

%%%%%%%%

%%>>%%      'bloivquainsubase','','Commento'
\newcommand{\bloivquainsubase}[9]{\begin{picture}(4,10)
   \put(0,0){\tratteggio}
   \put(0,0){\psline{#1}(1,0)}
   \put(1,0){\punto}
   \psline{#2}(1,0)(4,0)
   \psline{#3}(1,0)(1,-16)(4,-16)
   \psline{#4}(0,10)(2,10)
   \put(2.5,10){\piu}
   \put(2.5,10){#9}
   \psline{#5}(3,10)(4,10)
   \put(2.5,0){\psline{#6}(0,9.5)(0,0.3)(0.3;80)(0.3;60)(0.3;40)(0.3;20)(0.3;0)(0.3;-20)(0.3;-40)(0.3;-60)(0.3;-80)(0,-0.3)(0,-6)(1.5,-6)}
   \put(4,0){$#7$}
   \put(4,-16){$#8$}
\end{picture}}

\newcommand{\bloivquainsulab}[4]{\begin{picture}(0,10)
   \put(1.0,10.25){\makebox(0,0)[b]{$#1$}}
   \put(1,0.5){\makebox(0,0)[b]{$#2$}}
   \put(2,5){\makebox(0,0)[r]{$#3$}}
   \put(1.5,-11){\makebox(0,0)[l]{$#4$}}
\end{picture}}

\newcommand{\bloivquainsu}[7]{\bloivquainsulab{#4}{#5}{#6}{#7}\bloivquainsubase{->}{->}{->}{<-}{<-}{<-}{#1}{#2}{#3}}
\newcommand{\bloivquainsuuno}[7]{\bloivquainsulab{#4}{#5}{#6}{#7}\bloivquainsubase{<-}{<-}{->}{->}{->}{<-}{#1}{#2}{#3}}
\newcommand{\bloivquainsudue}[7]{\bloivquainsulab{#4}{#5}{#6}{#7}\bloivquainsubase{<-}{->}{<-}{->}{<-}{->}{#1}{#2}{#3}}

%%%%%%%%%%% 3333

%%>>%%      'bloivquaoutgiubase','','Commento'
\newcommand{\bloivquaoutgiubase}[7]{\begin{picture}(4,10)
   \put(0,0){\tratteggio}
   \put(0,10){\psline{#1}(1,0)}
   \put(1,10){\punto}
   \psline{#2}(1,10)(4,10)
   \put(1,0){\psline{#3}(0,10)(0,0.3)(0.3;80)(0.3;60)(0.3;40)(0.3;20)(0.3;0)(0.3;-20)(0.3;-40)(0.3;-60)(0.3;-80)(0,-0.3)(0,-6)(-1,-6)}
   \put(2.5,0){\piu}
   \put(2.5,0){#7}
   \psline{#5}(3,0)(4,0)
   \psline{#6}(2.5,-0.5)(2.5,-16)(0,-16)
   \psline{#4}(0,0)(2,0)
\end{picture}}


\newcommand{\bloivquaoutgiulab}[4]{\begin{picture}(0,10)
   \put(1,10.25){\makebox(0,0)[b]{$#1$}}
   \put(3.25,0.25){\makebox(0,0)[lb]{$#2$}}
   \put(1.5,5){\makebox(0,0)[l]{$#3$}}
   \put(2,-11){\makebox(0,0)[r]{$#4$}}
\end{picture}}


\newcommand{\bloivquaoutgiu}[5]{\bloivquaoutgiulab{#2}{#3}{#4}{#5}\bloivquaoutgiubase{<-}{<-}{->}{->}{->}{<-}{#1}}
\newcommand{\bloivquaoutgiuuno}[5]{\bloivquaoutgiulab{#2}{#3}{#4}{#5}\bloivquaoutgiubase{->}{->}{->}{<-}{<-}{<-}{#1}}
\newcommand{\bloivquaoutgiudue}[5]{\bloivquaoutgiulab{#2}{#3}{#4}{#5}\bloivquaoutgiubase{<-}{->}{<-}{->}{<-}{->}{#1}}

%%%%%%%%%%% 4444

%%>>%%      'bloivquaoutsubase','','Commento'
\newcommand{\bloivquaoutsubase}[7]{\begin{picture}(4,10)
   \put(0,0){\tratteggio}
   \put(0,0){\psline{#1}(3,0)}
   \put(3,0){\punto}
   \psline{#2}(3,0)(4,0)
   \psline{#3}(3,0)(3,-16)(0,-16)
   \put(1.5,10){\piu}
   \put(1.5,10){#7}
   \psline{#5}(2,10)(4,10)
   \put(1.5,0){\psline{#6}(0,9.5)(0,0.3)(0.3;80)(0.3;60)(0.3;40)(0.3;20)(0.3;0)(0.3;-20)(0.3;-40)(0.3;-60)(0.3;-80)(0,-0.3)(0,-6)(-1.5,-6)}
   \psline{#4}(0,10)(1,10)
\end{picture}}


\newcommand{\bloivquaoutsulab}[4]{\begin{picture}(0,10)
   \put(3,10.25){\makebox(0,0)[b]{$#1$}}
   \put(3,0.25){\makebox(0,0)[b]{$#2$}}
   \put(2,5){\makebox(0,0)[l]{$#3$}}
   \put(2.5,-11){\makebox(0,0)[r]{$#4$}}
\end{picture}}


\newcommand{\bloivquaoutsu}[5]{\bloivquaoutsulab{#2}{#3}{#4}{#5}\bloivquaoutsubase{<-}{<-}{->}{->}{->}{<-}{#1}}
\newcommand{\bloivquaoutsuuno}[5]{\bloivquaoutsulab{#2}{#3}{#4}{#5}\bloivquaoutsubase{->}{->}{->}{<-}{<-}{<-}{#1}}
\newcommand{\bloivquaoutsudue}[5]{\bloivquaoutsulab{#2}{#3}{#4}{#5}\bloivquaoutsubase{<-}{->}{<-}{->}{<-}{->}{#1}}



%%%%%%%%%%%%%%%%%%%%%% Mason: Loop %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%>>%%        'indxver','{4}{5}{3}{4}(0,-2.5)(8,15)B','(x,y,3,4): \\ \\ (x,y)=(4,5);'
  \newcommand{\indxver}[4]{
  \rput(0,#2){
  \rput(#1,0){\psline(-0.25,0)(0.25,0)}
  \rput(-0.5,0){\rput[r](#1,0){\tiny #3}}
  \rput(0.5,0){\rput[l](#1,0){\tiny #4}}  }
  }
 %
%%>>%%        'indxorzsu','{2}{2}{3}','(x,2,3): \\ \\ (x,10)=(2,10);'
  \newcommand{\indxorzsu}[3]{
  \psline(#1,9.75)(#1,10.25)
  \rput[b](#1,10.5){\tiny #2}
  \rput[t](#1,9.5){\tiny #3}
  }
 %
%%>>%%        'indxorzgiu','{2}{2}{3}','(x,2,3): \\ \\ (x,0)=(2,0);'
  \newcommand{\indxorzgiu}[3]{
  \psline(#1,-0.25)(#1,0.25)
  \rput[b](#1,0.5){\tiny #2}
  \rput[t](#1,-0.5){\tiny #3}
  }
 %
%%>>%%        'loopxysnt','{2}{4}{->}{<<-}{linecolor=blue}',''
  \newcommand{\loopxysnt}[5]{%
  \rput(1,4.5){\psline[#5]{#3}(-1,#2)(-#1,#2)}
  \rput(1,4.0){\psarc[#5](-#1,#2){0.5}{90}{180}}
  \rput(0.5,4){\psline[#5](-#1,#2)(-#1,1)}
  \rput(0.5,6){\psline[#5](-#1,-1)(-#1,-#2)}
  \rput(1,6.0){\psarc[#5](-#1,-#2){0.5}{180}{270}}
  \rput(1,5.5){\psline[#5]{#4}(-1,-#2)(-#1,-#2)}
  }
%%>>%%        'loopxydst','{2}{4}{->}{<<-}{linecolor=blue}','\small Mezzi anelli.\\ Centro in (0,5). \\ Parametri: \\ 1=larg=2\\ 2=alt/2=4\\ 3=-$>$\\ 4=$<<$- \\ 5=linecolor=blue'
  \newcommand{\loopxydst}[5]{
  \rput(-1,4.5){\psline[#5]{#3}(1,#2)(#1,#2)}
  \rput(-1,4.0){\psarc[#5](#1,#2){0.5}{0}{90}}
  \rput(-0.5,4){\psline[#5](#1,#2)(#1,1)}
  \rput(-0.5,6){\psline[#5](#1,-1)(#1,-#2)}
  \rput(-1,6.0){\psarc[#5](#1,-#2){0.5}{270}{0}}
  \rput(-1,5.5){\psline[#5]{#4}(1,-#2)(#1,-#2)}
  }
%%>>%%        'loopxsnt','{2}{->}{<<-}{linecolor=magenta}',''
  \newcommand{\loopxsnt}[4]{\loopxysnt{#1}{5}{#2}{#3}{#4}}

%%>>%%        'loopxdst','{2}{->}{<<-}{linecolor=magenta}','\small Mezzi anelli.\\ Centro in (0,5).\\ Altezza 10. \\ Parametri: \\ 1=larg=2\\ 2=-$>$\\ 3=$<<$- \\ 4=linecolor=magenta'
  \newcommand{\loopxdst}[4]{\loopxydst{#1}{5}{#2}{#3}{#4}}
  %
%%>>%%        'loopxsntor','{2}{linestyle=dashed}',''
  \newcommand{\loopxsntor}[2]{\loopxsnt{#1}{<-}{-}{#2}}
%%>>%%        'loopxsntaor','{2}{linestyle=dashed}','\small Mezzi anelli.\\ Centro in (0,5).\\ Altezza 10. \\ Senso: or, aor. \\ Parametri: \\ 1=larg=2;\\ 2=linestyle=dashed;'
  \newcommand{\loopxsntaor}[2]{\loopxsnt{#1}{-}{<-}{#2}}
%%>>%%        'loopsntor','{linewidth=1.5pt}(-4,-2.5)(8,15)',''
  \newcommand{\loopsntor}[1]{\loopxsnt{4}{<-}{-}{#1}}
%%>>%%        'loopsntaor','{linewidth=1.5pt}',''
  \newcommand{\loopsntaor}[1]{\loopxsnt{4}{-}{<-}{#1}}
%%>>%%        'loopvisntor','{linewidth=1.5pt}',''
  \newcommand{\loopvisntor}[1]{\loopxsnt{3}{<-}{-}{#1}}
%%>>%%        'loopvisntaor','{linewidth=1.5pt}',''
  \newcommand{\loopvisntaor}[1]{\loopxsnt{3}{-}{<-}{#1}}
%%>>%%        'loopivsntor','{linewidth=1.5pt}',''
  \newcommand{\loopivsntor}[1]{\loopxsnt{2}{<-}{-}{#1}}
%%>>%%        'loopivsntaor','{linewidth=1.5pt}','\small Mezzi anelli.\\ Centro in (0,5).\\ Altezza 10. \\ Senso: or, aor. \\ Larghezza 4,3,2. \\ Parametri: \\ 1=linewidth=1.5pt;'
  \newcommand{\loopivsntaor}[1]{\loopxsnt{2}{-}{<-}{#1}}
 %
%%>>%%        'loopxysntor','{2}{4}{linecolor=red}',''
  \newcommand{\loopxysntor}[3]{\loopxysnt{#1}{#2}{<-}{-}{#3}}
%%>>%%        'loopxysntaor','{2}{4}{linecolor=red}','\small Mezzi anelli.\\ Centro in (0,5).\\ Senso: or, aor. \\ Parametri: \\ 1=larg=2;\\ 2=alt/2=4;\\ 3=linecolor=red;'
  \newcommand{\loopxysntaor}[3]{\loopxysnt{#1}{#2}{-}{<-}{#3}}
 %
%%>>%%        'loopxdstor','{2}{linecolor=green}',''
  \newcommand{\loopxdstor}[2]{\loopxdst{#1}{-}{<-}{#2}}
%%>>%%        'loopxdstaor','{2}{linecolor=green}','\small Mezzi anelli.\\ Centro in (0,5).\\ Altezza 10.\\ Senso: or, aor. \\ Parametri: \\ 1=larg=2;\\ 2=linecolor=green;'
  \newcommand{\loopxdstaor}[2]{\loopxdst{#1}{<-}{-}{#2}}
%%>>%%        'loopdstor','{linecolor=green}',''
  \newcommand{\loopdstor}[1]{\loopxdst{4}{-}{<-}{#1}}
%%>>%%        'loopdstaor','{linecolor=green}',''
  \newcommand{\loopdstaor}[1]{\loopxdst{4}{<-}{-}{#1}}
%%>>%%        'loopvidstor','{linecolor=green}',''
  \newcommand{\loopvidstor}[1]{\loopxdst{3}{-}{<-}{#1}}
%%>>%%        'loopvidstaor','{linecolor=green}',''
  \newcommand{\loopvidstaor}[1]{\loopxdst{3}{<-}{-}{#1}}
%%>>%%        'loopivdstor','{linecolor=green}',''
  \newcommand{\loopivdstor}[1]{\loopxdst{2}{-}{<-}{#1}}
%%>>%%        'loopivdstaor','{linecolor=green}','\small Mezzi anelli.\\ Centro in (0,5).\\ Altezza 10.\\ Larghezza 4,3,2.\\ Senso: or, aor. \\ Parametri: \\ 1=linecolor=green;'
  \newcommand{\loopivdstaor}[1]{\loopxdst{2}{<-}{-}{#1}}
 %
%%>>%%        'loopxydstor','{2}{4}{linecolor=blue}',''
  \newcommand{\loopxydstor}[3]{\loopxydst{#1}{#2}{-}{<-}{#3}}
%%>>%%        'loopxydstaor','{2}{4}{linecolor=blue}','\small Mezzi anelli.\\ Centro in (0,5).\\ Senso: or, aor. \\ Parametri: \\ 1=larg=2;\\ 2=alt/2=4;\\ 3=linecolor=blue;'
  \newcommand{\loopxydstaor}[3]{\loopxydst{#1}{#2}{<-}{-}{#3}}
 %
%%>>%%        'loopor','{linecolor=red}(-4,-2.5)(8,15)',''
  \newcommand{\loopor}[1]{\loopxdstor{4}{#1}\loopxsntor{4}{#1}  }
%%>>%%        'loopaor','{linecolor=red}',''
  \newcommand{\loopaor}[1]{\loopxdstaor{4}{#1} \loopxsntaor{4}{#1}  }
%%>>%%        'loopvior','{linecolor=red}',''
  \newcommand{\loopvior}[1]{\loopxdstor{3}{#1}\loopxsntor{3}{#1}  }
%%>>%%        'loopviaor','{linecolor=red}',''
  \newcommand{\loopviaor}[1]{\loopxdstaor{3}{#1} \loopxsntaor{3}{#1}  }
%%>>%%        'loopivor','{linecolor=red}',''
  \newcommand{\loopivor}[1]{\loopxdstor{2}{#1}\loopxsntor{2}{#1}  }
%%>>%%        'loopivaor','{linecolor=red}','\small Anelli interi.\\ Centro in (0,5).\\ Altezza 10.\\ Larghezza 4,3,2.\\ Senso: or, aor. \\ Parametri: \\ 1=linecolor=red;'
  \newcommand{\loopivaor}[1]{\loopxdstaor{2}{#1} \loopxsntaor{2}{#1}  }
%
%%>>%%        'loopxor','{2.5}{linecolor=cyan}',''
  \newcommand{\loopxor}[2]{\loopxdstor{#1}{#2}\loopxsntor{#1}{#2}  }
%%>>%%        'loopxaor','{2.5}{linecolor=cyan}','\small Anelli interi.\\ Centro in (0,5).\\ Altezza 10.\\ Senso: or, aor. \\ Parametri: \\ 1=larg=2.5;\\ 2=linecolor=cyan;'
  \newcommand{\loopxaor}[2]{\loopxdstaor{#1}{#2} \loopxsntaor{#1}{#2}  }
%
%%>>%%        'loopxyor','{3}{4}{linecolor=blue}',''
  \newcommand{\loopxyor}[3]{\loopxydstor{#1}{#2}{#3}\loopxysntor{#1}{#2}{#3}  }
%%>>%%        'loopxyaor','{3}{4}{linecolor=blue}','\small Anelli interi.\\ Centro in (0,5).\\ Senso: or, aor. \\ Parametri: \\ 1=larg=2;\\ 2=alt/2=2;\\ 3=linecolor=blue;'
  \newcommand{\loopxyaor}[3]{\loopxydstaor{#1}{#2}{#3}\loopxysntaor{#1}{#2}{#3}  }

%%%%%%%%%%%%%%%  IN IN

%\newcommand{\bloparingiu}[3]{\begin{picture}(8,10)
%   \put(0,0){\tratteggio}
%   \put(0,10){\psline{->}(2,0)}
%   \put(2,10){\punto}
%   \put(2,10){\psline{->}(5,8)}
%   \put(2,10){\psline{->}(5,-8)}
%   \put(2,0){\psline{->}(5,8)(0.5;58)}
%   \put(2,0){\psline{->}(5,-8)(0.5;-58)}
%   \psline(7,-8)(8,-8)
%   \psline(7,8)(8,8)
%   \psline(7,2)(8,2)
%   \psline(7,18)(8,18)
%   \put(2,0){
%   \put(0,0){\pscircle[linewidth=0.4pt]{0.5}}
%   \psline(0.5; 0)(0;0)
%   \psline(0.5; 120)(0;0)
%   \psline(0.5; 240)(0;0)
%   \psline{->}(-0.5,0)(-2,0)
%    #3
%    }
%    \put(8,8){$#1$}
%    \put(8,-8){$#2$}
%\end{picture}}
%
%\newcommand{\bloviparingiu}[3]{\begin{picture}(6,10)
%   \put(0,0){\tratteggio}
%   \put(0,10){\psline{->}(2,0)}
%   \put(2,10){\punto}
%   \put(2,10){\psline{->}(3,8)}
%   \put(2,10){\psline{->}(3,-8)}
%   \put(2,0){\psline{->}(3,8)(0.5;58)}
%   \put(2,0){\psline{->}(3,-8)(0.5;-58)}
%   \psline(5,-8)(6,-8)
%   \psline(5,8)(6,8)
%   \psline(5,2)(6,2)
%   \psline(5,18)(6,18)
%   \put(2,0){
%   \put(0,0){\pscircle[linewidth=0.4pt]{0.5}}
%   \psline(0.5; 0)(0;0)
%   \psline(0.5; 120)(0;0)
%   \psline(0.5; 240)(0;0)
%   \psline{->}(-0.5,0)(-2,0)
%    #3
%    }
%    \put(6,8){$#1$}
%    \put(6,-8){$#2$}
%\end{picture}}
%

%
%
%\newcommand{\bloviparoutgiu}[1]{\begin{picture}(6,10)
%   \put(0,8){\tratteggio}
%   \put(0,-8){\tratteggio}
%   \put(6,10){\psline{->}(-2,0)}
%   \put(4,10){\punto}
%   \put(4,10){\psline{->}(-3,8)}
%   \put(4,10){\psline{->}(-3,-8)}
%   \put(4,0){\psline{->}(-3,8)(0.5;-238)}
%   \put(4,0){\psline{->}(-3,-8)(0.5;238)}
%   \psline(1,-8)(0,-8)
%   \psline(1,8)(0,8)
%   \psline(1,2)(0,2)
%   \psline(1,18)(0,18)
%   \put(4,0){
%   \put(0,0){\pscircle[linewidth=0.4pt]{0.5}}
%   \psline(0.5;180)(0;0)
%   \psline(0.5; 60)(0;0)
%   \psline(0.5;-60)(0;0)
%   \psline{->}(0.5,0)(2,0)
%    #1
%    }
%\end{picture}}

%%
%\newcommand{\aggiungi}[1]{\begin{picture}(0,0) #1 \end{picture}}


%\newcommand{\addgiusolo}[2]{\addgiuvar{4}{#1}{#2}}
\newcommand{\addsusolo}[2]{\addsuvar{4}{#1}{#2}}
%\newcommand{\escigiusolo}[1]{\escigiuvar{4}{#1}}
%\newcommand{\escisusolo}[1]{\escisuvar{4}{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%








\endinput

